Sources of Uncertainty in 3D Scene Reconstruction

The process of 3D scene reconstruction can be affected by numerous uncertainty sources in real-world scenes. While Neural Radiance Fields (NeRFs) and 3D Gaussian Splatting (GS) achieve high-fidelity rendering, they lack built-in mechanisms to directly address or quantify uncertainties arising from the presence of noise, occlusions, confounding outliers, and imprecise camera pose inputs. In this paper, we introduce a taxonomy that categorizes different sources of uncertainty inherent in these methods. Moreover, we extend NeRF- and GS-based methods with uncertainty estimation techniques, including learning uncertainty outputs and ensembles, and perform an empirical study to assess their ability to capture the sensitivity of the reconstruction. Our study highlights the need for addressing various uncertainty aspects when designing NeRF/GS-based methods for uncertainty-aware 3D reconstruction.

==> results/noisyview-mipnerf360-avg/groupplot-avg-var-old.tex <==


\pgfplotsset{every axis title/.append style={at={(0.5,0.80)}}} %{at={(0.5,0.84)}}}
\pgfplotsset{every axis x label/.append style={at={(0.5,0.05)}}}
\pgfplotsset{every axis y label/.append style={at={(0.15,0.5)}}}


\begin{tikzpicture}
\tikzstyle{every node}=[font=\scriptsize]
\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\definecolor{lightgray204}{RGB}{204,204,204}


\begin{groupplot}[
  group style={group size= 2 by 1, horizontal sep=1.25cm, vertical sep=.5cm},
  tick align=outside,
  tick pos=left,
  grid=both,
  xlabel={Noise scale},
  xlabel={Avg. variance},
  xmin=-0.1, xmax=2.1,
  xtick={0,1,2},
  xticklabels={0,0.1,0.2},
  xtick style={color=black},
  x grid style={darkgray176,solid},
  y grid style={darkgray176,solid},
  ytick style={color=black},
  tick label style={font=\tiny}
]

%% Gaussian Noise
\nextgroupplot[
height=\figureheight,
width=\figurewidth,
legend cell align={left},
legend columns=1,%3,
legend style={
  nodes={scale=0.8},
  fill opacity=0.8, 
  draw opacity=1, 
  text opacity=1, 
  at={(2.65,0.0)}, %{(0.03,1.1)}, 
  anchor=south west,
  draw=lightgray204},
%title={Gaussian Noise},
xlabel={Noise scale},
xticklabels={0,0.1,0.2},
%xticklabel=\empty,
%ylabel={PSNR~$\rightarrow$},
ymin=-0.000914076997923985, ymax=0.0194333730252058,
ytick style={color=black}
]
\addplot [thick, steelblue31119180, mark=*, mark size=1, mark options={solid}]
table {%
0 0.00296415873647978
1 0.00722684380080965
2 0.0185084889332453
};
\addlegendentry{Active-Nerfacto}
\addplot [thick, darkorange25512714, mark=*, mark size=1, mark options={solid}]
table {%
0 0.00345189025392756
1 0.00615475181904104
2 0.0169340694944064
};
\addlegendentry{Active-Splatfacto}
\addplot [thick, forestgreen4416044, mark=*, mark size=1, mark options={solid}]
table {%
0 0.000153489754464115
1 0.000145964218972949
2 0.00012634604354389
};
\addlegendentry{MC-Dropout-Nerfacto}
\addplot [thick, crimson2143940, mark=*, mark size=1, mark options={solid}]
table {%
0 2.28801544229403e-05
1 1.08070940364592e-05
2 1.35734823743405e-05
};
\addlegendentry{Laplace-NeRF}
\addplot [thick, mediumpurple148103189, mark=*, mark size=1, mark options={solid}]
table {%
0 0.000834113146993332
1 0.000809037213912234
2 0.000777921632915321
};
\addlegendentry{Ensemble-Nerfacto}
\addplot [thick, sienna1408675, mark=*, mark size=1, mark options={solid}]
table {%
0 0.00284104024467524
1 0.00481508229131578
2 0.00799068006583386
};
\addlegendentry{Ensemble-Splatfacto}



%% Gaussian blur
\nextgroupplot[
height=\figureheight,
width=\figurewidth,
%title={Gaussian Blur},
xlabel={Kernel size},
xticklabels={0,5,7},
%xticklabel=\empty,
% ylabel={SSIM~$\rightarrow$},
ymin=-0.000223647451502984, ymax=0.0049006123194431,
ytick style={color=black}
]
\addplot [thick, steelblue31119180, mark=*, mark size=1, mark options={solid}]
table {%
0 0.00296415873647978
1 0.00126303605065914
2 0.000719452771591023
};
\addplot [thick, darkorange25512714, mark=*, mark size=1, mark options={solid}]
table {%
0 0.00345189025392756
1 0.00253620855801273
2 0.00466769142076373
};
\addplot [thick, forestgreen4416044, mark=*, mark size=1, mark options={solid}]
table {%
0 0.000153489754464115
1 0.000105565228295745
2 7.42438569432124e-05
};
\addplot [thick, crimson2143940, mark=*, mark size=1, mark options={solid}]
table {%
0 2.28801544229403e-05
1 2.32073376764674e-05
2 9.27344717638334e-06
};
\addplot [thick, mediumpurple148103189, mark=*, mark size=1, mark options={solid}]
table {%
0 0.000834113146993332
1 0.000635726594029822
2 0.000561221303845135
};
\addplot [thick, sienna1408675, mark=*, mark size=1, mark options={solid}]
table {%
0 0.00284104024467524
1 0.00213266460741579
2 0.0016524754804171
};


\end{groupplot}

\end{tikzpicture}

==> results/varyingview-mipnerf360-auce-coverage/active-nerfacto/avg_length.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.039, xmax=1.039,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.0092473089573337, ymax=0.2096960992165,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.01 0.000704664141476923
0.02 0.00140943906973139
0.03 0.00211443552256136
0.04 0.00281976443921287
0.05 0.00352553735614228
0.06 0.00423186687495779
0.07 0.00493886464535305
0.08 0.00564664417853039
0.09 0.0063553196483309
0.1 0.00706500639289143
0.11 0.00777582109808002
0.12 0.00848788119364855
0.13 0.00920130442478725
0.14 0.00991621270881791
0.15 0.0106327280919128
0.16 0.0113509746431033
0.17 0.012071078270838
0.18 0.0127931684351419
0.19 0.0135173752917399
0.2 0.014243830137008
0.21 0.0149726722409524
0.22 0.0157040406556549
0.23 0.0164380760385944
0.24 0.0171749214434386
0.25 0.017914730787166
0.26 0.0186576558599965
0.27 0.0194038511188181
0.28 0.0201534815979738
0.29 0.0209067133665393
0.3 0.0216637142592539
0.31 0.0224246661532588
0.32 0.0231897458020598
0.33 0.0239591453908552
0.34 0.0247330566096963
0.35 0.0255116866332524
0.36 0.0262952400698182
0.37 0.0270839321004275
0.38 0.0278779916581442
0.39 0.0286776523858076
0.4 0.029483156060019
0.41 0.0302947570344107
0.42 0.0311127236060577
0.43 0.0319373281649565
0.44 0.032768861423444
0.45 0.0336076234872687
0.46 0.0344539353048551
0.47 0.0353081279217642
0.48 0.0361705458078708
0.49 0.0370415608627242
0.5 0.0379215616765199
0.51 0.0388109494833054
0.52 0.0397101617701682
0.53 0.0406196445320041
0.54 0.0415398855241294
0.55 0.0424713910204705
0.56 0.0434147015999681
0.57 0.0443704015270357
0.58 0.0453390915233749
0.59 0.0463214349602912
0.6 0.04731812742675
0.61 0.0483299145896775
0.62 0.0493576052408592
0.63 0.0504020541951781
0.64 0.0514641982363286
0.65 0.0525450306427909
0.66 0.0536456460708756
0.67 0.0547672082425635
0.68 0.0559109996567245
0.69 0.0570784149579206
0.7 0.0582709677752429
0.71 0.0594903396082141
0.72 0.0607383521057815
0.73 0.0620170312203152
0.74 0.0633286326387764
0.75 0.0646756230015694
0.76 0.0660608074227149
0.77 0.0674872848840079
0.78 0.0689585936571718
0.79 0.0704786955761453
0.8 0.0720521514465777
0.81 0.073684152478516
0.82 0.0753807240191148
0.83 0.0771488558739468
0.84 0.0789967692657397
0.85 0.0809341873458611
0.86 0.0829727966465814
0.87 0.0851267327671129
0.88 0.0874134009932174
0.89 0.0898545596596025
0.9 0.0924779293669206
0.91 0.0953196556090188
0.92 0.0984281033424516
0.93 0.101870306070515
0.94 0.105743089054435
0.95 0.110194259488181
0.96 0.115467087585555
0.97 0.122008106659902
0.98 0.13079330658179
0.99 0.144819793863567
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.000840489793773312
0.02 0.00168111171422847
0.03 0.00252199783470822
0.04 0.00336328061223745
0.05 0.00420509316672092
0.06 0.00504756893826712
0.07 0.00589084234610552
0.08 0.00673504838967691
0.09 0.00758032252739873
0.1 0.00842680311454091
0.11 0.00927462853898946
0.12 0.0101239401316882
0.13 0.0109748771389272
0.14 0.0118275859756264
0.15 0.0126822121576546
0.16 0.0135389016061179
0.17 0.0143978069867984
0.18 0.0152590815519501
0.19 0.0161228806958279
0.2 0.0169893617923584
0.21 0.0178586900896912
0.22 0.0187310319840182
0.23 0.0196065526374986
0.24 0.020485427360323
0.25 0.0213678375091202
0.26 0.0222539627999054
0.27 0.0231439892578632
0.28 0.0240381138323448
0.29 0.0249365310809903
0.3 0.0258394469630285
0.31 0.0267470726004086
0.32 0.0276596238097664
0.33 0.0285773280900292
0.34 0.0295004124001621
0.35 0.0304291254529691
0.36 0.0313637092409208
0.37 0.0323044235005015
0.38 0.033251540270084
0.39 0.0342053383185017
0.4 0.0351661064688251
0.41 0.0361341423264845
0.42 0.0371097737663325
0.43 0.0380933236275358
0.44 0.0390851350946759
0.45 0.0400855740220627
0.46 0.0410950120724464
0.47 0.0421138525229729
0.48 0.0431425045086197
0.49 0.0441814106566477
0.5 0.0452310313341928
0.51 0.0462918515648751
0.52 0.0473643903544162
0.53 0.048449177634642
0.54 0.0495467951652803
0.55 0.0506578505149249
0.56 0.0517829931276496
0.57 0.0529228983930128
0.58 0.054078308824639
0.59 0.0552500011045576
0.6 0.0564388046451337
0.61 0.0576456215282383
0.62 0.0588714011096273
0.63 0.0601171698827018
0.64 0.0613840447524652
0.65 0.0626732114598591
0.66 0.0639859674001938
0.67 0.0653237157342784
0.68 0.0666879771744722
0.69 0.0680804192318383
0.7 0.0695028334642466
0.71 0.0709572402255984
0.72 0.0724458113035007
0.73 0.0739709613976085
0.74 0.0755353741188222
0.75 0.0771420022311247
0.76 0.0787941771665491
0.77 0.0804956225231873
0.78 0.0822505215552141
0.79 0.0840636342198457
0.8 0.0859403715445112
0.81 0.0878869429307073
0.82 0.0899105316348488
0.83 0.0920194817788616
0.84 0.0942235822557855
0.85 0.0965344412822961
0.86 0.0989659937034978
0.87 0.101535106725333
0.88 0.104262541755078
0.89 0.107174243662304
0.9 0.110303269954101
0.91 0.113692743467964
0.92 0.117400354148106
0.93 0.121506052775825
0.94 0.126125319191859
0.95 0.13143445757455
0.96 0.137723638223387
0.97 0.145525462244386
0.98 0.156004018835176
0.99 0.172734151789505
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.000923505087954287
0.02 0.0018471553267429
0.03 0.00277109614014876
0.04 0.00369547251576679
0.05 0.00462043068379497
0.06 0.00554611830575748
0.07 0.00647268199091271
0.08 0.00740027014528637
0.09 0.00832903277302743
0.1 0.00925912006872546
0.11 0.0101906854653433
0.12 0.0111238836974601
0.13 0.012058868134682
0.14 0.0129957986870924
0.15 0.0139348367127295
0.16 0.0148761410097104
0.17 0.0158198813811334
0.18 0.0167662242064842
0.19 0.017715339232679
0.2 0.0186674046868508
0.21 0.019622596647245
0.22 0.0205810986112339
0.23 0.021543095920263
0.24 0.0225087773682163
0.25 0.023478343354197
0.26 0.024451990989269
0.27 0.0254299257134844
0.28 0.0264123618835736
0.29 0.0273995171338768
0.3 0.0283916129822737
0.31 0.0293888858574609
0.32 0.030391571698005
0.33 0.0313999156678604
0.34 0.0324141740838737
0.35 0.0334346141115474
0.36 0.0344615087023578
0.37 0.0354951380374677
0.38 0.0365358032708285
0.39 0.0375838086522851
0.4 0.03863946652577
0.41 0.0397031180699305
0.42 0.0407751134859798
0.43 0.0418558098761062
0.44 0.0429455812684925
0.45 0.0440448317445133
0.46 0.0451539734206193
0.47 0.0462734450680534
0.48 0.0474036981169463
0.49 0.0485452160651732
0.5 0.0496985093015271
0.51 0.0508641070986608
0.52 0.0520425796261945
0.53 0.0532345081053359
0.54 0.05444053933154
0.55 0.0556613376242642
0.56 0.0568976038747229
0.57 0.0581501053210843
0.58 0.0594196319783494
0.59 0.0607070502504858
0.6 0.0620132793606002
0.61 0.0633392877555416
0.62 0.0646861365914861
0.63 0.0660549546119389
0.64 0.067446957068536
0.65 0.0688634523930196
0.66 0.0703058770868663
0.67 0.0717757509295235
0.68 0.0732747636883689
0.69 0.0748047317449384
0.7 0.07636764293478
0.71 0.0779657003502129
0.72 0.0796012988558253
0.73 0.0812770849213935
0.74 0.082996015310586
0.75 0.084761329346299
0.76 0.0865766988412103
0.77 0.0884461871591301
0.78 0.0903744241633541
0.79 0.0923666149943941
0.8 0.0944287165220185
0.81 0.0965675543320473
0.82 0.0987910129288004
0.83 0.101108261038534
0.84 0.103530060382946
0.85 0.106069170411057
0.86 0.108740884613825
0.87 0.111563750273801
0.88 0.11456056652217
0.89 0.117759854078978
0.9 0.121197944618005
0.91 0.124922194780167
0.92 0.128996014281367
0.93 0.133507232901263
0.94 0.138582736667462
0.95 0.144416266542111
0.96 0.151326628064123
0.97 0.159899035841429
0.98 0.171412569425581
0.99 0.189795138564958
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.000971914859904658
0.02 0.00194398265384433
0.03 0.0029163557808762
0.04 0.00388918764808104
0.05 0.00486263207099734
0.06 0.00583684355687231
0.07 0.00681197724129587
0.08 0.00778818927041519
0.09 0.00876563698196224
0.1 0.00974447939344454
0.11 0.0107248767837448
0.12 0.0117069929338668
0.13 0.0126909885203458
0.14 0.0136770333272887
0.15 0.0146652948507841
0.16 0.0156559424931965
0.17 0.0166491524572344
0.18 0.0176451035042996
0.19 0.0186439714761864
0.2 0.0196459432808191
0.21 0.0206512055135724
0.22 0.0216599523017393
0.23 0.0226723756771879
0.24 0.0236886787143922
0.25 0.0247090699279365
0.26 0.0257337551653617
0.27 0.0267629527786441
0.28 0.0277968877845971
0.29 0.0288357891613292
0.3 0.0298798908794728
0.31 0.0309294387911993
0.32 0.031984684008
0.33 0.0330458859902102
0.34 0.0341133117380583
0.35 0.0351872446667576
0.36 0.0362679678740421
0.37 0.0373557800646337
0.38 0.0384509943565751
0.39 0.0395539356016201
0.4 0.040664933268308
0.41 0.0417843390737448
0.42 0.0429125276022899
0.43 0.0440498730422768
0.44 0.0451967722716127
0.45 0.0463536453097119
0.46 0.0475209276381532
0.47 0.0486990818870877
0.48 0.0498885817660004
0.49 0.0510899354776822
0.5 0.0523036842640638
0.51 0.0535303822333699
0.52 0.0547706294153921
0.53 0.0560250409256528
0.54 0.0572942916618756
0.55 0.0585790780316739
0.56 0.0598801527920031
0.57 0.0611983125377115
0.58 0.0625343876773468
0.59 0.0638892957013391
0.6 0.0652639900779774
0.61 0.0666595083998224
0.62 0.0680769603851147
0.63 0.0695175274894772
0.64 0.070982499913306
0.65 0.0724732484970317
0.66 0.0739912817136935
0.67 0.0755382052858522
0.68 0.0771157958280375
0.69 0.0787259631960113
0.7 0.0803708003729034
0.71 0.0820526318656402
0.72 0.0837739673433813
0.73 0.0855376043913676
0.74 0.0873466372327591
0.75 0.0892044874498035
0.76 0.0911150159973476
0.77 0.0930825003797123
0.78 0.0951118157875707
0.79 0.0972084321962896
0.8 0.0993786396506698
0.81 0.101629584221614
0.82 0.103969594195315
0.83 0.106408309046641
0.84 0.108957066690516
0.85 0.111629270247121
0.86 0.114441038000026
0.87 0.117411871992475
0.88 0.120565794871301
0.89 0.123932786159122
0.9 0.127551092342925
0.91 0.13147056655313
0.92 0.135757928241408
0.93 0.140505622246448
0.94 0.145847193625449
0.95 0.151986511001287
0.96 0.159259105740283
0.97 0.168280883613683
0.98 0.180397949863964
0.99 0.199744126117689
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/active-nerfacto/empirical_coverage.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.05, ymax=1.05,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 1
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.0027583630183707
0.02 0.00548032711312246
0.03 0.00819435728622878
0.04 0.010904477864189
0.05 0.0136046625981268
0.06 0.0163056064450088
0.07 0.0190080763456709
0.08 0.0217117727118472
0.09 0.0244135343285531
0.1 0.0271167269876137
0.11 0.0298258809707536
0.12 0.0325376800297104
0.13 0.0352552538493824
0.14 0.0379722321889505
0.15 0.0406955423014747
0.16 0.0434293080772886
0.17 0.0461618490239164
0.18 0.0489006940363506
0.19 0.0516421660235976
0.2 0.0543953311198108
0.21 0.0571474903953251
0.22 0.0599091666945507
0.23 0.0626844657782293
0.24 0.0654647534916032
0.25 0.068249945810756
0.26 0.0710507672676996
0.27 0.0738545412709747
0.28 0.0766741332565252
0.29 0.0795040061376285
0.3 0.0823428312921135
0.31 0.0851942299743485
0.32 0.0880579138840713
0.33 0.0909398318224713
0.34 0.0938345740503154
0.35 0.0967389270625268
0.36 0.0996577281039765
0.37 0.102592703274401
0.38 0.105544840640749
0.39 0.108515332214687
0.4 0.111502376210585
0.41 0.11450050204714
0.42 0.117523349621952
0.43 0.120566898633786
0.44 0.123628865875903
0.45 0.126714978941391
0.46 0.129826757851828
0.47 0.132960543494546
0.48 0.136120799167758
0.49 0.139298886880325
0.5 0.142503831043933
0.51 0.145738445174115
0.52 0.14900019133975
0.53 0.15229764146455
0.54 0.155624369103503
0.55 0.158980504697365
0.56 0.162374140413692
0.57 0.165812393774197
0.58 0.169282848279841
0.59 0.172794790968151
0.6 0.176351342459918
0.61 0.179946440330639
0.62 0.183588384598484
0.63 0.187277857410636
0.64 0.191024189690084
0.65 0.194810734474754
0.66 0.198661687092861
0.67 0.202573103907118
0.68 0.206548371531688
0.69 0.210597882946737
0.7 0.214714009370374
0.71 0.218907826272506
0.72 0.22318367340953
0.73 0.227545582101415
0.74 0.232001604321975
0.75 0.236563862699205
0.76 0.241230614247229
0.77 0.246012322698914
0.78 0.25092016866685
0.79 0.255965712142182
0.8 0.261154178432364
0.81 0.266502308967462
0.82 0.272027516497687
0.83 0.277745639118447
0.84 0.283682669490155
0.85 0.289862415976242
0.86 0.296305913178849
0.87 0.303063762849185
0.88 0.310175112733859
0.89 0.31769236641802
0.9 0.325677768807723
0.91 0.334240129812785
0.92 0.343470610463989
0.93 0.353544458423148
0.94 0.3647030520185
0.95 0.377288821526627
0.96 0.391863543837618
0.97 0.409428999303222
0.98 0.43217476872078
0.99 0.466473378253989
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.00619073764067179
0.02 0.0110252146264509
0.03 0.0157722467079591
0.04 0.0204748447907135
0.05 0.025159650591703
0.06 0.0298372313477578
0.07 0.0345092437596444
0.08 0.03916745155392
0.09 0.0438304329651375
0.1 0.0484834731479614
0.11 0.0531457793241717
0.12 0.0578107364107243
0.13 0.0624781028393637
0.14 0.0671446226866263
0.15 0.0718070836028199
0.16 0.0764769955867946
0.17 0.0811510238787317
0.18 0.085840237692416
0.19 0.0905316087897363
0.2 0.0952345994956092
0.21 0.0999447742640562
0.22 0.104663049149436
0.23 0.109395678633848
0.24 0.114128433055559
0.25 0.118870971696536
0.26 0.123622904306895
0.27 0.128388116575388
0.28 0.133167787668559
0.29 0.137954529913416
0.3 0.142753069711716
0.31 0.147566952030935
0.32 0.152399110656618
0.33 0.157246232977883
0.34 0.162097571574702
0.35 0.16697526060641
0.36 0.171877396554083
0.37 0.176789565349858
0.38 0.181723620793971
0.39 0.186672393106413
0.4 0.191641142515766
0.41 0.196630020797737
0.42 0.2016463331888
0.43 0.206675985624002
0.44 0.211732677805685
0.45 0.216818432001371
0.46 0.221925490463268
0.47 0.2270629845437
0.48 0.232231337737255
0.49 0.237429508684071
0.5 0.242653118425326
0.51 0.247912236837438
0.52 0.253204848868844
0.53 0.258537199772604
0.54 0.263911206533125
0.55 0.26932222979405
0.56 0.274774306239794
0.57 0.280270786201936
0.58 0.285803955558819
0.59 0.291380665273325
0.6 0.297016424451054
0.61 0.302702167112946
0.62 0.308436363972499
0.63 0.314236211335082
0.64 0.320084834422188
0.65 0.325999122146462
0.66 0.331984829676676
0.67 0.338035861804007
0.68 0.344161223570968
0.69 0.350365571482226
0.7 0.356645533907144
0.71 0.363011590961317
0.72 0.369476998776159
0.73 0.376038462208629
0.74 0.382709403217444
0.75 0.389498246558771
0.76 0.396407025853874
0.77 0.403441312819018
0.78 0.410620620315166
0.79 0.417951738736236
0.8 0.425438040650277
0.81 0.433113003905627
0.82 0.440985283164958
0.83 0.449083252005858
0.84 0.457406807533248
0.85 0.466005777455128
0.86 0.474900215367147
0.87 0.484127922725522
0.88 0.493736931378136
0.89 0.503783526867898
0.9 0.514349326948557
0.91 0.525495637766963
0.92 0.537369616471447
0.93 0.550118806822975
0.94 0.56399759973449
0.95 0.579339192731033
0.96 0.596679261950021
0.97 0.617009154588079
0.98 0.642395051490172
0.99 0.678705549234867
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.00724496863168547
0.02 0.0136325386929907
0.03 0.0198822494366912
0.04 0.0260817668388297
0.05 0.0322530650307483
0.06 0.0384035476093023
0.07 0.0445343286556464
0.08 0.050651396998692
0.09 0.0567620997565112
0.1 0.0628646276024606
0.11 0.0689570713377995
0.12 0.0750511671935489
0.13 0.0811411327277436
0.14 0.0872335505572821
0.15 0.093326226041551
0.16 0.0994161729024842
0.17 0.105511574412182
0.18 0.11160561417017
0.19 0.117708447306624
0.2 0.123802948017923
0.21 0.129901886938171
0.22 0.136016319726518
0.23 0.14213997695791
0.24 0.148276094748602
0.25 0.154403819182092
0.26 0.160542128895648
0.27 0.166691044248231
0.28 0.172843329214111
0.29 0.179014213297856
0.3 0.185180654088551
0.31 0.191363061429354
0.32 0.197553174260942
0.33 0.203751391532607
0.34 0.209963445237872
0.35 0.216193151612123
0.36 0.222435339186079
0.37 0.228690264234508
0.38 0.234956764750687
0.39 0.241249965185866
0.4 0.247547709649328
0.41 0.253874160269806
0.42 0.260220799380202
0.43 0.266587344527009
0.44 0.27296272297724
0.45 0.279357487162408
0.46 0.285783403114128
0.47 0.292227423191604
0.48 0.298695339230492
0.49 0.305190022659071
0.5 0.311713754503415
0.51 0.318258447581082
0.52 0.324832794458945
0.53 0.331436971662394
0.54 0.338076011384263
0.55 0.344745767277276
0.56 0.351445441329647
0.57 0.358185079957216
0.58 0.364965361667976
0.59 0.371790903506418
0.6 0.378654008586164
0.61 0.385559254361677
0.62 0.392509484008366
0.63 0.399518240928071
0.64 0.406579493698789
0.65 0.413690757231741
0.66 0.420862619461554
0.67 0.428089568119777
0.68 0.435382635498903
0.69 0.442738706421782
0.7 0.45016680302616
0.71 0.457673670100547
0.72 0.465268046272076
0.73 0.472948458934279
0.74 0.480731052304998
0.75 0.488602624893226
0.76 0.496576013730663
0.77 0.504665437280599
0.78 0.512880442823531
0.79 0.521230316895801
0.8 0.52972552163207
0.81 0.538380142858672
0.82 0.54719391497173
0.83 0.55620561154835
0.84 0.56543107040557
0.85 0.574894634563644
0.86 0.584614435506211
0.87 0.594621492048456
0.88 0.604965265208515
0.89 0.615704132752856
0.9 0.626866080731182
0.91 0.638553711877531
0.92 0.650855117529712
0.93 0.663936092420405
0.94 0.677963214162448
0.95 0.693235127764481
0.96 0.710217988510644
0.97 0.72972517131316
0.98 0.753413043475934
0.99 0.785954885046432
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.0101039585731854
0.02 0.0174664277311492
0.03 0.0246487823182506
0.04 0.0317566886866266
0.05 0.0388243899556113
0.06 0.0458763617786859
0.07 0.0528997841791999
0.08 0.059904068130839
0.09 0.0668983822443339
0.1 0.0738873467181317
0.11 0.0808676346417567
0.12 0.0878458067946476
0.13 0.0948203458421128
0.14 0.101788057028478
0.15 0.108756225710252
0.16 0.115717543131997
0.17 0.122677209823545
0.18 0.129637330420695
0.19 0.136591468417638
0.2 0.143547659698796
0.21 0.150513396480901
0.22 0.15747831430231
0.23 0.164453485449848
0.24 0.171428788072318
0.25 0.178405477953769
0.26 0.18538585985669
0.27 0.192372609434649
0.28 0.199367346976224
0.29 0.206358972721144
0.3 0.213359587429405
0.31 0.220363841468831
0.32 0.227368181799166
0.33 0.234391320937291
0.34 0.24141751345349
0.35 0.248455404602702
0.36 0.255492246379198
0.37 0.262548290234055
0.38 0.269608871062211
0.39 0.276685738688214
0.4 0.283771258552828
0.41 0.290862219932611
0.42 0.297975209765946
0.43 0.305099152502415
0.44 0.312240352709686
0.45 0.319402704955107
0.46 0.326568156253983
0.47 0.333759721283672
0.48 0.340966450515614
0.49 0.348190247635895
0.5 0.355437748134476
0.51 0.362706716027846
0.52 0.369990971824002
0.53 0.37729718288365
0.54 0.384635215911941
0.55 0.391998021473886
0.56 0.39938560099669
0.57 0.406809800799778
0.58 0.414256972041698
0.59 0.421736379598337
0.6 0.429242020447809
0.61 0.436784759554541
0.62 0.444363968280051
0.63 0.451983060192451
0.64 0.459645222465216
0.65 0.467345938357545
0.66 0.47508227725332
0.67 0.482875337967339
0.68 0.490719732244281
0.69 0.498618983315868
0.7 0.506571287161701
0.71 0.514586481547206
0.72 0.522669614049061
0.73 0.530816819351841
0.74 0.539041087863616
0.75 0.547341387513478
0.76 0.555729550219261
0.77 0.564213416777772
0.78 0.572791041276544
0.79 0.581470665588143
0.8 0.590277298715218
0.81 0.599212789735777
0.82 0.608278552087828
0.83 0.617511570682848
0.84 0.626920592073227
0.85 0.636517526938344
0.86 0.646322278547061
0.87 0.656376490345393
0.88 0.666707997417517
0.89 0.677352076673676
0.9 0.688378962736464
0.91 0.699843478451467
0.92 0.71181649232978
0.93 0.724426742365873
0.94 0.737832802059005
0.95 0.752271881543633
0.96 0.768134073570165
0.97 0.786041833558503
0.98 0.807365541142568
0.99 0.835896662493282
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/active-nerfacto/empirical_coverage_absolute_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.0288264694768005, ymax=0.605355859012811,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.00731938765617662
0.02 0.0146063268016855
0.03 0.0218737983218439
0.04 0.0291327691340594
0.05 0.0363953374018731
0.06 0.0436943935549911
0.07 0.0509919236543291
0.08 0.0582882272881528
0.09 0.0655864656714469
0.1 0.0728832730123862
0.11 0.0801741190292463
0.12 0.0874623199702897
0.13 0.0947447461506176
0.14 0.10202776781105
0.15 0.109304457698525
0.16 0.116570691922711
0.17 0.123838150976083
0.18 0.131099305963649
0.19 0.138357833976402
0.2 0.145604668880189
0.21 0.152852509604675
0.22 0.160090833305449
0.23 0.167315534221771
0.24 0.174535246508397
0.25 0.181750054189244
0.26 0.1889492327323
0.27 0.196145458729025
0.28 0.203325866743475
0.29 0.210495993862371
0.3 0.217657168707886
0.31 0.224805770025651
0.32 0.231942086115929
0.33 0.239060168177529
0.34 0.246165425949685
0.35 0.253261072937473
0.36 0.260342271896023
0.37 0.267407296725599
0.38 0.274455159359251
0.39 0.281484667785313
0.4 0.288497623789415
0.41 0.29549949795286
0.42 0.302476650378048
0.43 0.309433101366214
0.44 0.316371134124097
0.45 0.323285021058609
0.46 0.330173242148172
0.47 0.337039456505454
0.48 0.343879200832242
0.49 0.350701113119675
0.5 0.357496168956067
0.51 0.364261554825885
0.52 0.37099980866025
0.53 0.37770235853545
0.54 0.384375630896497
0.55 0.391019495302635
0.56 0.397625859586308
0.57 0.404187606225803
0.58 0.410717151720159
0.59 0.417205209031849
0.6 0.423648657540082
0.61 0.430053559669361
0.62 0.436411615401516
0.63 0.442722142589364
0.64 0.448975810309916
0.65 0.455189265525246
0.66 0.461338312907139
0.67 0.467426896092882
0.68 0.473451628468312
0.69 0.479402117053263
0.7 0.485285990629626
0.71 0.491092173727494
0.72 0.49681632659047
0.73 0.502454417898585
0.74 0.507998395678025
0.75 0.513436137300795
0.76 0.518769385752771
0.77 0.523987677301086
0.78 0.52907983133315
0.79 0.534034287857818
0.8 0.538845821567636
0.81 0.543497691032538
0.82 0.547972483502313
0.83 0.552254360881553
0.84 0.556317330509845
0.85 0.560137584023758
0.86 0.563694086821151
0.87 0.566936237150815
0.88 0.569824887266141
0.89 0.57230763358198
0.9 0.574322231192277
0.91 0.575759870187215
0.92 0.576529389536011
0.93 0.576455541576852
0.94 0.5752969479815
0.95 0.572711178473373
0.96 0.568136456162382
0.97 0.560571000696778
0.98 0.54782523127922
0.99 0.523526621746011
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.00684283952788329
0.02 0.0122947628409302
0.03 0.0176604580422659
0.04 0.0229923461890525
0.05 0.0283000402410834
0.06 0.0335884208978852
0.07 0.0388677683099745
0.08 0.0441464570154806
0.09 0.0494112089261732
0.1 0.0546758841602339
0.11 0.0599280923639197
0.12 0.0651699068348094
0.13 0.0704145304918714
0.14 0.0756890343033893
0.15 0.0809656320114899
0.16 0.0862329016039417
0.17 0.0914933356829266
0.18 0.0967375074515438
0.19 0.101977263613309
0.2 0.107204545439368
0.21 0.112422837382248
0.22 0.117632501288483
0.23 0.122826637440767
0.24 0.128020992222551
0.25 0.133203849140921
0.26 0.138377454544435
0.27 0.143536397642948
0.28 0.148681179395351
0.29 0.153818332747483
0.3 0.158942800300305
0.31 0.164051606904446
0.32 0.169141550624664
0.33 0.174216639585114
0.34 0.179286607264787
0.35 0.184330098814403
0.36 0.189349118309018
0.37 0.194357861944871
0.38 0.199344899095463
0.39 0.204316695647852
0.4 0.209268381028481
0.41 0.214199497603399
0.42 0.219103150740352
0.43 0.223993371656708
0.44 0.228856406182219
0.45 0.233689771167073
0.46 0.238501986909758
0.47 0.243284785164783
0.48 0.248036678218456
0.49 0.252758468609817
0.5 0.257454288097188
0.51 0.262116308368008
0.52 0.266795151131156
0.53 0.271462800227396
0.54 0.276088793466875
0.55 0.28067777020595
0.56 0.285225693760206
0.57 0.289729213798064
0.58 0.294196044441181
0.59 0.298619334726674
0.6 0.302983575548946
0.61 0.307297832887054
0.62 0.311563636027501
0.63 0.315763788664918
0.64 0.319915165577811
0.65 0.324000877853538
0.66 0.328015170323324
0.67 0.331964138195993
0.68 0.335838776429032
0.69 0.339634428517774
0.7 0.343354466092856
0.71 0.346988409038683
0.72 0.350523001223841
0.73 0.353961537791371
0.74 0.357290596782556
0.75 0.360501753441229
0.76 0.363592974146126
0.77 0.366558687180982
0.78 0.369379379684834
0.79 0.372048261263764
0.8 0.374561959349723
0.81 0.376886996094373
0.82 0.379014716835042
0.83 0.380916747994142
0.84 0.382593192466752
0.85 0.383994222544872
0.86 0.385099784632853
0.87 0.385872077274478
0.88 0.386263068621864
0.89 0.386216473132102
0.9 0.385650673051444
0.91 0.384504362233037
0.92 0.382630383528553
0.93 0.379881193177025
0.94 0.37600240026551
0.95 0.370660807268967
0.96 0.363320738049979
0.97 0.352990845411921
0.98 0.337604948509828
0.99 0.311294450765134
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.00498767439047959
0.02 0.00913805803594501
0.03 0.0131537226438307
0.04 0.0171025039223755
0.05 0.0210142309095122
0.06 0.024897894848354
0.07 0.0287692457596816
0.08 0.0326325641099488
0.09 0.0364775824633071
0.1 0.0403129060652419
0.11 0.0441417513442592
0.12 0.0479544895583498
0.13 0.0517604016650358
0.14 0.0555548281835151
0.15 0.0593433994223732
0.16 0.0631261939114167
0.17 0.066917187096216
0.18 0.0707435387214789
0.19 0.0745676260781716
0.2 0.0783976450822769
0.21 0.0822223711502795
0.22 0.0860295838477896
0.23 0.0898246643539966
0.24 0.0936085201358109
0.25 0.0974231265908668
0.26 0.101225450881065
0.27 0.105017391593703
0.28 0.108804911043458
0.29 0.112571811872953
0.3 0.116343755142475
0.31 0.120098906463608
0.32 0.123846297826049
0.33 0.127583045705985
0.34 0.131307415216289
0.35 0.135013122306411
0.36 0.138705891504378
0.37 0.142385680217211
0.38 0.146052762205764
0.39 0.149693952914246
0.4 0.153330075864569
0.41 0.156937819465317
0.42 0.160525261450495
0.43 0.164092085126634
0.44 0.167650636937772
0.45 0.171189932898984
0.46 0.174698470938507
0.47 0.178189043116962
0.48 0.18165532548914
0.49 0.185096059714772
0.5 0.188507070960563
0.51 0.191897208959649
0.52 0.195257303503513
0.53 0.198588363791199
0.54 0.201923988615737
0.55 0.205254232722724
0.56 0.208554558670353
0.57 0.211814920042784
0.58 0.215034638332024
0.59 0.218209096493582
0.6 0.221345991413836
0.61 0.224440745638323
0.62 0.227490515991634
0.63 0.230481759071929
0.64 0.233420506301211
0.65 0.236309242768259
0.66 0.239137380538446
0.67 0.241910431880223
0.68 0.244617364501097
0.69 0.247261293578218
0.7 0.24983319697384
0.71 0.252326329899453
0.72 0.254731953727924
0.73 0.257051541065721
0.74 0.259268947695002
0.75 0.261397375106774
0.76 0.263423986269337
0.77 0.265334562719401
0.78 0.267119557176469
0.79 0.268769683104199
0.8 0.270274478367931
0.81 0.271619857141328
0.82 0.27280608502827
0.83 0.27379438845165
0.84 0.27456892959443
0.85 0.275105365436356
0.86 0.275385564493788
0.87 0.275378507951544
0.88 0.275034734791484
0.89 0.274295867247144
0.9 0.273133919268818
0.91 0.271446288122469
0.92 0.269144882470288
0.93 0.266063907579596
0.94 0.262036785837552
0.95 0.256764872235519
0.96 0.249782011489356
0.97 0.24027482868684
0.98 0.226586956524066
0.99 0.204045114953568
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.00588921807519952
0.02 0.00905457881239094
0.03 0.0120301654039883
0.04 0.014925819993335
0.05 0.0178030639181893
0.06 0.0207286215260044
0.07 0.0236431930645368
0.08 0.0265496064023712
0.09 0.0294478388502473
0.1 0.0323327897608699
0.11 0.0352011185788958
0.12 0.038063131486279
0.13 0.0409448237251436
0.14 0.043842802971584
0.15 0.0467575588424137
0.16 0.0496716133153715
0.17 0.052583328278912
0.18 0.0554916678050277
0.19 0.0584015723143791
0.2 0.0613009054117698
0.21 0.0641868942646392
0.22 0.0670697223041719
0.23 0.0699373961045746
0.24 0.072804638011656
0.25 0.0756641507855999
0.26 0.0785228512915176
0.27 0.0813849204535395
0.28 0.0842370557273192
0.29 0.0870883243710247
0.3 0.0899359791734988
0.31 0.0927961279438047
0.32 0.0956541680327102
0.33 0.0984945594256805
0.34 0.101327833710444
0.35 0.104147386733998
0.36 0.106998347642203
0.37 0.109832790050496
0.38 0.112661898856233
0.39 0.115472731461729
0.4 0.118272122546837
0.41 0.121070809843925
0.42 0.123849974673671
0.43 0.126637435471125
0.44 0.129415526612075
0.45 0.13217631937659
0.46 0.134937963570911
0.47 0.137674466702184
0.48 0.140394523368424
0.49 0.143099324412262
0.5 0.145780514589345
0.51 0.148446545366287
0.52 0.151097489352716
0.53 0.153726155458049
0.54 0.156323938118674
0.55 0.158897287622603
0.56 0.161446512590716
0.57 0.163959083759834
0.58 0.166448654161246
0.59 0.168906361143611
0.6 0.171338425600439
0.61 0.173734112452313
0.62 0.176093463760258
0.63 0.178412500327896
0.64 0.180689865941392
0.65 0.182928895806952
0.66 0.185132294289388
0.67 0.187279461164741
0.68 0.189375763739138
0.69 0.191417561465366
0.7 0.193428712838299
0.71 0.195413518452794
0.72 0.197330385950939
0.73 0.199183180648159
0.74 0.200958912136384
0.75 0.202658612486522
0.76 0.204270449780739
0.77 0.205786583222228
0.78 0.207208958723456
0.79 0.208529334411858
0.8 0.209722701284782
0.81 0.210787210264223
0.82 0.211721447912172
0.83 0.212488429317152
0.84 0.213079407926773
0.85 0.213482473061656
0.86 0.213677721452939
0.87 0.213623509654607
0.88 0.213292002582483
0.89 0.212647923326325
0.9 0.211621037263536
0.91 0.210156521548533
0.92 0.20818350767022
0.93 0.205573257634127
0.94 0.202167197940995
0.95 0.197728118456366
0.96 0.191865926429835
0.97 0.183958166441497
0.98 0.172634458857432
0.99 0.154103337506718
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/active-nerfacto/empirical_coverage_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.60536105694147, ymax=0.0289356259786452,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 -0.00724163698162931
0.02 -0.0145196728868776
0.03 -0.0218056427137712
0.04 -0.0290955221358109
0.05 -0.0363953374018731
0.06 -0.0436943935549911
0.07 -0.0509919236543291
0.08 -0.0582882272881528
0.09 -0.0655864656714469
0.1 -0.0728832730123862
0.11 -0.0801741190292463
0.12 -0.0874623199702897
0.13 -0.0947447461506176
0.14 -0.10202776781105
0.15 -0.109304457698525
0.16 -0.116570691922711
0.17 -0.123838150976083
0.18 -0.131099305963649
0.19 -0.138357833976402
0.2 -0.145604668880189
0.21 -0.152852509604675
0.22 -0.160090833305449
0.23 -0.167315534221771
0.24 -0.174535246508397
0.25 -0.181750054189244
0.26 -0.1889492327323
0.27 -0.196145458729025
0.28 -0.203325866743475
0.29 -0.210495993862371
0.3 -0.217657168707886
0.31 -0.224805770025651
0.32 -0.231942086115929
0.33 -0.239060168177529
0.34 -0.246165425949685
0.35 -0.253261072937473
0.36 -0.260342271896023
0.37 -0.267407296725599
0.38 -0.274455159359251
0.39 -0.281484667785313
0.4 -0.288497623789415
0.41 -0.29549949795286
0.42 -0.302476650378048
0.43 -0.309433101366214
0.44 -0.316371134124097
0.45 -0.323285021058609
0.46 -0.330173242148172
0.47 -0.337039456505454
0.48 -0.343879200832242
0.49 -0.350701113119675
0.5 -0.357496168956067
0.51 -0.364261554825885
0.52 -0.37099980866025
0.53 -0.37770235853545
0.54 -0.384375630896497
0.55 -0.391019495302635
0.56 -0.397625859586308
0.57 -0.404187606225803
0.58 -0.410717151720159
0.59 -0.417205209031849
0.6 -0.423648657540082
0.61 -0.430053559669361
0.62 -0.436411615401516
0.63 -0.442722142589364
0.64 -0.448975810309916
0.65 -0.455189265525246
0.66 -0.461338312907139
0.67 -0.467426896092882
0.68 -0.473451628468312
0.69 -0.479402117053263
0.7 -0.485285990629626
0.71 -0.491092173727494
0.72 -0.49681632659047
0.73 -0.502454417898585
0.74 -0.507998395678025
0.75 -0.513436137300795
0.76 -0.518769385752771
0.77 -0.523987677301086
0.78 -0.52907983133315
0.79 -0.534034287857818
0.8 -0.538845821567636
0.81 -0.543497691032538
0.82 -0.547972483502313
0.83 -0.552254360881553
0.84 -0.556317330509845
0.85 -0.560137584023758
0.86 -0.563694086821151
0.87 -0.566936237150815
0.88 -0.569824887266141
0.89 -0.57230763358198
0.9 -0.574322231192277
0.91 -0.575759870187215
0.92 -0.576529389536011
0.93 -0.576455541576852
0.94 -0.5752969479815
0.95 -0.572711178473373
0.96 -0.568136456162382
0.97 -0.560571000696778
0.98 -0.54782523127922
0.99 -0.523526621746011
};
\addplot [semithick, darkorange25512714]
table {%
0.01 -0.00380926235932821
0.02 -0.00897478537354913
0.03 -0.014227753292041
0.04 -0.0195251552092865
0.05 -0.0248403494082969
0.06 -0.0301627686522422
0.07 -0.0354907562403556
0.08 -0.0408325484460799
0.09 -0.0461695670348625
0.1 -0.0515165268520386
0.11 -0.0568542206758282
0.12 -0.0621892635892757
0.13 -0.0675218971606363
0.14 -0.0728553773133737
0.15 -0.0781929163971801
0.16 -0.0835230044132053
0.17 -0.0888489761212682
0.18 -0.094159762307584
0.19 -0.0994683912102637
0.2 -0.104765400504391
0.21 -0.110055225735944
0.22 -0.115336950850564
0.23 -0.120604321366152
0.24 -0.125871566944441
0.25 -0.131129028303464
0.26 -0.136377095693105
0.27 -0.141611883424612
0.28 -0.146832212331441
0.29 -0.152045470086584
0.3 -0.157246930288284
0.31 -0.162433047969065
0.32 -0.167600889343382
0.33 -0.172753767022117
0.34 -0.177902428425298
0.35 -0.18302473939359
0.36 -0.188122603445917
0.37 -0.193210434650142
0.38 -0.198276379206029
0.39 -0.203327606893588
0.4 -0.208358857484234
0.41 -0.213369979202263
0.42 -0.2183536668112
0.43 -0.223324014375998
0.44 -0.228267322194315
0.45 -0.233181567998629
0.46 -0.238074509536732
0.47 -0.2429370154563
0.48 -0.247768662262745
0.49 -0.252570491315929
0.5 -0.257346881574674
0.51 -0.262087763162562
0.52 -0.266795151131156
0.53 -0.271462800227396
0.54 -0.276088793466875
0.55 -0.28067777020595
0.56 -0.285225693760206
0.57 -0.289729213798064
0.58 -0.294196044441181
0.59 -0.298619334726674
0.6 -0.302983575548946
0.61 -0.307297832887054
0.62 -0.311563636027501
0.63 -0.315763788664918
0.64 -0.319915165577811
0.65 -0.324000877853538
0.66 -0.328015170323324
0.67 -0.331964138195993
0.68 -0.335838776429032
0.69 -0.339634428517774
0.7 -0.343354466092856
0.71 -0.346988409038683
0.72 -0.350523001223841
0.73 -0.353961537791371
0.74 -0.357290596782556
0.75 -0.360501753441229
0.76 -0.363592974146126
0.77 -0.366558687180982
0.78 -0.369379379684834
0.79 -0.372048261263764
0.8 -0.374561959349723
0.81 -0.376886996094373
0.82 -0.379014716835042
0.83 -0.380916747994142
0.84 -0.382593192466752
0.85 -0.383994222544872
0.86 -0.385099784632853
0.87 -0.385872077274478
0.88 -0.386263068621864
0.89 -0.386216473132102
0.9 -0.385650673051444
0.91 -0.384504362233037
0.92 -0.382630383528553
0.93 -0.379881193177025
0.94 -0.37600240026551
0.95 -0.370660807268967
0.96 -0.363320738049979
0.97 -0.352990845411921
0.98 -0.337604948509828
0.99 -0.311294450765134
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 -0.00275503136831453
0.02 -0.00636746130700929
0.03 -0.0101177505633088
0.04 -0.0139182331611702
0.05 -0.0177469349692516
0.06 -0.0215964523906977
0.07 -0.0254656713443536
0.08 -0.029348603001308
0.09 -0.0332379002434888
0.1 -0.0371353723975393
0.11 -0.0410429286622005
0.12 -0.0449488328064511
0.13 -0.0488588672722564
0.14 -0.0527664494427179
0.15 -0.0566737739584491
0.16 -0.0605838270975157
0.17 -0.0644884255878177
0.18 -0.0683943858298297
0.19 -0.0722915526933763
0.2 -0.0761970519820769
0.21 -0.0800981130618288
0.22 -0.0839836802734816
0.23 -0.0878600230420903
0.24 -0.0917239052513979
0.25 -0.0955961808179082
0.26 -0.0994578711043517
0.27 -0.103308955751769
0.28 -0.107156670785889
0.29 -0.110985786702143
0.3 -0.114819345911449
0.31 -0.118636938570646
0.32 -0.122446825739058
0.33 -0.126248608467393
0.34 -0.130036554762128
0.35 -0.133806848387877
0.36 -0.137564660813921
0.37 -0.141309735765493
0.38 -0.145043235249312
0.39 -0.148750034814134
0.4 -0.152452290350672
0.41 -0.156125839730194
0.42 -0.159779200619798
0.43 -0.163412655472991
0.44 -0.16703727702276
0.45 -0.170642512837592
0.46 -0.174216596885872
0.47 -0.177772576808396
0.48 -0.181304660769508
0.49 -0.184809977340929
0.5 -0.188286245496585
0.51 -0.191741552418918
0.52 -0.195167205541055
0.53 -0.198563028337606
0.54 -0.201923988615737
0.55 -0.205254232722724
0.56 -0.208554558670353
0.57 -0.211814920042784
0.58 -0.215034638332024
0.59 -0.218209096493582
0.6 -0.221345991413836
0.61 -0.224440745638323
0.62 -0.227490515991634
0.63 -0.230481759071929
0.64 -0.233420506301211
0.65 -0.236309242768259
0.66 -0.239137380538446
0.67 -0.241910431880223
0.68 -0.244617364501097
0.69 -0.247261293578218
0.7 -0.24983319697384
0.71 -0.252326329899453
0.72 -0.254731953727924
0.73 -0.257051541065721
0.74 -0.259268947695002
0.75 -0.261397375106774
0.76 -0.263423986269337
0.77 -0.265334562719401
0.78 -0.267119557176469
0.79 -0.268769683104199
0.8 -0.270274478367931
0.81 -0.271619857141328
0.82 -0.27280608502827
0.83 -0.27379438845165
0.84 -0.27456892959443
0.85 -0.275105365436356
0.86 -0.275385564493788
0.87 -0.275378507951544
0.88 -0.275034734791484
0.89 -0.274295867247144
0.9 -0.273133919268818
0.91 -0.271446288122469
0.92 -0.269144882470288
0.93 -0.266063907579596
0.94 -0.262036785837552
0.95 -0.256764872235519
0.96 -0.249782011489356
0.97 -0.24027482868684
0.98 -0.226586956524066
0.99 -0.204045114953568
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.000103958573185406
0.02 -0.0025335722688508
0.03 -0.00535121768174938
0.04 -0.00824331131337327
0.05 -0.0111756100443886
0.06 -0.014123638221314
0.07 -0.0171002158208001
0.08 -0.0200959318691609
0.09 -0.023101617755666
0.1 -0.0261126532818683
0.11 -0.0291323653582433
0.12 -0.0321541932053524
0.13 -0.0351796541578872
0.14 -0.0382119429715223
0.15 -0.0412437742897476
0.16 -0.044282456868003
0.17 -0.0473227901764553
0.18 -0.0503626695793046
0.19 -0.053408531582362
0.2 -0.0564523403012039
0.21 -0.059486603519099
0.22 -0.0625216856976902
0.23 -0.0655465145501518
0.24 -0.068571211927682
0.25 -0.071594522046231
0.26 -0.0746141401433105
0.27 -0.0776273905653514
0.28 -0.0806326530237764
0.29 -0.0836410272788563
0.3 -0.0866404125705949
0.31 -0.0896361585311693
0.32 -0.0926318182008342
0.33 -0.0956086790627091
0.34 -0.0985824865465096
0.35 -0.101544595397298
0.36 -0.104507753620802
0.37 -0.107451709765945
0.38 -0.110391128937789
0.39 -0.113314261311786
0.4 -0.116228741447172
0.41 -0.119137780067389
0.42 -0.122024790234054
0.43 -0.124900847497585
0.44 -0.127759647290314
0.45 -0.130597295044893
0.46 -0.133431843746016
0.47 -0.136240278716328
0.48 -0.139033549484386
0.49 -0.141809752364105
0.5 -0.144562251865524
0.51 -0.147293283972154
0.52 -0.150009028175998
0.53 -0.15270281711635
0.54 -0.155364784088059
0.55 -0.158001978526114
0.56 -0.16061439900331
0.57 -0.163190199200222
0.58 -0.165743027958302
0.59 -0.168263620401663
0.6 -0.170757979552191
0.61 -0.173215240445459
0.62 -0.175636031719949
0.63 -0.178016939807549
0.64 -0.180354777534783
0.65 -0.182654061642455
0.66 -0.18491772274668
0.67 -0.187124662032661
0.68 -0.189280267755719
0.69 -0.191381016684132
0.7 -0.193428712838299
0.71 -0.195413518452794
0.72 -0.197330385950939
0.73 -0.199183180648159
0.74 -0.200958912136384
0.75 -0.202658612486522
0.76 -0.204270449780739
0.77 -0.205786583222228
0.78 -0.207208958723456
0.79 -0.208529334411858
0.8 -0.209722701284782
0.81 -0.210787210264223
0.82 -0.211721447912172
0.83 -0.212488429317152
0.84 -0.213079407926773
0.85 -0.213482473061656
0.86 -0.213677721452939
0.87 -0.213623509654607
0.88 -0.213292002582483
0.89 -0.212647923326325
0.9 -0.211621037263536
0.91 -0.210156521548533
0.92 -0.20818350767022
0.93 -0.205573257634127
0.94 -0.202167197940995
0.95 -0.197728118456366
0.96 -0.191865926429835
0.97 -0.183958166441497
0.98 -0.172634458857432
0.99 -0.154103337506718
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/active-nerfacto/empirical_coverage_negative_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.0288264694768005, ymax=0.605355859012811,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.00728051231890296
0.02 0.0145629998442815
0.03 0.0218397205178076
0.04 0.0291141456349352
0.05 0.0363953374018731
0.06 0.0436943935549911
0.07 0.0509919236543291
0.08 0.0582882272881528
0.09 0.0655864656714469
0.1 0.0728832730123862
0.11 0.0801741190292463
0.12 0.0874623199702897
0.13 0.0947447461506176
0.14 0.10202776781105
0.15 0.109304457698525
0.16 0.116570691922711
0.17 0.123838150976083
0.18 0.131099305963649
0.19 0.138357833976402
0.2 0.145604668880189
0.21 0.152852509604675
0.22 0.160090833305449
0.23 0.167315534221771
0.24 0.174535246508397
0.25 0.181750054189244
0.26 0.1889492327323
0.27 0.196145458729025
0.28 0.203325866743475
0.29 0.210495993862371
0.3 0.217657168707886
0.31 0.224805770025651
0.32 0.231942086115929
0.33 0.239060168177529
0.34 0.246165425949685
0.35 0.253261072937473
0.36 0.260342271896023
0.37 0.267407296725599
0.38 0.274455159359251
0.39 0.281484667785313
0.4 0.288497623789415
0.41 0.29549949795286
0.42 0.302476650378048
0.43 0.309433101366214
0.44 0.316371134124097
0.45 0.323285021058609
0.46 0.330173242148172
0.47 0.337039456505454
0.48 0.343879200832242
0.49 0.350701113119675
0.5 0.357496168956067
0.51 0.364261554825885
0.52 0.37099980866025
0.53 0.37770235853545
0.54 0.384375630896497
0.55 0.391019495302635
0.56 0.397625859586308
0.57 0.404187606225803
0.58 0.410717151720159
0.59 0.417205209031849
0.6 0.423648657540082
0.61 0.430053559669361
0.62 0.436411615401516
0.63 0.442722142589364
0.64 0.448975810309916
0.65 0.455189265525246
0.66 0.461338312907139
0.67 0.467426896092882
0.68 0.473451628468312
0.69 0.479402117053263
0.7 0.485285990629626
0.71 0.491092173727494
0.72 0.49681632659047
0.73 0.502454417898585
0.74 0.507998395678025
0.75 0.513436137300795
0.76 0.518769385752771
0.77 0.523987677301086
0.78 0.52907983133315
0.79 0.534034287857818
0.8 0.538845821567636
0.81 0.543497691032538
0.82 0.547972483502313
0.83 0.552254360881553
0.84 0.556317330509845
0.85 0.560137584023758
0.86 0.563694086821151
0.87 0.566936237150815
0.88 0.569824887266141
0.89 0.57230763358198
0.9 0.574322231192277
0.91 0.575759870187215
0.92 0.576529389536011
0.93 0.576455541576852
0.94 0.5752969479815
0.95 0.572711178473373
0.96 0.568136456162382
0.97 0.560571000696778
0.98 0.54782523127922
0.99 0.523526621746011
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.00532605094360575
0.02 0.0106347741072397
0.03 0.0159441056671534
0.04 0.0212587506991695
0.05 0.0265701948246901
0.06 0.0318755947750637
0.07 0.0371792622751651
0.08 0.0424895027307803
0.09 0.0477903879805179
0.1 0.0530962055061363
0.11 0.058391156519874
0.12 0.0636795852120425
0.13 0.0689682138262538
0.14 0.0742722058083815
0.15 0.079579274204335
0.16 0.0848779530085735
0.17 0.0901711559020974
0.18 0.0954486348795639
0.19 0.100722827411786
0.2 0.105984972971879
0.21 0.111239031559096
0.22 0.116484726069523
0.23 0.121715479403459
0.24 0.126946279583496
0.25 0.132166438722193
0.26 0.13737727511877
0.27 0.14257414053378
0.28 0.147756695863396
0.29 0.152931901417034
0.3 0.158094865294294
0.31 0.163242327436756
0.32 0.168371219984023
0.33 0.173485203303615
0.34 0.178594517845042
0.35 0.183677419103996
0.36 0.188735860877468
0.37 0.193784148297507
0.38 0.198810639150746
0.39 0.20382215127072
0.4 0.208813619256357
0.41 0.213784738402831
0.42 0.218728408775776
0.43 0.223658693016353
0.44 0.228561864188267
0.45 0.233435669582851
0.46 0.238288248223245
0.47 0.243110900310541
0.48 0.247902670240601
0.49 0.252664479962873
0.5 0.257400584835931
0.51 0.262102035765285
0.52 0.266795151131156
0.53 0.271462800227396
0.54 0.276088793466875
0.55 0.28067777020595
0.56 0.285225693760206
0.57 0.289729213798064
0.58 0.294196044441181
0.59 0.298619334726674
0.6 0.302983575548946
0.61 0.307297832887054
0.62 0.311563636027501
0.63 0.315763788664918
0.64 0.319915165577811
0.65 0.324000877853538
0.66 0.328015170323324
0.67 0.331964138195993
0.68 0.335838776429032
0.69 0.339634428517774
0.7 0.343354466092856
0.71 0.346988409038683
0.72 0.350523001223841
0.73 0.353961537791371
0.74 0.357290596782556
0.75 0.360501753441229
0.76 0.363592974146126
0.77 0.366558687180982
0.78 0.369379379684834
0.79 0.372048261263764
0.8 0.374561959349723
0.81 0.376886996094373
0.82 0.379014716835042
0.83 0.380916747994142
0.84 0.382593192466752
0.85 0.383994222544872
0.86 0.385099784632853
0.87 0.385872077274478
0.88 0.386263068621864
0.89 0.386216473132102
0.9 0.385650673051444
0.91 0.384504362233037
0.92 0.382630383528553
0.93 0.379881193177025
0.94 0.37600240026551
0.95 0.370660807268967
0.96 0.363320738049979
0.97 0.352990845411921
0.98 0.337604948509828
0.99 0.311294450765134
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.00387135287939706
0.02 0.00775275967147715
0.03 0.0116357366035697
0.04 0.0155103685417729
0.05 0.0193805829393819
0.06 0.0232471736195258
0.07 0.0271174585520176
0.08 0.0309905835556284
0.09 0.0348577413533979
0.1 0.0387241392313906
0.11 0.0425923400032299
0.12 0.0464516611824004
0.13 0.0503096344686461
0.14 0.0541606388131165
0.15 0.0580085866904111
0.16 0.0618550105044662
0.17 0.0657028063420168
0.18 0.0695689622756543
0.19 0.0734295893857739
0.2 0.0772973485321769
0.21 0.0811602421060542
0.22 0.0850066320606356
0.23 0.0888423436980435
0.24 0.0926662126936044
0.25 0.0965096537043875
0.26 0.100341660992708
0.27 0.104163173672736
0.28 0.107980790914674
0.29 0.111778799287548
0.3 0.115581550526962
0.31 0.119367922517127
0.32 0.123146561782553
0.33 0.126915827086689
0.34 0.130671984989209
0.35 0.134409985347144
0.36 0.13813527615915
0.37 0.141847707991352
0.38 0.145547998727538
0.39 0.14922199386419
0.4 0.152891183107621
0.41 0.156531829597755
0.42 0.160152231035146
0.43 0.163752370299812
0.44 0.167343956980266
0.45 0.170916222868288
0.46 0.17445753391219
0.47 0.177980809962679
0.48 0.181479993129324
0.49 0.18495301852785
0.5 0.188396658228574
0.51 0.191819380689283
0.52 0.195212254522284
0.53 0.198575696064402
0.54 0.201923988615737
0.55 0.205254232722724
0.56 0.208554558670353
0.57 0.211814920042784
0.58 0.215034638332024
0.59 0.218209096493582
0.6 0.221345991413836
0.61 0.224440745638323
0.62 0.227490515991634
0.63 0.230481759071929
0.64 0.233420506301211
0.65 0.236309242768259
0.66 0.239137380538446
0.67 0.241910431880223
0.68 0.244617364501097
0.69 0.247261293578218
0.7 0.24983319697384
0.71 0.252326329899453
0.72 0.254731953727924
0.73 0.257051541065721
0.74 0.259268947695002
0.75 0.261397375106774
0.76 0.263423986269337
0.77 0.265334562719401
0.78 0.267119557176469
0.79 0.268769683104199
0.8 0.270274478367931
0.81 0.271619857141328
0.82 0.27280608502827
0.83 0.27379438845165
0.84 0.27456892959443
0.85 0.275105365436356
0.86 0.275385564493788
0.87 0.275378507951544
0.88 0.275034734791484
0.89 0.274295867247144
0.9 0.273133919268818
0.91 0.271446288122469
0.92 0.269144882470288
0.93 0.266063907579596
0.94 0.262036785837552
0.95 0.256764872235519
0.96 0.249782011489356
0.97 0.24027482868684
0.98 0.226586956524066
0.99 0.204045114953568
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.00289262975100706
0.02 0.00579407554062087
0.03 0.00869069154286885
0.04 0.0115845656533541
0.05 0.014489336981289
0.06 0.0174261298736592
0.07 0.0203717044426684
0.08 0.0233227691357661
0.09 0.0262747283029567
0.1 0.0292227215213691
0.11 0.0321667419685696
0.12 0.0351086623458157
0.13 0.0380622389415154
0.14 0.0410273729715531
0.15 0.0440006665660807
0.16 0.0469770350916873
0.17 0.0499530592276837
0.18 0.0529271686921662
0.19 0.0559050519483706
0.2 0.0588766228564868
0.21 0.0618367488918691
0.22 0.064795704000931
0.23 0.0677419553273632
0.24 0.070687924969669
0.25 0.0736293364159154
0.26 0.076568495717414
0.27 0.0795061555094455
0.28 0.0824348543755478
0.29 0.0853646758249405
0.3 0.0882881958720469
0.31 0.091216143237487
0.32 0.0941429931167722
0.33 0.0970516192441948
0.34 0.0999551601284766
0.35 0.102845991065648
0.36 0.105753050631502
0.37 0.108642249908221
0.38 0.111526513897011
0.39 0.114393496386757
0.4 0.117250431997004
0.41 0.120104294955657
0.42 0.122937382453863
0.43 0.125769141484355
0.44 0.128587586951194
0.45 0.131386807210741
0.46 0.134184903658464
0.47 0.136957372709256
0.48 0.139714036426405
0.49 0.142454538388184
0.5 0.145171383227435
0.51 0.147869914669221
0.52 0.150553258764357
0.53 0.1532144862872
0.54 0.155844361103367
0.55 0.158449633074358
0.56 0.161030455797013
0.57 0.163574641480028
0.58 0.166095841059774
0.59 0.168584990772637
0.6 0.171048202576315
0.61 0.173474676448886
0.62 0.175864747740103
0.63 0.178214720067723
0.64 0.180522321738088
0.65 0.182791478724703
0.66 0.185025008518034
0.67 0.187202061598701
0.68 0.189328015747429
0.69 0.191399289074749
0.7 0.193428712838299
0.71 0.195413518452794
0.72 0.197330385950939
0.73 0.199183180648159
0.74 0.200958912136384
0.75 0.202658612486522
0.76 0.204270449780739
0.77 0.205786583222228
0.78 0.207208958723456
0.79 0.208529334411858
0.8 0.209722701284782
0.81 0.210787210264223
0.82 0.211721447912172
0.83 0.212488429317152
0.84 0.213079407926773
0.85 0.213482473061656
0.86 0.213677721452939
0.87 0.213623509654607
0.88 0.213292002582483
0.89 0.212647923326325
0.9 0.211621037263536
0.91 0.210156521548533
0.92 0.20818350767022
0.93 0.205573257634127
0.94 0.202167197940995
0.95 0.197728118456366
0.96 0.191865926429835
0.97 0.183958166441497
0.98 0.172634458857432
0.99 0.154103337506718
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/active-splatfacto/avg_length.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.039, xmax=1.039,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.00824456220419365, ymax=0.183226249987058,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.01 0.000660313953105411
0.02 0.00132072956306621
0.03 0.00198135452688254
0.04 0.00264229075920316
0.05 0.00330364259492075
0.06 0.00396551660968048
0.07 0.00462801572714972
0.08 0.00529124879658745
0.09 0.00595532104043177
0.1 0.00662033973928085
0.11 0.00728641596685267
0.12 0.00795366113478373
0.13 0.00862218030792453
0.14 0.00929209318684738
0.15 0.00996351323480479
0.16 0.0106365532794044
0.17 0.0113113335656461
0.18 0.0119879755974521
0.19 0.0126666017641593
0.2 0.0133473357444577
0.21 0.0140303036229599
0.22 0.0147156400930408
0.23 0.0154034747825635
0.24 0.0160939454199012
0.25 0.0167871898084177
0.26 0.0174833563774156
0.27 0.0181825867768179
0.28 0.0188850369996247
0.29 0.0195908616501258
0.3 0.0203002165259792
0.31 0.0210132734378671
0.32 0.0217301999698301
0.33 0.0224511742796253
0.34 0.0231763809997927
0.35 0.0239060021316905
0.36 0.0246402400466625
0.37 0.0253792908134724
0.38 0.0261233668757751
0.39 0.0268727050407137
0.4 0.0276275089645004
0.41 0.0283880271532888
0.42 0.0291545142463316
0.43 0.0299272173402178
0.44 0.0307064131732441
0.45 0.0314923843758643
0.46 0.0322854288986277
0.47 0.0330858585983038
0.48 0.033894001001783
0.49 0.0347101939421554
0.5 0.0355348031846496
0.51 0.0363682172306682
0.52 0.037210837249049
0.53 0.0380630778686104
0.54 0.0389253980709247
0.55 0.0397982687525717
0.56 0.0406822136775353
0.57 0.0415777585344378
0.58 0.0424854831757655
0.59 0.0434060030991539
0.6 0.0443399561958405
0.61 0.0452880701965935
0.62 0.0462510776589547
0.63 0.0472297946272398
0.64 0.0482250808359592
0.65 0.0492378805492359
0.66 0.0502692238709019
0.67 0.0513202110400704
0.68 0.0523920019529749
0.69 0.0534859411808235
0.7 0.0546034369481776
0.71 0.0557460628912335
0.72 0.0569155212013376
0.73 0.0581137279629826
0.74 0.0593427801198301
0.75 0.0606049906497399
0.76 0.0619029875819417
0.77 0.0632396892010688
0.78 0.0646183943723291
0.79 0.0660428103584076
0.8 0.0675172452724975
0.81 0.0690465262601159
0.82 0.0706363112306274
0.83 0.07229317290733
0.84 0.0740247731749834
0.85 0.0758402536497591
0.86 0.0777505591518854
0.87 0.07976892656049
0.88 0.0819116716804314
0.89 0.0841991848582028
0.9 0.08665744625524
0.91 0.089320293411167
0.92 0.0922331247444934
0.93 0.0954586805450262
0.94 0.099087693674654
0.95 0.103258724498482
0.96 0.108199657764559
0.97 0.114329002555341
0.98 0.122561256607538
0.99 0.135704938929982
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.000458656531772317
0.02 0.000917384794208451
0.03 0.00137625736512072
0.04 0.0018353466143256
0.05 0.00229472468513378
0.06 0.00275446472540688
0.07 0.00321464015747947
0.08 0.00367532428335029
0.09 0.00413659187151329
0.1 0.00459851691257695
0.11 0.00506117664176689
0.12 0.00552464688857432
0.13 0.00598900444591272
0.14 0.00645432886154164
0.15 0.0069206989991021
0.16 0.0073881957167957
0.17 0.00785690162944656
0.18 0.0083269002325371
0.19 0.00879827623949625
0.2 0.00927111694190909
0.21 0.00974550995276566
0.22 0.0102215480103288
0.23 0.0106993211655215
0.24 0.0111789239469361
0.25 0.0116604555369219
0.26 0.0121440158293028
0.27 0.0126297045659949
0.28 0.0131176287963321
0.29 0.0136078967391846
0.3 0.0141006188618346
0.31 0.0145959107829092
0.32 0.0150938923682715
0.33 0.0155946833831358
0.34 0.0160984126649873
0.35 0.0166052124280101
0.36 0.0171152154625415
0.37 0.0176285649184312
0.38 0.0181454078006258
0.39 0.0186658963047543
0.4 0.0191901889249745
0.41 0.0197184469698194
0.42 0.0202508496783135
0.43 0.0207875750828807
0.44 0.0213288086135581
0.45 0.0218747477387733
0.46 0.0224256003524382
0.47 0.022981581685407
0.48 0.023542919266613
0.49 0.0241098517342674
0.5 0.0246826315355311
0.51 0.025261521984053
0.52 0.025846807399977
0.53 0.0264387769065676
0.54 0.0270377487082467
0.55 0.0276440538051844
0.56 0.0282580428074537
0.57 0.0288800939963505
0.58 0.0295106018144311
0.59 0.0301499941118312
0.6 0.0307987277557793
0.61 0.0314572882878602
0.62 0.0321261991045715
0.63 0.0328060157544732
0.64 0.0334973504687108
0.65 0.0342008508147437
0.66 0.0349172246387253
0.67 0.0356472364150347
0.68 0.0363917145552064
0.69 0.0371515677528506
0.7 0.0379277854401673
0.71 0.0387214560019218
0.72 0.0395337699869877
0.73 0.0403660478699519
0.74 0.0412197510399683
0.75 0.0420964897330378
0.76 0.0429980849734815
0.77 0.0439265626928133
0.78 0.0448842151753927
0.79 0.0458736316144093
0.8 0.0468977724920968
0.81 0.0479600191811982
0.82 0.0490642911691475
0.83 0.0502151474451263
0.84 0.0514179269479294
0.85 0.0526789696114283
0.86 0.0540058686877165
0.87 0.0554078383139575
0.88 0.0568961987898769
0.89 0.0584851202181148
0.9 0.0601926339981166
0.91 0.0620422734392335
0.92 0.0640655224023879
0.93 0.06630600882322
0.94 0.0688267458203192
0.95 0.0717239518985241
0.96 0.0751559646995481
0.97 0.0794134264288094
0.98 0.0851315900363177
0.99 0.0942612470549507
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.000620672638634514
0.02 0.00124144284908278
0.03 0.00186240817065905
0.04 0.00248366645742693
0.05 0.00310531581880104
0.06 0.00372745515460766
0.07 0.00435018337141169
0.08 0.00497360001106617
0.09 0.00559780603510544
0.1 0.00622290260582641
0.11 0.0068489924259386
0.12 0.00747617953877833
0.13 0.00810456712639489
0.14 0.00873426285484215
0.15 0.0093653749792531
0.16 0.00999801076065334
0.17 0.0106322824208894
0.18 0.0112683036636669
0.19 0.0119061894781592
0.2 0.0125460566546294
0.21 0.0131880250527303
0.22 0.0138322191863816
0.23 0.0144787615199628
0.24 0.0151277798249541
0.25 0.0157794096229612
0.26 0.016433782178281
0.27 0.0170910349380604
0.28 0.0177513151943154
0.29 0.0184147662682528
0.3 0.0190815377183682
0.31 0.0197517874202603
0.32 0.0204256764453576
0.33 0.0211033668308384
0.34 0.0217850334392099
0.35 0.0224708566195885
0.36 0.023161013550332
0.37 0.0238557000525182
0.38 0.0245551122034325
0.39 0.0252594571269893
0.4 0.025968952903011
0.41 0.0266838136193587
0.42 0.0274042838368765
0.43 0.0281306009549709
0.44 0.0288630206858914
0.45 0.0296018089969218
0.46 0.0303472448569776
0.47 0.03109962318938
0.48 0.0318592462420583
0.49 0.0326264436706254
0.5 0.0334015525640859
0.51 0.0341849315154903
0.52 0.0349769639866608
0.53 0.0357780407463834
0.54 0.0365885955473
0.55 0.037409070013737
0.56 0.0382399440363239
0.57 0.0390817311753344
0.58 0.0399349582662831
0.59 0.0408002121250626
0.6 0.0416781064891748
0.61 0.042569297809542
0.62 0.0434744908232995
0.63 0.0443944489201176
0.64 0.0453299934667065
0.65 0.0462819962802689
0.66 0.0472514262890277
0.67 0.0482393025111443
0.68 0.0492467652142978
0.69 0.0502750315549628
0.7 0.0513254386068462
0.71 0.0523994668619075
0.72 0.0534987238497092
0.73 0.0546249949578076
0.74 0.0557802604194045
0.75 0.0569667020901288
0.76 0.0581867754886933
0.77 0.0594432285539918
0.78 0.0607391645760577
0.79 0.0620780841455358
0.8 0.063463993568738
0.81 0.0649014692548261
0.82 0.066395815859358
0.83 0.0679532037435338
0.84 0.069580854459386
0.85 0.0712873505099477
0.86 0.0730829641379306
0.87 0.0749801648983643
0.88 0.0769942788490594
0.89 0.07914446957927
0.9 0.0814551467297233
0.91 0.083958157197891
0.92 0.0866961009921882
0.93 0.0897280195848421
0.94 0.0931391841760026
0.95 0.09705980494842
0.96 0.101704140842572
0.97 0.107465515725337
0.98 0.115203570030773
0.99 0.127558200178911
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.000849194096636526
0.02 0.00169852177861722
0.03 0.00254811635375967
0.04 0.0033981118344057
0.05 0.00424864220124461
0.06 0.00509984313435882
0.07 0.00595184956224249
0.08 0.00680479794637866
0.09 0.00765882634182555
0.1 0.00851407353279509
0.11 0.00937067950464643
0.12 0.0102287858808002
0.13 0.0110885357757393
0.14 0.0119500756866487
0.15 0.0128135520354891
0.16 0.0136791138623606
0.17 0.014546915124244
0.18 0.0154171094430368
0.19 0.0162898533609218
0.2 0.0171653080963676
0.21 0.0180436390428096
0.22 0.018925014872919
0.23 0.0198096034049967
0.24 0.020697580703511
0.25 0.0215891284984916
0.26 0.0224844316209461
0.27 0.0233836740720423
0.28 0.0242870585868508
0.29 0.0251947818249158
0.3 0.0261070463876477
0.31 0.0270240727215036
0.32 0.0279460766033689
0.33 0.0288732806158565
0.34 0.0298059264703505
0.35 0.0307442578065691
0.36 0.0316885200322836
0.37 0.0326389791135767
0.38 0.0335959008852507
0.39 0.0345595783902087
0.4 0.0355302962498156
0.41 0.0365083569819697
0.42 0.0374940930783921
0.43 0.0384878293692947
0.44 0.0394899125486162
0.45 0.0405007102278895
0.46 0.041520600986583
0.47 0.0425499943884835
0.48 0.0435892988603991
0.49 0.0446389653902572
0.5 0.0456994544645112
0.51 0.0467712654463117
0.52 0.0478549068565095
0.53 0.0489509323898196
0.54 0.0500599130915156
0.55 0.0511824784021674
0.56 0.0523192677827669
0.57 0.0534709837889273
0.58 0.0546383571499164
0.59 0.0558221836095935
0.6 0.0570233027757366
0.61 0.058242616824446
0.62 0.0594810903386497
0.63 0.0607397619880184
0.64 0.0620197534754643
0.65 0.0633222694373341
0.66 0.0646486221753876
0.67 0.0660002246226692
0.68 0.067378616346471
0.69 0.0687854736304929
0.7 0.0702226271667204
0.71 0.0716920945667095
0.72 0.0731960754472259
0.73 0.0747370275116784
0.74 0.0763176353969026
0.75 0.0779409049436504
0.76 0.0796101964159119
0.77 0.0813292539620724
0.78 0.0831023333579082
0.79 0.0849342134819582
0.8 0.0868303935839904
0.81 0.0887971236071825
0.82 0.0908416706630524
0.83 0.0929724622174117
0.84 0.095199383346273
0.85 0.0975341805171162
0.86 0.099990909573785
0.87 0.102586629844553
0.88 0.105342308004439
0.89 0.108284162488375
0.9 0.111445606586498
0.91 0.114870176317545
0.92 0.118616181125848
0.93 0.122764406943075
0.94 0.127431511519504
0.95 0.132795629172656
0.96 0.139149934532819
0.97 0.147032558305368
0.98 0.15761965026792
0.99 0.174523031251092
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/active-splatfacto/empirical_coverage.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.05, ymax=1.05,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 1
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.00447529570666702
0.02 0.00621095350061277
0.03 0.00792888900809367
0.04 0.00963309119799223
0.05 0.0113331238449067
0.06 0.0130288599885597
0.07 0.0147276287094341
0.08 0.0164318068138884
0.09 0.0181361717649604
0.1 0.0198372461556833
0.11 0.021534677322292
0.12 0.0232307197464735
0.13 0.0249403549531452
0.14 0.0266624816206249
0.15 0.0283727521425289
0.16 0.0300890232525836
0.17 0.0318036155816089
0.18 0.0335202637104484
0.19 0.0352375073951595
0.2 0.0369650116284194
0.21 0.0386966774462048
0.22 0.0404328123289666
0.23 0.0421737048833602
0.24 0.0439175154457823
0.25 0.0456810343489474
0.26 0.0474601380335736
0.27 0.0492597280606736
0.28 0.0511324780059971
0.29 0.0530488397086454
0.3 0.05498691058795
0.31 0.0569966585461954
0.32 0.0588910914953672
0.33 0.0607385518368243
0.34 0.0625650138660228
0.35 0.0643914154325276
0.36 0.0662209524867125
0.37 0.0680540901370149
0.38 0.0698974092397565
0.39 0.0717502384239161
0.4 0.0736129854937836
0.41 0.0754750790685951
0.42 0.0773440834496216
0.43 0.0792101889636971
0.44 0.0810731215951919
0.45 0.0829220760484493
0.46 0.084750930749289
0.47 0.0865591328405523
0.48 0.0883624648112228
0.49 0.0901630394339939
0.5 0.0919689448925114
0.51 0.0937766809856121
0.52 0.0955952464910513
0.53 0.0974201987903763
0.54 0.0992532528200005
0.55 0.101100715184047
0.56 0.102965476990532
0.57 0.104903458806929
0.58 0.106777574746874
0.59 0.108658600618664
0.6 0.110553675708297
0.61 0.112471905406434
0.62 0.114402439905378
0.63 0.116349586104985
0.64 0.118316630427427
0.65 0.120306994647815
0.66 0.12232306658877
0.67 0.124369810828312
0.68 0.126440237005944
0.69 0.128543590746329
0.7 0.130681425895282
0.71 0.132862853340114
0.72 0.135080809783621
0.73 0.137343044422223
0.74 0.139655843537178
0.75 0.142019085145002
0.76 0.144472249425025
0.77 0.146967556603698
0.78 0.149481822082942
0.79 0.152064268019432
0.8 0.154725306256388
0.81 0.157466174816135
0.82 0.160295102744719
0.83 0.163228317074571
0.84 0.166264447266518
0.85 0.169429048518893
0.86 0.172725242784286
0.87 0.176182561285175
0.88 0.179828700893928
0.89 0.183739674704228
0.9 0.187819827728897
0.91 0.192194610009022
0.92 0.196920665420438
0.93 0.202104946262604
0.94 0.207861039740094
0.95 0.214428196302149
0.96 0.222011497751127
0.97 0.231167807427753
0.98 0.243158498168539
0.99 0.261517461878748
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.0106000166589701
0.02 0.0134810733117778
0.03 0.0163537806372817
0.04 0.0192196788842284
0.05 0.0220895140051397
0.06 0.0249571203385873
0.07 0.0278198496941752
0.08 0.0306902559018429
0.09 0.0335563517584542
0.1 0.0364190550976199
0.11 0.0392836335163388
0.12 0.0421464709170888
0.13 0.0450091909746504
0.14 0.0478733678331745
0.15 0.0507365311550155
0.16 0.053596617976977
0.17 0.0564627198393551
0.18 0.0593305634470871
0.19 0.0622004784998503
0.2 0.0650672947916242
0.21 0.0679371172030388
0.22 0.0708106539838224
0.23 0.0736913649157465
0.24 0.0765728167900511
0.25 0.079451832467736
0.26 0.0823320984385802
0.27 0.0852192850815003
0.28 0.08810651734929
0.29 0.0910069437486867
0.3 0.0939416944406049
0.31 0.0969979403945762
0.32 0.0998730116825304
0.33 0.102747536945833
0.34 0.105622876184682
0.35 0.108507931286035
0.36 0.11139757978353
0.37 0.114292516181235
0.38 0.117194050146903
0.39 0.120101992177939
0.4 0.123018464835263
0.41 0.125952071650301
0.42 0.128890702734081
0.43 0.131834878004023
0.44 0.13478701960551
0.45 0.137751083136861
0.46 0.140732537839739
0.47 0.143717139010105
0.48 0.14671765763081
0.49 0.149735493387926
0.5 0.152765005688576
0.51 0.155808563246885
0.52 0.158868537107366
0.53 0.161957470129419
0.54 0.165061291385593
0.55 0.168197817115627
0.56 0.171367499811952
0.57 0.174666269702803
0.58 0.177829607021504
0.59 0.18101621481651
0.6 0.184223416362725
0.61 0.187457483814366
0.62 0.19071821669688
0.63 0.194006772892585
0.64 0.197327400048009
0.65 0.200681341097868
0.66 0.204067628640482
0.67 0.207490273600693
0.68 0.210957557695227
0.69 0.214464799543275
0.7 0.218013868978932
0.71 0.221617924974769
0.72 0.225275198327416
0.73 0.228988376399205
0.74 0.232769355436806
0.75 0.236617119426299
0.76 0.240598939459925
0.77 0.244605154450367
0.78 0.248650489216135
0.79 0.252777593159709
0.8 0.257010751310465
0.81 0.261343272236843
0.82 0.265803804715545
0.83 0.270386714134838
0.84 0.275117860268604
0.85 0.280014105611629
0.86 0.28508300355314
0.87 0.290370052636898
0.88 0.295923202082853
0.89 0.301765457856349
0.9 0.307828434571518
0.91 0.314270712138431
0.92 0.321162978293597
0.93 0.328632979737236
0.94 0.336819235790855
0.95 0.345997741187934
0.96 0.356430187564898
0.97 0.36885113144829
0.98 0.384707002592196
0.99 0.408198618406277
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.0154420916590606
0.02 0.020211725101579
0.03 0.0249912979513173
0.04 0.029757363342014
0.05 0.034533038001498
0.06 0.0393027265771483
0.07 0.0440784027785916
0.08 0.0488416587858009
0.09 0.0536087180205859
0.1 0.0583731026243194
0.11 0.0631379030843024
0.12 0.067905918498334
0.13 0.0726673610740865
0.14 0.0774347212574974
0.15 0.0821965243022183
0.16 0.0869633442954088
0.17 0.0917163391351455
0.18 0.0964742509656715
0.19 0.101228816674748
0.2 0.105992937924092
0.21 0.110754817611819
0.22 0.115514210683848
0.23 0.120277239248955
0.24 0.125039649357884
0.25 0.129811524818623
0.26 0.134576114162174
0.27 0.139346295566303
0.28 0.144128588555303
0.29 0.148920854052014
0.3 0.153741558482616
0.31 0.158644482858932
0.32 0.163398946393594
0.33 0.168154838288872
0.34 0.172917432553191
0.35 0.177682875818755
0.36 0.182454205906678
0.37 0.187233022789969
0.38 0.192019174160761
0.39 0.196816833977923
0.4 0.20162183592545
0.41 0.20643884990898
0.42 0.211271052137705
0.43 0.216110682070977
0.44 0.220966190694545
0.45 0.225832780157246
0.46 0.23070985500814
0.47 0.235598255418214
0.48 0.240515148706265
0.49 0.245437696578704
0.5 0.250373603368227
0.51 0.255336875641989
0.52 0.260320816690678
0.53 0.265326679027623
0.54 0.270351043012186
0.55 0.275405480706472
0.56 0.280489448656538
0.57 0.285652913891572
0.58 0.290746797523548
0.59 0.295866527893141
0.6 0.301012694605614
0.61 0.306191486679041
0.62 0.311399145809063
0.63 0.316649238395657
0.64 0.321930259491583
0.65 0.327246673198643
0.66 0.332604525500773
0.67 0.33800271791452
0.68 0.34343115650162
0.69 0.348919050080947
0.7 0.354445851287279
0.71 0.360027501435652
0.72 0.365673241544315
0.73 0.371378104150406
0.74 0.377158174700739
0.75 0.383015115452831
0.76 0.388962797464518
0.77 0.394976798448479
0.78 0.401060599477021
0.79 0.407243595228857
0.8 0.413529570075536
0.81 0.41993943680617
0.82 0.426477511334785
0.83 0.433154009254529
0.84 0.440003601755875
0.85 0.447036789941316
0.86 0.454274881407395
0.87 0.4617490364596
0.88 0.469492129833125
0.89 0.477578824721162
0.9 0.485968914317837
0.91 0.494795316305141
0.92 0.504131928339475
0.93 0.514090102443935
0.94 0.524881101489389
0.95 0.536732257431592
0.96 0.550032072251295
0.97 0.565553977978781
0.98 0.584830513651391
0.99 0.61234133140028
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.0207873640610694
0.02 0.0281323704181471
0.03 0.0354920586404265
0.04 0.0428423400509216
0.05 0.0501935017130135
0.06 0.0575389244240149
0.07 0.0648734411118553
0.08 0.0722125193797375
0.09 0.0795432258225546
0.1 0.0868597510437475
0.11 0.0941798632747825
0.12 0.101483459727502
0.13 0.108770536270458
0.14 0.11604543725089
0.15 0.123327048457192
0.16 0.130591345218539
0.17 0.137846629475701
0.18 0.145092493691974
0.19 0.152340489538969
0.2 0.159575646031932
0.21 0.166806440520818
0.22 0.174020773679423
0.23 0.181231889123003
0.24 0.188442111745832
0.25 0.195649822001483
0.26 0.202849928801398
0.27 0.210055041747731
0.28 0.217246971987404
0.29 0.224433087370184
0.3 0.231654276925206
0.31 0.238927988577375
0.32 0.246085419105423
0.33 0.253228878325377
0.34 0.260353728695605
0.35 0.267483146472936
0.36 0.274599471947556
0.37 0.281713128979667
0.38 0.288827958088102
0.39 0.295950259928622
0.4 0.303057854457844
0.41 0.310173516111135
0.42 0.317283406811425
0.43 0.324389097452795
0.44 0.331508051016097
0.45 0.338636402168584
0.46 0.345765035858338
0.47 0.352899673180705
0.48 0.3600339216259
0.49 0.367172796352002
0.5 0.374322900388334
0.51 0.381487146485244
0.52 0.388661737733055
0.53 0.395845751942287
0.54 0.403018105711307
0.55 0.410208296637321
0.56 0.417426927836278
0.57 0.424696247600334
0.58 0.431898162533304
0.59 0.439108468584131
0.6 0.446336174707485
0.61 0.45358850455816
0.62 0.460851760440983
0.63 0.468133163499744
0.64 0.475442434336714
0.65 0.482762634093814
0.66 0.490119034105781
0.67 0.497502769072972
0.68 0.504901972636084
0.69 0.512331140006484
0.7 0.519799749251311
0.71 0.527298745631314
0.72 0.53484548310612
0.73 0.542432761224766
0.74 0.550069306932245
0.75 0.55774987553091
0.76 0.565503536462906
0.77 0.573298138293731
0.78 0.581148251626083
0.79 0.589072857292034
0.8 0.597088126814688
0.81 0.605186610287904
0.82 0.613393788599743
0.83 0.62171073564274
0.84 0.630143469962503
0.85 0.63871508405653
0.86 0.647441953027095
0.87 0.656352221154003
0.88 0.665476160103159
0.89 0.674843939940605
0.9 0.684477545322429
0.91 0.694446575687311
0.92 0.704820931321231
0.93 0.715673046036438
0.94 0.727156123008848
0.95 0.739463817945248
0.96 0.752893502979164
0.97 0.768008259789659
0.98 0.785923032675035
0.99 0.809847779262083
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/active-splatfacto/empirical_coverage_absolute_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.0369416096286123, ymax=0.775773802200859,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.00881715157806513
0.02 0.0162495304064738
0.03 0.0239730623045358
0.04 0.0318007954803867
0.05 0.0398044654113227
0.06 0.0478984286948308
0.07 0.0559865882270196
0.08 0.0640915564525337
0.09 0.0722796602611708
0.1 0.0804688663839308
0.11 0.0886585580513771
0.12 0.0968847248535884
0.13 0.105166141791547
0.14 0.11343769389874
0.15 0.12172277418237
0.16 0.130003253166088
0.17 0.138285387214086
0.18 0.146560556095058
0.19 0.154829882089263
0.2 0.163089214348354
0.21 0.171343886971174
0.22 0.179583293478664
0.23 0.18782629511664
0.24 0.196082484554218
0.25 0.204318965651053
0.26 0.212539861966426
0.27 0.220740271939326
0.28 0.228867521994003
0.29 0.236951160291354
0.3 0.24501308941205
0.31 0.253003341453805
0.32 0.261108908504633
0.33 0.269261448163176
0.34 0.277434986133977
0.35 0.285608584567472
0.36 0.293779047513287
0.37 0.301945909862985
0.38 0.310102590760244
0.39 0.318249761576084
0.4 0.326387014506216
0.41 0.334524920931405
0.42 0.342655916550378
0.43 0.350789811036303
0.44 0.358926878404808
0.45 0.367077923951551
0.46 0.375249069250711
0.47 0.383440867159448
0.48 0.391637535188777
0.49 0.399836960566006
0.5 0.408031055107489
0.51 0.416223319014388
0.52 0.424404753508949
0.53 0.432579801209624
0.54 0.44074674718
0.55 0.448899284815953
0.56 0.457034523009468
0.57 0.465096541193071
0.58 0.473222425253126
0.59 0.481341399381336
0.6 0.489446324291703
0.61 0.497528094593566
0.62 0.505597560094622
0.63 0.513650413895015
0.64 0.521683369572573
0.65 0.529693005352185
0.66 0.53767693341123
0.67 0.545630189171688
0.68 0.553559762994056
0.69 0.561456409253671
0.7 0.569318574104718
0.71 0.577137146659886
0.72 0.584919190216379
0.73 0.592656955577777
0.74 0.600344156462822
0.75 0.607980914854998
0.76 0.615527750574975
0.77 0.623032443396301
0.78 0.630518177917058
0.79 0.637935731980569
0.8 0.645274693743612
0.81 0.652533825183865
0.82 0.659704897255281
0.83 0.666771682925429
0.84 0.673735552733482
0.85 0.680570951481107
0.86 0.687274757215714
0.87 0.693817438714825
0.88 0.700171299106072
0.89 0.706260325295772
0.9 0.712180172271104
0.91 0.717805389990978
0.92 0.723079334579562
0.93 0.727895053737396
0.94 0.732138960259906
0.95 0.735571803697851
0.96 0.737988502248874
0.97 0.738832192572247
0.98 0.736841501831461
0.99 0.728482538121252
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.0109367895022566
0.02 0.0155363689421279
0.03 0.0207053904431241
0.04 0.0265046995063189
0.05 0.0325897319989063
0.06 0.0390785288034375
0.07 0.0457994842777943
0.08 0.0526917090661937
0.09 0.0595874302063228
0.1 0.0664847975185313
0.11 0.0735129273337765
0.12 0.0805490466035588
0.13 0.0875876464258087
0.14 0.0946242234067333
0.15 0.10165678906701
0.16 0.108695767140253
0.17 0.115726040052313
0.18 0.122753813637306
0.19 0.129778948477659
0.2 0.136803976445001
0.21 0.143825976476897
0.22 0.150846402722913
0.23 0.157858292680986
0.24 0.164868433820835
0.25 0.171880084156658
0.26 0.178890140229437
0.27 0.185894428565026
0.28 0.192897119241906
0.29 0.199885874706749
0.3 0.206839905511861
0.31 0.213673407458409
0.32 0.220683520974196
0.33 0.227757440565529
0.34 0.234881056366684
0.35 0.241997464351627
0.36 0.249105976383017
0.37 0.256208684674887
0.38 0.263303407968931
0.39 0.270391610543046
0.4 0.277471086827686
0.41 0.284531839932375
0.42 0.29158615169252
0.43 0.298634634665506
0.44 0.305674807414075
0.45 0.312702423809722
0.46 0.319713075935338
0.47 0.326717397619805
0.48 0.333706780169861
0.49 0.340677713108704
0.5 0.347637437909821
0.51 0.354581581793728
0.52 0.361508811323718
0.53 0.368406613286327
0.54 0.375289953916311
0.55 0.382140566355686
0.56 0.388954944580482
0.57 0.395641498527678
0.58 0.40246121416823
0.59 0.409258026942101
0.6 0.416035865818773
0.61 0.422793704314756
0.62 0.429524171806559
0.63 0.436227545275227
0.64 0.442896618409693
0.65 0.449533456761843
0.66 0.456135879334815
0.67 0.462702418825186
0.68 0.469224817232981
0.69 0.475705449485088
0.7 0.482144965652081
0.71 0.48852901499471
0.72 0.494859586096281
0.73 0.501133404604905
0.74 0.507339600023339
0.75 0.513477889873454
0.76 0.519481074213255
0.77 0.525459756870867
0.78 0.53139969922115
0.79 0.53725676956476
0.8 0.543008941892742
0.81 0.548660417377926
0.82 0.554196195284455
0.83 0.559613285865162
0.84 0.564882139731396
0.85 0.569985894388371
0.86 0.57491699644686
0.87 0.579629947363102
0.88 0.584076797917147
0.89 0.588234542143651
0.9 0.592171565428482
0.91 0.595729287861569
0.92 0.598837021706403
0.93 0.601367020262764
0.94 0.603180764209145
0.95 0.604002258812065
0.96 0.603569812435102
0.97 0.60114886855171
0.98 0.595292997407804
0.99 0.581801381593723
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.0123329026410629
0.02 0.0151165892713093
0.03 0.0182690000420455
0.04 0.0215931612201911
0.05 0.0252236899305876
0.06 0.0292729280186246
0.07 0.0335344111431275
0.08 0.0379590494145394
0.09 0.0426657687244161
0.1 0.047388227606683
0.11 0.0522694876787485
0.12 0.0573117798045637
0.13 0.0623507679928855
0.14 0.0673911876933479
0.15 0.0724419873000103
0.16 0.0775330942238828
0.17 0.0826342101955833
0.18 0.0877294605265502
0.19 0.0928209910239642
0.2 0.0979026843914698
0.21 0.102974314168574
0.22 0.108051008592903
0.23 0.113114541215912
0.24 0.118253084589854
0.25 0.12343457173012
0.26 0.128613959398573
0.27 0.133781593389967
0.28 0.138945972996586
0.29 0.144098117747196
0.3 0.149220536086298
0.31 0.154258907308569
0.32 0.159539333641687
0.33 0.164820049947771
0.34 0.170087050129555
0.35 0.17534490001409
0.36 0.180596153680682
0.37 0.18583555634987
0.38 0.191064194676074
0.39 0.196280180426191
0.4 0.20148112332219
0.41 0.206669285257801
0.42 0.211836483090962
0.43 0.216991730786594
0.44 0.222128684885806
0.45 0.227246817934006
0.46 0.232355775350753
0.47 0.237448838192958
0.48 0.242516825910448
0.49 0.24757279570691
0.5 0.252613140068812
0.51 0.257620469225328
0.52 0.262609034993584
0.53 0.267567673656531
0.54 0.272502390295589
0.55 0.277403591275151
0.56 0.282271672362198
0.57 0.287054121363207
0.58 0.291906035757733
0.59 0.296731068078454
0.6 0.301520568296545
0.61 0.306289374790052
0.62 0.311026361113887
0.63 0.315716334050468
0.64 0.320374288471885
0.65 0.324994521518991
0.66 0.329568479444006
0.67 0.33409941219402
0.68 0.338595803125831
0.69 0.343029221364101
0.7 0.347421846045335
0.71 0.351754392376827
0.72 0.356020455915957
0.73 0.360222175079734
0.74 0.364346702735918
0.75 0.368404693806224
0.76 0.372369716577933
0.77 0.376282261388014
0.78 0.380122325209903
0.79 0.383870164009611
0.8 0.387511879026026
0.81 0.391028882650789
0.82 0.394415134535395
0.83 0.397659342447262
0.84 0.400728475282102
0.85 0.403619771980523
0.86 0.406313161873891
0.87 0.408777757665062
0.88 0.410972503086086
0.89 0.412822522979513
0.9 0.414366758328018
0.91 0.415491705786315
0.92 0.416107172286569
0.93 0.4160992998435
0.94 0.415262306579211
0.95 0.413377331455281
0.96 0.410044777791544
0.97 0.404489602527824
0.98 0.395180511226344
0.99 0.37765866859972
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.0141951404234812
0.02 0.015449725159981
0.03 0.0170109535077804
0.04 0.018725595615172
0.05 0.020596121736279
0.06 0.0226986723671041
0.07 0.0249044361530493
0.08 0.027130493319231
0.09 0.0294589749435411
0.1 0.0318653102922082
0.11 0.0343425483423171
0.12 0.0369000181496844
0.13 0.039457034268763
0.14 0.0420784410697507
0.15 0.0448663063358281
0.16 0.0477265442993988
0.17 0.0505721310015463
0.18 0.0534074361120461
0.19 0.0562345570701914
0.2 0.0590603295575699
0.21 0.0619074681407649
0.22 0.0647373714291464
0.23 0.0675619232461473
0.24 0.0704016227343484
0.25 0.0732490515643597
0.26 0.0761138889376387
0.27 0.0789992931311524
0.28 0.0818667212934985
0.29 0.0847248672911245
0.3 0.0875512656254856
0.31 0.0903304114163666
0.32 0.0931845024770011
0.33 0.0960269243230712
0.34 0.0988820790295874
0.35 0.101746561513683
0.36 0.104648312138916
0.37 0.107583836771128
0.38 0.110509498932385
0.39 0.113412681132517
0.4 0.116297745791118
0.41 0.119171406969862
0.42 0.122024900322847
0.43 0.124862088950929
0.44 0.127671752490316
0.45 0.130460302475597
0.46 0.13322141145563
0.47 0.135959857301511
0.48 0.138679214562823
0.49 0.1413656187845
0.5 0.144029021087763
0.51 0.14666711714753
0.52 0.149275157326908
0.53 0.151875797471664
0.54 0.154470062021369
0.55 0.157025445705692
0.56 0.159551074127783
0.57 0.162026962328374
0.58 0.164530926650222
0.59 0.167013653567411
0.6 0.169457009458796
0.61 0.17185793253513
0.62 0.174258130758548
0.63 0.176609405535595
0.64 0.178928001459595
0.65 0.181317819084842
0.66 0.183659498673954
0.67 0.185956780951818
0.68 0.18821688222971
0.69 0.190427110136484
0.7 0.192584456041512
0.71 0.194698623935692
0.72 0.196755161827427
0.73 0.198763379178131
0.74 0.200719401234919
0.75 0.202629628317134
0.76 0.204457163394375
0.77 0.206216604895977
0.78 0.207918663739715
0.79 0.209526738352748
0.8 0.211034854890258
0.81 0.212449658773015
0.82 0.213734792195304
0.83 0.214904332250516
0.84 0.215936281826018
0.85 0.216828640251579
0.86 0.217563373804432
0.87 0.218125248040582
0.88 0.21846637226755
0.89 0.218567679487012
0.9 0.218417944441406
0.91 0.217970740857608
0.92 0.21714187202188
0.93 0.215871847788178
0.94 0.214029967902714
0.95 0.211415025247822
0.96 0.20770664038509
0.97 0.202326291247895
0.98 0.194194151753365
0.99 0.180165311335039
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/active-splatfacto/empirical_coverage_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.776313170403913, ymax=0.0482683418927352,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 -0.00552470429333298
0.02 -0.0137890464993872
0.03 -0.0220711109919064
0.04 -0.0303669088020077
0.05 -0.0386668761550933
0.06 -0.0469711400114402
0.07 -0.0552723712905658
0.08 -0.0635681931861116
0.09 -0.0718638282350395
0.1 -0.0801627538443167
0.11 -0.088465322677708
0.12 -0.0967692802535265
0.13 -0.105059645046855
0.14 -0.113337518379375
0.15 -0.121627247857471
0.16 -0.129910976747416
0.17 -0.138196384418391
0.18 -0.146479736289551
0.19 -0.15476249260484
0.2 -0.163034988371581
0.21 -0.171303322553795
0.22 -0.179567187671033
0.23 -0.18782629511664
0.24 -0.196082484554218
0.25 -0.204318965651053
0.26 -0.212539861966426
0.27 -0.220740271939326
0.28 -0.228867521994003
0.29 -0.236951160291354
0.3 -0.24501308941205
0.31 -0.253003341453805
0.32 -0.261108908504633
0.33 -0.269261448163176
0.34 -0.277434986133977
0.35 -0.285608584567472
0.36 -0.293779047513287
0.37 -0.301945909862985
0.38 -0.310102590760244
0.39 -0.318249761576084
0.4 -0.326387014506216
0.41 -0.334524920931405
0.42 -0.342655916550378
0.43 -0.350789811036303
0.44 -0.358926878404808
0.45 -0.367077923951551
0.46 -0.375249069250711
0.47 -0.383440867159448
0.48 -0.391637535188777
0.49 -0.399836960566006
0.5 -0.408031055107489
0.51 -0.416223319014388
0.52 -0.424404753508949
0.53 -0.432579801209624
0.54 -0.44074674718
0.55 -0.448899284815953
0.56 -0.457034523009468
0.57 -0.465096541193071
0.58 -0.473222425253126
0.59 -0.481341399381336
0.6 -0.489446324291703
0.61 -0.497528094593566
0.62 -0.505597560094622
0.63 -0.513650413895015
0.64 -0.521683369572573
0.65 -0.529693005352185
0.66 -0.53767693341123
0.67 -0.545630189171688
0.68 -0.553559762994056
0.69 -0.561456409253671
0.7 -0.569318574104718
0.71 -0.577137146659886
0.72 -0.584919190216379
0.73 -0.592656955577777
0.74 -0.600344156462822
0.75 -0.607980914854998
0.76 -0.615527750574975
0.77 -0.623032443396301
0.78 -0.630518177917058
0.79 -0.637935731980569
0.8 -0.645274693743612
0.81 -0.652533825183865
0.82 -0.659704897255281
0.83 -0.666771682925429
0.84 -0.673735552733482
0.85 -0.680570951481107
0.86 -0.687274757215714
0.87 -0.693817438714825
0.88 -0.700171299106072
0.89 -0.706260325295772
0.9 -0.712180172271104
0.91 -0.717805389990978
0.92 -0.723079334579562
0.93 -0.727895053737396
0.94 -0.732138960259906
0.95 -0.735571803697851
0.96 -0.737988502248874
0.97 -0.738832192572247
0.98 -0.736841501831461
0.99 -0.728482538121252
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.000600016658970048
0.02 -0.00651892668822224
0.03 -0.0136462193627184
0.04 -0.0207803211157715
0.05 -0.0279104859948603
0.06 -0.0350428796614127
0.07 -0.0421801503058247
0.08 -0.0493097440981571
0.09 -0.0564436482415458
0.1 -0.0635809449023801
0.11 -0.0707163664836612
0.12 -0.0778535290829112
0.13 -0.0849908090253496
0.14 -0.0921266321668255
0.15 -0.0992634688449845
0.16 -0.106403382023023
0.17 -0.113537280160645
0.18 -0.120669436552913
0.19 -0.12779952150015
0.2 -0.134932705208376
0.21 -0.142062882796961
0.22 -0.149189346016178
0.23 -0.156308635084253
0.24 -0.163427183209949
0.25 -0.170548167532264
0.26 -0.17766790156142
0.27 -0.1847807149185
0.28 -0.19189348265071
0.29 -0.198993056251313
0.3 -0.206058305559395
0.31 -0.213002059605424
0.32 -0.22012698831747
0.33 -0.227252463054167
0.34 -0.234377123815318
0.35 -0.241492068713965
0.36 -0.24860242021647
0.37 -0.255707483818765
0.38 -0.262805949853097
0.39 -0.269898007822062
0.4 -0.276981535164737
0.41 -0.284047928349699
0.42 -0.291109297265919
0.43 -0.298165121995977
0.44 -0.30521298039449
0.45 -0.312248916863139
0.46 -0.319267462160261
0.47 -0.326282860989895
0.48 -0.33328234236919
0.49 -0.340264506612074
0.5 -0.347234994311424
0.51 -0.354191436753115
0.52 -0.361131462892634
0.53 -0.368042529870581
0.54 -0.374938708614407
0.55 -0.381802182884373
0.56 -0.388632500188048
0.57 -0.395333730297197
0.58 -0.402170392978495
0.59 -0.40898378518349
0.6 -0.415776583637275
0.61 -0.422542516185634
0.62 -0.42928178330312
0.63 -0.435993227107415
0.64 -0.442672599951991
0.65 -0.449318658902132
0.66 -0.455932371359518
0.67 -0.462509726399307
0.68 -0.469042442304773
0.69 -0.475535200456725
0.7 -0.481986131021068
0.71 -0.488382075025231
0.72 -0.494724801672584
0.73 -0.501011623600795
0.74 -0.507230644563194
0.75 -0.513382880573701
0.76 -0.519401060540075
0.77 -0.525394845549633
0.78 -0.531349510783865
0.79 -0.537222406840291
0.8 -0.542989248689535
0.81 -0.548656727763157
0.82 -0.554196195284455
0.83 -0.559613285865162
0.84 -0.564882139731396
0.85 -0.569985894388371
0.86 -0.57491699644686
0.87 -0.579629947363102
0.88 -0.584076797917147
0.89 -0.588234542143651
0.9 -0.592171565428482
0.91 -0.595729287861569
0.92 -0.598837021706403
0.93 -0.601367020262764
0.94 -0.603180764209145
0.95 -0.604002258812065
0.96 -0.603569812435102
0.97 -0.60114886855171
0.98 -0.595292997407804
0.99 -0.581801381593723
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.00544209165906063
0.02 0.000211725101578961
0.03 -0.00500870204868268
0.04 -0.0102426366579859
0.05 -0.0154669619985019
0.06 -0.0206972734228516
0.07 -0.0259215972214083
0.08 -0.031158341214199
0.09 -0.036391281979414
0.1 -0.0416268973756806
0.11 -0.0468620969156976
0.12 -0.052094081501666
0.13 -0.0573326389259134
0.14 -0.0625652787425026
0.15 -0.0678034756977817
0.16 -0.0730366557045911
0.17 -0.0782836608648544
0.18 -0.0835257490343284
0.19 -0.0887711833252518
0.2 -0.0940070620759079
0.21 -0.0992451823881813
0.22 -0.104485789316152
0.23 -0.109722760751045
0.24 -0.114960350642116
0.25 -0.120188475181377
0.26 -0.125423885837826
0.27 -0.130653704433697
0.28 -0.135871411444697
0.29 -0.141079145947986
0.3 -0.146258441517384
0.31 -0.151355517141068
0.32 -0.156601053606406
0.33 -0.161845161711127
0.34 -0.167082567446808
0.35 -0.172317124181245
0.36 -0.177545794093322
0.37 -0.182766977210031
0.38 -0.187980825839239
0.39 -0.193183166022077
0.4 -0.19837816407455
0.41 -0.20356115009102
0.42 -0.208728947862295
0.43 -0.213889317929023
0.44 -0.219033809305455
0.45 -0.224167219842754
0.46 -0.22929014499186
0.47 -0.234401744581786
0.48 -0.239484851293735
0.49 -0.244562303421296
0.5 -0.249626396631773
0.51 -0.254663124358011
0.52 -0.259679183309322
0.53 -0.264673320972377
0.54 -0.269648956987814
0.55 -0.274594519293528
0.56 -0.279510551343462
0.57 -0.284347086108428
0.58 -0.289253202476452
0.59 -0.294133472106859
0.6 -0.298987305394386
0.61 -0.303808513320959
0.62 -0.308600854190937
0.63 -0.313350761604343
0.64 -0.318069740508416
0.65 -0.322753326801356
0.66 -0.327395474499227
0.67 -0.33199728208548
0.68 -0.33656884349838
0.69 -0.341080949919053
0.7 -0.345554148712721
0.71 -0.349972498564348
0.72 -0.354326758455685
0.73 -0.358621895849594
0.74 -0.362841825299261
0.75 -0.366984884547169
0.76 -0.371037202535482
0.77 -0.375023201551521
0.78 -0.378939400522979
0.79 -0.382756404771143
0.8 -0.386470429924464
0.81 -0.39006056319383
0.82 -0.393522488665215
0.83 -0.396845990745471
0.84 -0.399996398244125
0.85 -0.402963210058684
0.86 -0.405725118592605
0.87 -0.408250963540399
0.88 -0.410507870166875
0.89 -0.412421175278838
0.9 -0.414031085682163
0.91 -0.415204683694859
0.92 -0.415868071660525
0.93 -0.415909897556065
0.94 -0.415118898510611
0.95 -0.413267742568408
0.96 -0.409967927748705
0.97 -0.404446022021218
0.98 -0.395169486348609
0.99 -0.37765866859972
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.0107873640610694
0.02 0.00813237041814707
0.03 0.00549205864042643
0.04 0.00284234005092165
0.05 0.000193501713013526
0.06 -0.00246107557598508
0.07 -0.00512655888814469
0.08 -0.00778748062026251
0.09 -0.0104567741774454
0.1 -0.0131402489562525
0.11 -0.0158201367252174
0.12 -0.0185165402724978
0.13 -0.0212294637295424
0.14 -0.0239545627491103
0.15 -0.0266729515428084
0.16 -0.029408654781461
0.17 -0.0321533705242988
0.18 -0.0349075063080262
0.19 -0.037659510461031
0.2 -0.040424353968068
0.21 -0.0431935594791823
0.22 -0.0459792263205767
0.23 -0.0487681108769968
0.24 -0.051557888254168
0.25 -0.0543501779985171
0.26 -0.0571500711986019
0.27 -0.0599449582522689
0.28 -0.0627530280125963
0.29 -0.0655669126298162
0.3 -0.0683457230747942
0.31 -0.0710720114226252
0.32 -0.0739145808945766
0.33 -0.0767711216746233
0.34 -0.0796462713043946
0.35 -0.0825168535270639
0.36 -0.0854005280524437
0.37 -0.0882868710203325
0.38 -0.0911720419118981
0.39 -0.0940497400713784
0.4 -0.0969421455421559
0.41 -0.0998264838888651
0.42 -0.102716593188575
0.43 -0.105610902547205
0.44 -0.108491948983903
0.45 -0.111363597831415
0.46 -0.114234964141662
0.47 -0.117100326819295
0.48 -0.1199660783741
0.49 -0.122827203647998
0.5 -0.125677099611666
0.51 -0.128512853514756
0.52 -0.131338262266945
0.53 -0.134154248057713
0.54 -0.136981894288693
0.55 -0.139791703362679
0.56 -0.142573072163722
0.57 -0.145303752399666
0.58 -0.148101837466696
0.59 -0.150891531415869
0.6 -0.153663825292515
0.61 -0.15641149544184
0.62 -0.159148239559017
0.63 -0.161866836500256
0.64 -0.164557565663286
0.65 -0.167237365906186
0.66 -0.169880965894219
0.67 -0.172497230927028
0.68 -0.175098027363916
0.69 -0.177668859993516
0.7 -0.180200250748689
0.71 -0.182701254368686
0.72 -0.18515451689388
0.73 -0.187567238775234
0.74 -0.189930693067755
0.75 -0.19225012446909
0.76 -0.194496463537094
0.77 -0.196701861706269
0.78 -0.198851748373917
0.79 -0.200927142707966
0.8 -0.202911873185312
0.81 -0.204813389712096
0.82 -0.206606211400257
0.83 -0.20828926435726
0.84 -0.209856530037497
0.85 -0.21128491594347
0.86 -0.212558046972905
0.87 -0.213647778845997
0.88 -0.214523839896841
0.89 -0.215156060059395
0.9 -0.215522454677572
0.91 -0.215553424312689
0.92 -0.215179068678769
0.93 -0.214326953963562
0.94 -0.212843876991152
0.95 -0.210536182054752
0.96 -0.207106497020836
0.97 -0.201991740210341
0.98 -0.194076967324965
0.99 -0.180152220737917
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/active-splatfacto/empirical_coverage_negative_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.0369416096286123, ymax=0.775773802200859,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.00717092793569906
0.02 0.0150192884529305
0.03 0.0230220866482211
0.04 0.0310838521411972
0.05 0.039235670783208
0.06 0.0474347843531355
0.07 0.0556294797587927
0.08 0.0638298748193226
0.09 0.0720717442481052
0.1 0.0803158101141238
0.11 0.0885619403645425
0.12 0.0968270025535574
0.13 0.105112893419201
0.14 0.113387606139057
0.15 0.12167501101992
0.16 0.129957114956752
0.17 0.138240885816239
0.18 0.146520146192305
0.19 0.154796187347052
0.2 0.163062101359967
0.21 0.171323604762484
0.22 0.179575240574849
0.23 0.18782629511664
0.24 0.196082484554218
0.25 0.204318965651053
0.26 0.212539861966426
0.27 0.220740271939326
0.28 0.228867521994003
0.29 0.236951160291354
0.3 0.24501308941205
0.31 0.253003341453805
0.32 0.261108908504633
0.33 0.269261448163176
0.34 0.277434986133977
0.35 0.285608584567472
0.36 0.293779047513287
0.37 0.301945909862985
0.38 0.310102590760244
0.39 0.318249761576084
0.4 0.326387014506216
0.41 0.334524920931405
0.42 0.342655916550378
0.43 0.350789811036303
0.44 0.358926878404808
0.45 0.367077923951551
0.46 0.375249069250711
0.47 0.383440867159448
0.48 0.391637535188777
0.49 0.399836960566006
0.5 0.408031055107489
0.51 0.416223319014388
0.52 0.424404753508949
0.53 0.432579801209624
0.54 0.44074674718
0.55 0.448899284815953
0.56 0.457034523009468
0.57 0.465096541193071
0.58 0.473222425253126
0.59 0.481341399381336
0.6 0.489446324291703
0.61 0.497528094593566
0.62 0.505597560094622
0.63 0.513650413895015
0.64 0.521683369572573
0.65 0.529693005352185
0.66 0.53767693341123
0.67 0.545630189171688
0.68 0.553559762994056
0.69 0.561456409253671
0.7 0.569318574104718
0.71 0.577137146659886
0.72 0.584919190216379
0.73 0.592656955577777
0.74 0.600344156462822
0.75 0.607980914854998
0.76 0.615527750574975
0.77 0.623032443396301
0.78 0.630518177917058
0.79 0.637935731980569
0.8 0.645274693743612
0.81 0.652533825183865
0.82 0.659704897255281
0.83 0.666771682925429
0.84 0.673735552733482
0.85 0.680570951481107
0.86 0.687274757215714
0.87 0.693817438714825
0.88 0.700171299106072
0.89 0.706260325295772
0.9 0.712180172271104
0.91 0.717805389990978
0.92 0.723079334579562
0.93 0.727895053737396
0.94 0.732138960259906
0.95 0.735571803697851
0.96 0.737988502248874
0.97 0.738832192572247
0.98 0.736841501831461
0.99 0.728482538121252
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.00516838642164325
0.02 0.0110276478151751
0.03 0.0171758049029212
0.04 0.0236425103110452
0.05 0.0302501089968833
0.06 0.0370607042324251
0.07 0.0439898172918095
0.08 0.0510007265821754
0.09 0.0580155392239343
0.1 0.0650328712104556
0.11 0.0721146469087188
0.12 0.079201287843235
0.13 0.0862892277255791
0.14 0.0933754277867794
0.15 0.100460128955997
0.16 0.107549574581638
0.17 0.114631660106479
0.18 0.121711625095109
0.19 0.128789234988904
0.2 0.135868340826688
0.21 0.142944429636929
0.22 0.150017874369546
0.23 0.15708346388262
0.24 0.164147808515392
0.25 0.171214125844461
0.26 0.178279020895428
0.27 0.185337571741763
0.28 0.192395300946308
0.29 0.199439465479031
0.3 0.206449105535628
0.31 0.213337733531917
0.32 0.220405254645833
0.33 0.227504951809848
0.34 0.234629090091001
0.35 0.241744766532796
0.36 0.248854198299743
0.37 0.255958084246826
0.38 0.263054678911014
0.39 0.270144809182554
0.4 0.277226310996211
0.41 0.284289884141037
0.42 0.291347724479219
0.43 0.298399878330742
0.44 0.305443893904282
0.45 0.31247567033643
0.46 0.319490269047799
0.47 0.32650012930485
0.48 0.333494561269526
0.49 0.340471109860389
0.5 0.347436216110623
0.51 0.354386509273421
0.52 0.361320137108176
0.53 0.368224571578454
0.54 0.375114331265359
0.55 0.38197137462003
0.56 0.388793722384265
0.57 0.395487614412437
0.58 0.402315803573363
0.59 0.409120906062795
0.6 0.415906224728024
0.61 0.422668110250195
0.62 0.429402977554839
0.63 0.436110386191321
0.64 0.442784609180842
0.65 0.449426057831987
0.66 0.456034125347166
0.67 0.462606072612247
0.68 0.469133629768877
0.69 0.475620324970906
0.7 0.482065548336575
0.71 0.48845554500997
0.72 0.494792193884432
0.73 0.50107251410285
0.74 0.507285122293266
0.75 0.513430385223577
0.76 0.519441067376665
0.77 0.52542730121025
0.78 0.531374605002508
0.79 0.537239588202526
0.8 0.542999095291139
0.81 0.548658572570541
0.82 0.554196195284455
0.83 0.559613285865162
0.84 0.564882139731396
0.85 0.569985894388371
0.86 0.57491699644686
0.87 0.579629947363102
0.88 0.584076797917147
0.89 0.588234542143651
0.9 0.592171565428482
0.91 0.595729287861569
0.92 0.598837021706403
0.93 0.601367020262764
0.94 0.603180764209145
0.95 0.604002258812065
0.96 0.603569812435102
0.97 0.60114886855171
0.98 0.595292997407804
0.99 0.581801381593723
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.00344540549100114
0.02 0.00745243208486516
0.03 0.0116388510453641
0.04 0.0159178989390885
0.05 0.0203453259645448
0.06 0.0249851007207381
0.07 0.0297280041822679
0.08 0.0345586953143692
0.09 0.0395285253519151
0.1 0.0445075624911818
0.11 0.0495657922972231
0.12 0.0547029306531149
0.13 0.0598417034593995
0.14 0.0649782332179252
0.15 0.070122731498896
0.16 0.0752848749642369
0.17 0.0804589355302189
0.18 0.0856276047804393
0.19 0.090796087174608
0.2 0.0959548732336888
0.21 0.101109748278378
0.22 0.106268398954527
0.23 0.111418650983478
0.24 0.116606717615985
0.25 0.121811523455749
0.26 0.1270189226182
0.27 0.132217648911832
0.28 0.137408692220641
0.29 0.142588631847591
0.3 0.147739488801841
0.31 0.152807212224819
0.32 0.158070193624046
0.33 0.163332605829449
0.34 0.168584808788182
0.35 0.173831012097667
0.36 0.179070973887002
0.37 0.184301266779951
0.38 0.189522510257656
0.39 0.194731673224134
0.4 0.19992964369837
0.41 0.205115217674411
0.42 0.210282715476629
0.43 0.215440524357808
0.44 0.22058124709563
0.45 0.22570701888838
0.46 0.230822960171307
0.47 0.235925291387372
0.48 0.241000838602091
0.49 0.246067549564103
0.5 0.251119768350293
0.51 0.25614179679167
0.52 0.261144109151453
0.53 0.266120497314454
0.54 0.271075673641701
0.55 0.27599905528434
0.56 0.28089111185283
0.57 0.285700603735818
0.58 0.290579619117092
0.59 0.295432270092656
0.6 0.300253936845466
0.61 0.305048944055506
0.62 0.309813607652412
0.63 0.314533547827405
0.64 0.319222014490151
0.65 0.323873924160174
0.66 0.328481976971617
0.67 0.33304834713975
0.68 0.337582323312105
0.69 0.342055085641577
0.7 0.346487997379028
0.71 0.350863445470588
0.72 0.355173607185821
0.73 0.359422035464664
0.74 0.363594264017589
0.75 0.367694789176696
0.76 0.371703459556708
0.77 0.375652731469767
0.78 0.379530862866441
0.79 0.383313284390377
0.8 0.386991154475245
0.81 0.39054472292231
0.82 0.393968811600305
0.83 0.397252666596367
0.84 0.400362436763113
0.85 0.403291491019604
0.86 0.406019140233248
0.87 0.408514360602731
0.88 0.41074018662648
0.89 0.412621849129176
0.9 0.41419892200509
0.91 0.415348194740587
0.92 0.415987621973547
0.93 0.416004598699783
0.94 0.415190602544911
0.95 0.413322537011845
0.96 0.410006352770124
0.97 0.404467812274521
0.98 0.395174998787477
0.99 0.37765866859972
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.00170388818120586
0.02 0.00365867737091696
0.03 0.00575944743367701
0.04 0.00794162778212518
0.05 0.0102013100116327
0.06 0.0125798739715446
0.07 0.015015497520597
0.08 0.0174589869697468
0.09 0.0199578745604932
0.1 0.0225027796242303
0.11 0.0250813425337673
0.12 0.0277082792110911
0.13 0.0303432489991527
0.14 0.0330165019094305
0.15 0.0357696289393182
0.16 0.0385675995404299
0.17 0.0413627507629226
0.18 0.0441574712100362
0.19 0.0469470337656112
0.2 0.0497423417628189
0.21 0.0525505138099736
0.22 0.0553582988748616
0.23 0.058165017061572
0.24 0.0609797554942582
0.25 0.0637996147814384
0.26 0.0666319800681203
0.27 0.0694721256917107
0.28 0.0723098746530474
0.29 0.0751458899604703
0.3 0.0779484943501399
0.31 0.0807012114194959
0.32 0.0835495416857889
0.33 0.0863990229988473
0.34 0.089264175166991
0.35 0.0921317075203734
0.36 0.0950244200956801
0.37 0.09793535389573
0.38 0.100840770422142
0.39 0.103731210601948
0.4 0.106619945666637
0.41 0.109498945429364
0.42 0.112370746755711
0.43 0.115236495749067
0.44 0.11808185073711
0.45 0.120911950153506
0.46 0.123728187798646
0.47 0.126530092060403
0.48 0.129322646468461
0.49 0.132096411216249
0.5 0.134853060349714
0.51 0.137589985331143
0.52 0.140306709796926
0.53 0.143015022764688
0.54 0.145725978155031
0.55 0.148408574534186
0.56 0.151062073145752
0.57 0.15366535736402
0.58 0.156316382058459
0.59 0.15895259249164
0.6 0.161560417375655
0.61 0.164134713988485
0.62 0.166703185158782
0.63 0.169238121017925
0.64 0.17174278356144
0.65 0.174277592495514
0.66 0.176770232284087
0.67 0.179227005939423
0.68 0.181657454796813
0.69 0.184047985065
0.7 0.186392353395101
0.71 0.188699939152189
0.72 0.190954839360654
0.73 0.193165308976682
0.74 0.195325047151337
0.75 0.197439876393112
0.76 0.199476813465734
0.77 0.201459233301123
0.78 0.203385206056816
0.79 0.205226940530357
0.8 0.206973364037785
0.81 0.208631524242556
0.82 0.210170501797781
0.83 0.211596798303888
0.84 0.212896405931757
0.85 0.214056778097524
0.86 0.215060710388668
0.87 0.215886513443289
0.88 0.216495106082195
0.89 0.216861869773204
0.9 0.216970199559489
0.91 0.216762082585149
0.92 0.216160470350324
0.93 0.21509940087587
0.94 0.213436922446933
0.95 0.210975603651287
0.96 0.207406568702963
0.97 0.202159015729118
0.98 0.194135559539165
0.99 0.180158766036478
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/ensemble-nerfacto/avg_length.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.039, xmax=1.039,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.0146514226863566, ymax=0.318793493618429,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.01 0.00147743621126487
0.02 0.00295510487918753
0.03 0.00443323775143068
0.04 0.00591206823188818
0.05 0.00739182934434168
0.06 0.00887275731111011
0.07 0.0103550865878351
0.08 0.0118390542078739
0.09 0.013324901444114
0.1 0.0148128684043532
0.11 0.0163031996113695
0.12 0.0177961432609496
0.13 0.0192919437162505
0.14 0.0207908596978101
0.15 0.0222931435908027
0.16 0.023799056494328
0.17 0.0253088647537823
0.18 0.0268228374718823
0.19 0.0283412474168343
0.2 0.0298643728219731
0.21 0.0313925012324372
0.22 0.0329259261890695
0.23 0.0344649437871716
0.24 0.0360098533976666
0.25 0.0375609783403869
0.26 0.0391186337167602
0.27 0.0406831489067363
0.28 0.042254862156922
0.29 0.0438341276909269
0.3 0.0454212981783513
0.31 0.0470167472204563
0.32 0.048620854892575
0.33 0.0502340191030089
0.34 0.0518566470259885
0.35 0.0534891607851314
0.36 0.0551319978794187
0.37 0.0567856149295504
0.38 0.0584504831021288
0.39 0.0601270931846787
0.4 0.0618159575008471
0.41 0.0635175974321086
0.42 0.0652325922428273
0.43 0.066961500611811
0.44 0.0687049355720401
0.45 0.0704635330627752
0.46 0.0722379516609474
0.47 0.0740288955996185
0.48 0.0758370943379292
0.49 0.0776633111499569
0.5 0.0795083629817093
0.51 0.0813731026006932
0.52 0.0832584416163781
0.53 0.0851653069084909
0.54 0.0870947306644973
0.55 0.0890477759686321
0.56 0.0910255730096556
0.57 0.0930293461941201
0.58 0.0950603530481719
0.59 0.0971199856321759
0.6 0.0992097034378056
0.61 0.101331071967535
0.62 0.103485783284308
0.63 0.105675631638094
0.64 0.107902574653399
0.65 0.110168707594329
0.66 0.112476317471755
0.67 0.114827842525388
0.68 0.11722598002351
0.69 0.119673645680413
0.7 0.12217401480173
0.71 0.124730604382968
0.72 0.127347259332815
0.73 0.130028211763064
0.74 0.132778185042114
0.75 0.13560235075027
0.76 0.138506597706356
0.77 0.141497431837707
0.78 0.144582261702983
0.79 0.147769383824251
0.8 0.151068383118239
0.81 0.15449010757449
0.82 0.158047226620875
0.83 0.161754393063183
0.84 0.165628836287625
0.85 0.169690930504709
0.86 0.173965176014367
0.87 0.178481227294034
0.88 0.183275586642991
0.89 0.188393856263588
0.9 0.193894157133837
0.91 0.199852255708555
0.92 0.206369616507418
0.93 0.213586713863859
0.94 0.221706588036969
0.95 0.231039157614181
0.96 0.242094427362367
0.97 0.255808696681737
0.98 0.274228200769382
0.99 0.303636906513666
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.000861069767592682
0.02 0.00172227494550129
0.03 0.00258375064482542
0.04 0.0034456328741862
0.05 0.00430805769806618
0.06 0.00517116233149869
0.07 0.00603508368771461
0.08 0.00689996038255438
0.09 0.00776593213636742
0.1 0.00863313896455887
0.11 0.00950172383443234
0.12 0.0103718319162457
0.13 0.0112436044671269
0.14 0.0121171929398
0.15 0.0129927441085361
0.16 0.0138704117179826
0.17 0.0147503479462079
0.18 0.0156327111946505
0.19 0.0165176608498208
0.2 0.0174053579275203
0.21 0.0182959721313727
0.22 0.0191896742696329
0.23 0.0200866322923518
0.24 0.0209870279493864
0.25 0.0218910440478681
0.26 0.022798866694753
0.27 0.0237106862167208
0.28 0.0246267024951338
0.29 0.0255471195246727
0.3 0.0264721432912939
0.31 0.0274019950598629
0.32 0.0283368899679705
0.33 0.029277062353423
0.34 0.0302227509222178
0.35 0.0311742030754271
0.36 0.0321316714914202
0.37 0.0330954210416585
0.38 0.0340657278996012
0.39 0.0350428807762605
0.4 0.036027171539783
0.41 0.0370189114759306
0.42 0.0380184327523024
0.43 0.0390260650027548
0.44 0.0400421625755178
0.45 0.0410670974882341
0.46 0.0421012519418669
0.47 0.0431450406771935
0.48 0.0441988796274836
0.49 0.0452632232199302
0.5 0.0463385464846919
0.51 0.0474253390000886
0.52 0.0485241368997425
0.53 0.0496354898433997
0.54 0.0507599819068231
0.55 0.0518982442605731
0.56 0.0530509322994062
0.57 0.0542187539084968
0.58 0.0554024536347325
0.59 0.0566028382162232
0.6 0.0578207454042119
0.61 0.0590571136118263
0.62 0.0603129081399288
0.63 0.061589176833929
0.64 0.0628870715856317
0.65 0.0642078074115166
0.66 0.0655527110279495
0.67 0.0669232141479346
0.68 0.0683208801953703
0.69 0.0697474122237048
0.7 0.0712046588263678
0.71 0.0726946771417752
0.72 0.0742196942109731
0.73 0.0757821943256606
0.74 0.077384911640973
0.75 0.0790308757783369
0.76 0.0807235135031729
0.77 0.0824666073384999
0.78 0.0842644834913517
0.79 0.0861219899946462
0.8 0.0880446871031081
0.81 0.0900389184417516
0.82 0.0921120496270998
0.83 0.0942726357772669
0.84 0.0965307055994996
0.85 0.0988981608909582
0.86 0.10138924561412
0.87 0.104021265840589
0.88 0.106815476839636
0.89 0.109798481131073
0.9 0.113004129860044
0.91 0.116476590332766
0.92 0.120274988519288
0.93 0.124481216410357
0.94 0.129213583039248
0.95 0.1346527270976
0.96 0.141095890500253
0.97 0.149088745045904
0.98 0.159823889692717
0.99 0.176963678351965
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.000645518473275558
0.02 0.00129113838121455
0.03 0.0019369613021457
0.04 0.00258308885562743
0.05 0.00322962326268039
0.06 0.00387666696369415
0.07 0.00452432330766151
0.08 0.00517269571845297
0.09 0.00582188899405738
0.1 0.00647200809542995
0.11 0.00712316088992436
0.12 0.00777545456822994
0.13 0.0084289969078972
0.14 0.00908390039907565
0.15 0.00974027509845761
0.16 0.0103982358776273
0.17 0.0110578981136241
0.18 0.0117193798868491
0.19 0.0123828002995836
0.2 0.0130482817844431
0.21 0.0137159480091238
0.22 0.0143859291860362
0.23 0.0150583527393984
0.24 0.0157333520130997
0.25 0.0164110663677187
0.26 0.0170916340636988
0.27 0.0177751985736115
0.28 0.018461909437193
0.29 0.0191519178692286
0.3 0.019845380057223
0.31 0.0205424613733363
0.32 0.0212433259128629
0.33 0.0219481444274718
0.34 0.022657100275799
0.35 0.0233703755255329
0.36 0.0240881606401648
0.37 0.0248106554132286
0.38 0.0255380648213315
0.39 0.0262706074509151
0.4 0.0270085001004975
0.41 0.0277519799164363
0.42 0.0285012909323452
0.43 0.0292566829054664
0.44 0.0300184213458793
0.45 0.0307867828768985
0.46 0.0315620587174532
0.47 0.0323445567461128
0.48 0.0331345886319044
0.49 0.0339324946622212
0.5 0.0347386320083467
0.51 0.0355533716264107
0.52 0.0363771085074424
0.53 0.03721025234669
0.54 0.0380532531985539
0.55 0.0389065752623606
0.56 0.039770709066209
0.57 0.0406461928694858
0.58 0.0415335750755994
0.59 0.042433465295413
0.6 0.0433465005594534
0.61 0.0442733654992551
0.62 0.0452147983853235
0.63 0.0461715823352457
0.64 0.0471445740654678
0.65 0.0481346887985937
0.66 0.0491429201344096
0.67 0.0501703504527317
0.68 0.0512181368762742
0.69 0.0522875650859434
0.7 0.0533800211162873
0.71 0.0544970432849136
0.72 0.0556403033206587
0.73 0.0568116642340987
0.74 0.0580131714888839
0.75 0.0592471066104947
0.76 0.0605160215804382
0.77 0.0618227692444323
0.78 0.0631705863634227
0.79 0.0645631030191681
0.8 0.0660044884153648
0.81 0.0674995057760153
0.82 0.069053674053945
0.83 0.0706734030500291
0.84 0.0723662115981971
0.85 0.0741410147796571
0.86 0.0760085131196042
0.87 0.0779816565031321
0.88 0.0800763945267289
0.89 0.0823126607365001
0.9 0.0847158397970402
0.91 0.0873190428020431
0.92 0.0901665873143806
0.93 0.0933198786273724
0.94 0.0968675899964234
0.95 0.100945155861305
0.96 0.105775406418973
0.97 0.111767419374702
0.98 0.119815232224059
0.99 0.132664409386921
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.000505164418406409
0.02 0.00101040825971594
0.03 0.00151581092578746
0.04 0.00202145198035887
0.05 0.00252741137315057
0.06 0.00303376954007073
0.07 0.00354060704432637
0.08 0.00404800479369936
0.09 0.00455604506443923
0.1 0.0050648101587613
0.11 0.00557438338559559
0.12 0.00608484980656387
0.13 0.00659629354638268
0.14 0.00710880245515222
0.15 0.00762246310428604
0.16 0.00813736401436015
0.17 0.00865359706889324
0.18 0.00917125364994662
0.19 0.00969042763026429
0.2 0.0102112149198132
0.21 0.0107337113040088
0.22 0.0112580200352903
0.23 0.01178423931192
0.24 0.0123124743321647
0.25 0.0128428349102483
0.26 0.0133754279155528
0.27 0.0139103656617761
0.28 0.0144477665778431
0.29 0.0149877472943618
0.3 0.0155304315531182
0.31 0.0160759471569537
0.32 0.0166244238789398
0.33 0.0171759955177324
0.34 0.017730803056429
0.35 0.0182889930619907
0.36 0.0188507110238064
0.37 0.0194161154468792
0.38 0.0199853653495782
0.39 0.0205586329009663
0.4 0.0211360862634198
0.41 0.0217179136183463
0.42 0.022304301259406
0.43 0.0228954489091278
0.44 0.0234915639967673
0.45 0.024092862252364
0.46 0.024699571774048
0.47 0.0253119316492666
0.48 0.0259301890857661
0.49 0.0265546079539865
0.5 0.0271854680898172
0.51 0.0278230605418794
0.52 0.0284676923743054
0.53 0.0291196874974254
0.54 0.0297793959822089
0.55 0.0304471809321349
0.56 0.0311234297313815
0.57 0.0318085557084861
0.58 0.0325029980435927
0.59 0.0332072259075445
0.6 0.0339217409361164
0.61 0.0346470795146843
0.62 0.0353838181019346
0.63 0.0361325710994322
0.64 0.0368940063805128
0.65 0.0376688412585836
0.66 0.0384578579539132
0.67 0.0392618884042034
0.68 0.0400818579909704
0.69 0.0409187657010436
0.7 0.041773691775908
0.71 0.0426478405802042
0.72 0.0435425240913562
0.73 0.0444591933668571
0.74 0.045399459223326
0.75 0.0463651035237027
0.76 0.047358122309387
0.77 0.0483807467895457
0.78 0.0494355055622706
0.79 0.0505252497091298
0.8 0.0516532396857553
0.81 0.0528231962544114
0.82 0.0540394465378803
0.83 0.0553069993438609
0.84 0.0566317398760401
0.85 0.0580206547482389
0.86 0.0594821017540228
0.87 0.0610262323086744
0.88 0.0626655186778564
0.89 0.0644155562769213
0.9 0.0662962123123682
0.91 0.0683334032925465
0.92 0.0705618182004098
0.93 0.0730294834156641
0.94 0.0758058267582037
0.95 0.0789968104959387
0.96 0.0827768252223982
0.97 0.0874660097502962
0.98 0.0937639966258074
0.99 0.103819405758584
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/ensemble-nerfacto/empirical_coverage.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.05, ymax=1.05,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 1
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.00514972046419918
0.02 0.00957189687434907
0.03 0.0139849664395896
0.04 0.0183963996311522
0.05 0.0228164118651269
0.06 0.0272545234852342
0.07 0.0317015768317575
0.08 0.0361389748022047
0.09 0.0405716474358511
0.1 0.0450040039085787
0.11 0.0494496609491184
0.12 0.0539032677335886
0.13 0.0583663437825241
0.14 0.0628357437332012
0.15 0.0673228922798875
0.16 0.0718233684051869
0.17 0.0763341544985184
0.18 0.0808640092645225
0.19 0.0854179721589666
0.2 0.0899859556022166
0.21 0.0945701242818803
0.22 0.099170844694465
0.23 0.103790227350875
0.24 0.108435083315768
0.25 0.113106379368118
0.26 0.117798818588339
0.27 0.122518540006513
0.28 0.12726568954385
0.29 0.13205249609329
0.3 0.136878005230422
0.31 0.14174641783404
0.32 0.146656532109747
0.33 0.151599579941323
0.34 0.156590072390149
0.35 0.161612056325091
0.36 0.166658732620591
0.37 0.171732131974471
0.38 0.176842860272932
0.39 0.181981949395233
0.4 0.187159253502274
0.41 0.192372589035253
0.42 0.197624596057323
0.43 0.202905630375113
0.44 0.208233062686095
0.45 0.213586996007092
0.46 0.218983325716342
0.47 0.224417349847141
0.48 0.229889455293083
0.49 0.235413249762097
0.5 0.240977860552103
0.51 0.246585721449489
0.52 0.252244916981667
0.53 0.257958155451828
0.54 0.263715569906043
0.55 0.269520945899726
0.56 0.275373863709365
0.57 0.281292184241793
0.58 0.287273652789607
0.59 0.293304310989997
0.6 0.299405784447249
0.61 0.305568182140023
0.62 0.311779959658465
0.63 0.318063859399004
0.64 0.324420026390632
0.65 0.330843760645111
0.66 0.337350976082116
0.67 0.343933135648118
0.68 0.350601834273765
0.69 0.357355980667405
0.7 0.364210139401828
0.71 0.371164237973601
0.72 0.37821635502024
0.73 0.385378825401182
0.74 0.392653547076979
0.75 0.400049852275378
0.76 0.407576320074773
0.77 0.415261033092959
0.78 0.423087679104365
0.79 0.431078905251101
0.8 0.439235170119458
0.81 0.447589811038805
0.82 0.456163196455146
0.83 0.464960044089794
0.84 0.474002413565108
0.85 0.483318190231673
0.86 0.492963417448295
0.87 0.502972646351636
0.88 0.513380623048889
0.89 0.524260974276533
0.9 0.535694588492163
0.91 0.547748664224325
0.92 0.560555570818419
0.93 0.574261505206403
0.94 0.589124351655039
0.95 0.605487935733514
0.96 0.62390429413079
0.97 0.6453533691957
0.98 0.671941538166984
0.99 0.709616403794751
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.00454040648744421
0.02 0.00901308005453672
0.03 0.0134802536304182
0.04 0.0179423187480904
0.05 0.0224113086082166
0.06 0.0268798001945331
0.07 0.0313542087993601
0.08 0.0358394637819534
0.09 0.0403204757819617
0.1 0.0448069646496126
0.11 0.049301204259888
0.12 0.0537980968965893
0.13 0.0583066456056919
0.14 0.0628303179382236
0.15 0.0673595357472
0.16 0.0719018878110433
0.17 0.0764651165307626
0.18 0.0810368090296656
0.19 0.0856178509835624
0.2 0.0902205873889982
0.21 0.0948398499746936
0.22 0.0994834591928309
0.23 0.104148080853261
0.24 0.108829595937047
0.25 0.113532613059346
0.26 0.118267081646307
0.27 0.123035319062389
0.28 0.127841002602548
0.29 0.132670331816525
0.3 0.137523236398134
0.31 0.142415160959064
0.32 0.147337135739588
0.33 0.152301387702162
0.34 0.157317326407654
0.35 0.162368871892939
0.36 0.167439254428536
0.37 0.172532338451325
0.38 0.177655683681974
0.39 0.182802765532062
0.4 0.187977399020985
0.41 0.19318244788199
0.42 0.198416139574958
0.43 0.203681441958787
0.44 0.208980900753552
0.45 0.214315837184074
0.46 0.219688980390285
0.47 0.225092415363461
0.48 0.230541095501517
0.49 0.236045187038397
0.5 0.241582857407427
0.51 0.247174826783083
0.52 0.252817084593454
0.53 0.258506930528236
0.54 0.264238909646385
0.55 0.270019724760013
0.56 0.275850672648937
0.57 0.281737695330031
0.58 0.287674686335712
0.59 0.29367463970106
0.6 0.299727960201224
0.61 0.305855226979504
0.62 0.312030308769429
0.63 0.318268221313336
0.64 0.324573933158485
0.65 0.330964760139753
0.66 0.337429309893878
0.67 0.343972004808534
0.68 0.350608970774802
0.69 0.357346484809532
0.7 0.364180247218743
0.71 0.371105726634586
0.72 0.378132893538297
0.73 0.385287835744454
0.74 0.392557980741587
0.75 0.399957537801295
0.76 0.407493755735729
0.77 0.41517172346323
0.78 0.423010527067941
0.79 0.431024639784576
0.8 0.439216072475314
0.81 0.447609237414749
0.82 0.456229766184914
0.83 0.465112524775444
0.84 0.474247191819686
0.85 0.483675288690656
0.86 0.493423832936657
0.87 0.50353262838585
0.88 0.514073757052431
0.89 0.52509893142005
0.9 0.536697415707181
0.91 0.548949737393941
0.92 0.562001519601959
0.93 0.576000249859102
0.94 0.591238414590127
0.95 0.608066885487932
0.96 0.627112413810078
0.97 0.64941843053515
0.98 0.677244112808315
0.99 0.716973672220943
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.00448116866362128
0.02 0.00890879038280557
0.03 0.0133298534858028
0.04 0.0177616983065374
0.05 0.0221911836538663
0.06 0.0266248050403633
0.07 0.0310788304678898
0.08 0.0355245998343839
0.09 0.0399764495517002
0.1 0.0444366554702719
0.11 0.0489071209056867
0.12 0.0533777905448664
0.13 0.0578647924305418
0.14 0.0623621981811098
0.15 0.066875996201631
0.16 0.0713987247617145
0.17 0.0759294385320284
0.18 0.080472399735596
0.19 0.0850274656007028
0.2 0.089615477864693
0.21 0.0942196998656384
0.22 0.0988327750950321
0.23 0.103462648902961
0.24 0.108114290263404
0.25 0.112796329174383
0.26 0.117495077952972
0.27 0.122217498767076
0.28 0.126965588676189
0.29 0.13173982822827
0.3 0.136541539549018
0.31 0.141376710092974
0.32 0.146237582714644
0.33 0.151136312511379
0.34 0.156065959760674
0.35 0.161053901628787
0.36 0.166067845569482
0.37 0.171104167065966
0.38 0.176169020150687
0.39 0.181262840771503
0.4 0.186382370747707
0.41 0.191522486419655
0.42 0.196684645976749
0.43 0.201883758951998
0.44 0.207106507064092
0.45 0.212364354919137
0.46 0.217656036716767
0.47 0.22298285361372
0.48 0.228349576345805
0.49 0.233753984754858
0.5 0.239203989928217
0.51 0.244702467137591
0.52 0.250240338831617
0.53 0.255829809606989
0.54 0.261467138670659
0.55 0.267148134747962
0.56 0.272882693163583
0.57 0.278670475909799
0.58 0.284506153685397
0.59 0.290409966788618
0.6 0.296364701822157
0.61 0.302388103048931
0.62 0.308472085447215
0.63 0.314627232284111
0.64 0.320848573591077
0.65 0.327151164514046
0.66 0.333530108699138
0.67 0.339988344200685
0.68 0.346527897852027
0.69 0.353165591255952
0.7 0.359895751083925
0.71 0.366725797985473
0.72 0.373657725781424
0.73 0.380711446830104
0.74 0.387878665585171
0.75 0.395176836023882
0.76 0.402609414870482
0.77 0.410195366346296
0.78 0.417939087990287
0.79 0.425860051312156
0.8 0.433968811028903
0.81 0.442280626090579
0.82 0.450813137591429
0.83 0.459604186724516
0.84 0.468653253790529
0.85 0.478002612417377
0.86 0.487680293518197
0.87 0.497734706283742
0.88 0.508222217030638
0.89 0.519198612061795
0.9 0.530745544788603
0.91 0.542965840660857
0.92 0.555987310181558
0.93 0.569991304536349
0.94 0.585232834078172
0.95 0.602085095637265
0.96 0.62116626765488
0.97 0.643544072839569
0.98 0.671468692564693
0.99 0.711457593657983
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.00413621718800848
0.02 0.00820105862274704
0.03 0.0122517044208561
0.04 0.0163092395344898
0.05 0.0203610459075896
0.06 0.0244116093639516
0.07 0.0284672606772703
0.08 0.0325264390745505
0.09 0.036592982163395
0.1 0.0406663869049609
0.11 0.0447436900119675
0.12 0.0488316513027286
0.13 0.0529303572566471
0.14 0.0570486032078746
0.15 0.0611622305399872
0.16 0.0652902882709955
0.17 0.0694276101865978
0.18 0.0735702607382604
0.19 0.0777279930505833
0.2 0.0818999677663908
0.21 0.0860852234909464
0.22 0.0902878287665866
0.23 0.094506059350547
0.24 0.0987435839899245
0.25 0.102992689801728
0.26 0.107268645384113
0.27 0.111564910884721
0.28 0.115880850241586
0.29 0.120218794578418
0.3 0.12458310553977
0.31 0.128968705725768
0.32 0.133370584800872
0.33 0.137788300963015
0.34 0.142241470879411
0.35 0.146736518501663
0.36 0.151247320038791
0.37 0.155782658886408
0.38 0.160350741666274
0.39 0.164936482642364
0.4 0.169542655034707
0.41 0.174171857690799
0.42 0.178829247526102
0.43 0.183518291630808
0.44 0.188228140302697
0.45 0.192970701135972
0.46 0.197755584288656
0.47 0.202564331803711
0.48 0.207419942809035
0.49 0.212305230457181
0.5 0.217229764451992
0.51 0.222193271750106
0.52 0.227208080511378
0.53 0.232265676808812
0.54 0.237362632166943
0.55 0.242505388090789
0.56 0.247706227096025
0.57 0.252955850360223
0.58 0.258258522742203
0.59 0.26361643522274
0.6 0.269025315690928
0.61 0.274498289686478
0.62 0.280032461895199
0.63 0.285636324748958
0.64 0.291308585688046
0.65 0.297052233670617
0.66 0.302866599364363
0.67 0.308770639519561
0.68 0.314751326813856
0.69 0.320836149221255
0.7 0.32700561918829
0.71 0.33327688603575
0.72 0.339657389523491
0.73 0.346142261078227
0.74 0.352748635075954
0.75 0.35949272976802
0.76 0.366375487195593
0.77 0.373396283980219
0.78 0.380585810693617
0.79 0.387949210425073
0.8 0.39550477240296
0.81 0.403260829717147
0.82 0.411255181501211
0.83 0.419501057203403
0.84 0.428022266040251
0.85 0.436835971424917
0.86 0.445999429017326
0.87 0.455545524666901
0.88 0.465522017196812
0.89 0.476008239239889
0.9 0.487082811272372
0.91 0.498839347807457
0.92 0.511424877783692
0.93 0.525045347591188
0.94 0.53993871118962
0.95 0.556541150307558
0.96 0.575506324437235
0.97 0.597952744680279
0.98 0.626336973004087
0.99 0.667652761678601
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/ensemble-nerfacto/empirical_coverage_absolute_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.0207238991401594, ymax=0.435201881943348,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.00605824535695551
0.02 0.0115374374575564
0.03 0.0170085427729624
0.04 0.0224710731450993
0.05 0.027921581561437
0.06 0.0333517478036259
0.07 0.0388109147206891
0.08 0.0443093827172256
0.09 0.0498118428287395
0.1 0.0553153481331567
0.11 0.0608050165703709
0.12 0.0662872254748165
0.13 0.0717616494300709
0.14 0.0772307382855853
0.15 0.0826840268202209
0.16 0.088176631594813
0.17 0.0936658455014816
0.18 0.0991359907354775
0.19 0.104582027841033
0.2 0.110014044397783
0.21 0.11542987571812
0.22 0.120829155305535
0.23 0.126209772649125
0.24 0.131564916684232
0.25 0.136893620631882
0.26 0.142201181411661
0.27 0.147481459993487
0.28 0.15273431045615
0.29 0.15794750390671
0.3 0.163121994769578
0.31 0.16825358216596
0.32 0.173343467890253
0.33 0.178400420058677
0.34 0.183409927609851
0.35 0.188387943674909
0.36 0.193341267379409
0.37 0.198267868025529
0.38 0.203157139727068
0.39 0.208018050604767
0.4 0.212840746497726
0.41 0.217627410964747
0.42 0.222375403942677
0.43 0.227094369624887
0.44 0.231766937313905
0.45 0.236413003992908
0.46 0.241016674283658
0.47 0.245582650152859
0.48 0.250110544706917
0.49 0.254586750237902
0.5 0.259022139447897
0.51 0.263414278550511
0.52 0.267755083018333
0.53 0.272041844548172
0.54 0.276284430093958
0.55 0.280479054100274
0.56 0.284626136290635
0.57 0.288707815758207
0.58 0.292726347210393
0.59 0.296695689010003
0.6 0.300594215552751
0.61 0.304431817859977
0.62 0.308220040341535
0.63 0.311936140600997
0.64 0.315579973609368
0.65 0.319156239354889
0.66 0.322649023917884
0.67 0.326066864351882
0.68 0.329398165726235
0.69 0.332644019332595
0.7 0.335789860598172
0.71 0.338835762026399
0.72 0.341783644979759
0.73 0.344621174598818
0.74 0.347346452923021
0.75 0.349950147724622
0.76 0.352423679925227
0.77 0.354738966907041
0.78 0.356912320895635
0.79 0.358921094748899
0.8 0.360764829880542
0.81 0.362410188961195
0.82 0.363836803544854
0.83 0.365039955910206
0.84 0.365997586434892
0.85 0.366681809768327
0.86 0.367036582551705
0.87 0.367027353648364
0.88 0.366619376951111
0.89 0.365739025723467
0.9 0.364305411507837
0.91 0.362251335775675
0.92 0.359444429181582
0.93 0.355738494793598
0.94 0.350875648344961
0.95 0.344512064266486
0.96 0.33609570586921
0.97 0.3246466308043
0.98 0.308058461833016
0.99 0.280383596205249
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.00558634435409334
0.02 0.0111049012864008
0.03 0.0166154166503031
0.04 0.0221228744762226
0.05 0.0276186981806633
0.06 0.0331201998054668
0.07 0.0386457912006398
0.08 0.0441605362180465
0.09 0.0496795242180383
0.1 0.0551930353503874
0.11 0.060698795740112
0.12 0.0662019031034106
0.13 0.0716933543943081
0.14 0.0771696820617765
0.15 0.0826404642528001
0.16 0.0880981121889566
0.17 0.0935348834692374
0.18 0.0989631909703344
0.19 0.104382149016438
0.2 0.109779412611002
0.21 0.115160150025306
0.22 0.120516540807169
0.23 0.125851919146739
0.24 0.131170404062953
0.25 0.136467386940654
0.26 0.141732918353693
0.27 0.146964680937611
0.28 0.152158997397452
0.29 0.157329668183475
0.3 0.162476763601866
0.31 0.167584839040936
0.32 0.172662864260412
0.33 0.177698612297838
0.34 0.182682673592346
0.35 0.187631128107061
0.36 0.192560745571463
0.37 0.197467661548675
0.38 0.202344316318026
0.39 0.207197234467938
0.4 0.212022600979016
0.41 0.21681755211801
0.42 0.221583860425042
0.43 0.226318558041213
0.44 0.231019099246448
0.45 0.235684162815926
0.46 0.240311019609715
0.47 0.244907584636539
0.48 0.249458904498483
0.49 0.253954812961603
0.5 0.258417142592573
0.51 0.262825173216917
0.52 0.267182915406546
0.53 0.271493069471764
0.54 0.275761090353615
0.55 0.279980275239987
0.56 0.284149327351064
0.57 0.288262304669969
0.58 0.292325313664288
0.59 0.29632536029894
0.6 0.300272039798776
0.61 0.304144773020496
0.62 0.307969691230571
0.63 0.311731778686664
0.64 0.315426066841515
0.65 0.319035239860247
0.66 0.322570690106122
0.67 0.326027995191466
0.68 0.329391029225198
0.69 0.332653515190468
0.7 0.335819752781257
0.71 0.338894273365414
0.72 0.341867106461703
0.73 0.344712164255546
0.74 0.347442019258413
0.75 0.350042462198705
0.76 0.352506244264271
0.77 0.35482827653677
0.78 0.356989472932059
0.79 0.358975360215424
0.8 0.360783927524686
0.81 0.362390762585251
0.82 0.363770233815086
0.83 0.364887475224556
0.84 0.365752808180314
0.85 0.366324711309344
0.86 0.366576167063343
0.87 0.36646737161415
0.88 0.365926242947569
0.89 0.36490106857995
0.9 0.363302584292819
0.91 0.361050262606059
0.92 0.357998480398041
0.93 0.353999750140898
0.94 0.348761585409873
0.95 0.341933114512068
0.96 0.332887586189922
0.97 0.32058156946485
0.98 0.302755887191686
0.99 0.273026327779056
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.00556119044097595
0.02 0.011092210653526
0.03 0.0166701465141973
0.04 0.0222383016934625
0.05 0.0278088163461336
0.06 0.0333751949596366
0.07 0.0389211695321102
0.08 0.044475400165616
0.09 0.0500235504482998
0.1 0.0555633445297281
0.11 0.0610928790943133
0.12 0.0666222094551336
0.13 0.0721352075694582
0.14 0.0776378018188902
0.15 0.083124003798369
0.16 0.0886012752382854
0.17 0.0940705614679715
0.18 0.0995276002644039
0.19 0.104972534399297
0.2 0.110384522135307
0.21 0.115780300134362
0.22 0.121167224904968
0.23 0.126537351097039
0.24 0.131885709736596
0.25 0.137203670825617
0.26 0.142504922047028
0.27 0.147782501232924
0.28 0.153034411323811
0.29 0.15826017177173
0.3 0.163458460450982
0.31 0.168623289907026
0.32 0.173762417285356
0.33 0.178863687488621
0.34 0.183934040239325
0.35 0.188946098371213
0.36 0.193932154430518
0.37 0.198895832934034
0.38 0.203830979849313
0.39 0.208737159228497
0.4 0.213617629252293
0.41 0.218477513580345
0.42 0.223315354023251
0.43 0.228116241048001
0.44 0.232893492935908
0.45 0.237635645080863
0.46 0.242343963283233
0.47 0.24701714638628
0.48 0.251650423654195
0.49 0.256246015245142
0.5 0.260796010071783
0.51 0.265297532862409
0.52 0.269759661168383
0.53 0.274170190393011
0.54 0.278532861329341
0.55 0.282851865252039
0.56 0.287117306836417
0.57 0.291329524090201
0.58 0.295493846314603
0.59 0.299590033211382
0.6 0.303635298177843
0.61 0.307611896951069
0.62 0.311527914552785
0.63 0.315372767715889
0.64 0.319151426408923
0.65 0.322848835485954
0.66 0.326469891300862
0.67 0.330011655799315
0.68 0.333472102147973
0.69 0.336834408744048
0.7 0.340104248916075
0.71 0.343274202014527
0.72 0.346342274218576
0.73 0.349288553169895
0.74 0.352121334414829
0.75 0.354823163976118
0.76 0.357390585129518
0.77 0.359804633653704
0.78 0.362060912009713
0.79 0.364139948687844
0.8 0.366031188971097
0.81 0.367719373909421
0.82 0.369186862408571
0.83 0.370395813275483
0.84 0.371346746209471
0.85 0.371997387582623
0.86 0.372319706481803
0.87 0.372265293716258
0.88 0.371777782969362
0.89 0.370801387938205
0.9 0.369254455211397
0.91 0.367034159339143
0.92 0.364012689818442
0.93 0.360008695463651
0.94 0.354767165921828
0.95 0.347914904362735
0.96 0.33883373234512
0.97 0.326455927160431
0.98 0.308531307435306
0.99 0.278542406342017
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.00591408585131414
0.02 0.0118325309812502
0.03 0.0177553130566718
0.04 0.0236907604655101
0.05 0.0296389540924103
0.06 0.0355883906360483
0.07 0.0415327393227296
0.08 0.0474735609254494
0.09 0.053407017836605
0.1 0.059333613095039
0.11 0.0652563099880324
0.12 0.0711683486972714
0.13 0.077069642743353
0.14 0.0829513967921255
0.15 0.0888377694600129
0.16 0.0947097117290045
0.17 0.100572389813402
0.18 0.10642973926174
0.19 0.112272006949417
0.2 0.118100032233609
0.21 0.123914776509054
0.22 0.129712171233413
0.23 0.135493940649453
0.24 0.141256416010075
0.25 0.147007310198272
0.26 0.152731354615887
0.27 0.158435089115279
0.28 0.164119149758414
0.29 0.169781205421582
0.3 0.17541689446023
0.31 0.181031294274232
0.32 0.186629415199128
0.33 0.192211699036985
0.34 0.197758529120589
0.35 0.203263481498336
0.36 0.208752679961209
0.37 0.214217341113592
0.38 0.219649258333726
0.39 0.225063517357636
0.4 0.230457344965293
0.41 0.235828142309201
0.42 0.241170752473898
0.43 0.246481708369192
0.44 0.251771859697303
0.45 0.257029298864028
0.46 0.262244415711344
0.47 0.267435668196289
0.48 0.272580057190965
0.49 0.277694769542819
0.5 0.282770235548008
0.51 0.287806728249894
0.52 0.292791919488622
0.53 0.297734323191188
0.54 0.302637367833058
0.55 0.307494611909211
0.56 0.312293772903976
0.57 0.317044149639777
0.58 0.321741477257797
0.59 0.32638356477726
0.6 0.330974684309072
0.61 0.335501710313522
0.62 0.339967538104802
0.63 0.344363675251042
0.64 0.348691414311954
0.65 0.352947766329383
0.66 0.357133400635637
0.67 0.361229360480439
0.68 0.365248673186144
0.69 0.369163850778745
0.7 0.37299438081171
0.71 0.376723113964251
0.72 0.380342610476509
0.73 0.383857738921773
0.74 0.387251364924046
0.75 0.39050727023198
0.76 0.393624512804407
0.77 0.396603716019781
0.78 0.399414189306383
0.79 0.402050789574927
0.8 0.404495227597039
0.81 0.406739170282853
0.82 0.408744818498789
0.83 0.410498942796597
0.84 0.411977733959749
0.85 0.413164028575083
0.86 0.414000570982674
0.87 0.414454475333099
0.88 0.414477982803188
0.89 0.413991760760111
0.9 0.412917188727629
0.91 0.411160652192543
0.92 0.408575122216308
0.93 0.404954652408812
0.94 0.40006128881038
0.95 0.393458849692442
0.96 0.384493675562765
0.97 0.372047255319721
0.98 0.353663026995913
0.99 0.322347238321399
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/ensemble-nerfacto/empirical_coverage_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.435201881943348, ymax=0.0207238991401594,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 -0.00485027953580083
0.02 -0.010428103125651
0.03 -0.0160150335604104
0.04 -0.0216036003688477
0.05 -0.027183588134873
0.06 -0.0327454765147657
0.07 -0.0382984231682425
0.08 -0.0438610251977953
0.09 -0.0494283525641488
0.1 -0.0549959960914213
0.11 -0.0605503390508816
0.12 -0.0660967322664114
0.13 -0.0716336562174759
0.14 -0.0771642562667988
0.15 -0.0826771077201126
0.16 -0.088176631594813
0.17 -0.0936658455014816
0.18 -0.0991359907354775
0.19 -0.104582027841033
0.2 -0.110014044397783
0.21 -0.11542987571812
0.22 -0.120829155305535
0.23 -0.126209772649125
0.24 -0.131564916684232
0.25 -0.136893620631882
0.26 -0.142201181411661
0.27 -0.147481459993487
0.28 -0.15273431045615
0.29 -0.15794750390671
0.3 -0.163121994769578
0.31 -0.16825358216596
0.32 -0.173343467890253
0.33 -0.178400420058677
0.34 -0.183409927609851
0.35 -0.188387943674909
0.36 -0.193341267379409
0.37 -0.198267868025529
0.38 -0.203157139727068
0.39 -0.208018050604767
0.4 -0.212840746497726
0.41 -0.217627410964747
0.42 -0.222375403942677
0.43 -0.227094369624887
0.44 -0.231766937313905
0.45 -0.236413003992908
0.46 -0.241016674283658
0.47 -0.245582650152859
0.48 -0.250110544706917
0.49 -0.254586750237902
0.5 -0.259022139447897
0.51 -0.263414278550511
0.52 -0.267755083018333
0.53 -0.272041844548172
0.54 -0.276284430093958
0.55 -0.280479054100274
0.56 -0.284626136290635
0.57 -0.288707815758207
0.58 -0.292726347210393
0.59 -0.296695689010003
0.6 -0.300594215552751
0.61 -0.304431817859977
0.62 -0.308220040341535
0.63 -0.311936140600997
0.64 -0.315579973609368
0.65 -0.319156239354889
0.66 -0.322649023917884
0.67 -0.326066864351882
0.68 -0.329398165726235
0.69 -0.332644019332595
0.7 -0.335789860598172
0.71 -0.338835762026399
0.72 -0.341783644979759
0.73 -0.344621174598818
0.74 -0.347346452923021
0.75 -0.349950147724622
0.76 -0.352423679925227
0.77 -0.354738966907041
0.78 -0.356912320895635
0.79 -0.358921094748899
0.8 -0.360764829880542
0.81 -0.362410188961195
0.82 -0.363836803544854
0.83 -0.365039955910206
0.84 -0.365997586434892
0.85 -0.366681809768327
0.86 -0.367036582551705
0.87 -0.367027353648364
0.88 -0.366619376951111
0.89 -0.365739025723467
0.9 -0.364305411507837
0.91 -0.362251335775675
0.92 -0.359444429181582
0.93 -0.355738494793598
0.94 -0.350875648344961
0.95 -0.344512064266486
0.96 -0.33609570586921
0.97 -0.3246466308043
0.98 -0.308058461833016
0.99 -0.280383596205249
};
\addplot [semithick, darkorange25512714]
table {%
0.01 -0.0054595935125558
0.02 -0.0109869199454633
0.03 -0.0165197463695818
0.04 -0.0220576812519095
0.05 -0.0275886913917834
0.06 -0.0331201998054668
0.07 -0.0386457912006398
0.08 -0.0441605362180465
0.09 -0.0496795242180383
0.1 -0.0551930353503874
0.11 -0.060698795740112
0.12 -0.0662019031034106
0.13 -0.0716933543943081
0.14 -0.0771696820617765
0.15 -0.0826404642528001
0.16 -0.0880981121889566
0.17 -0.0935348834692374
0.18 -0.0989631909703344
0.19 -0.104382149016438
0.2 -0.109779412611002
0.21 -0.115160150025306
0.22 -0.120516540807169
0.23 -0.125851919146739
0.24 -0.131170404062953
0.25 -0.136467386940654
0.26 -0.141732918353693
0.27 -0.146964680937611
0.28 -0.152158997397452
0.29 -0.157329668183475
0.3 -0.162476763601866
0.31 -0.167584839040936
0.32 -0.172662864260412
0.33 -0.177698612297838
0.34 -0.182682673592346
0.35 -0.187631128107061
0.36 -0.192560745571463
0.37 -0.197467661548675
0.38 -0.202344316318026
0.39 -0.207197234467938
0.4 -0.212022600979016
0.41 -0.21681755211801
0.42 -0.221583860425042
0.43 -0.226318558041213
0.44 -0.231019099246448
0.45 -0.235684162815926
0.46 -0.240311019609715
0.47 -0.244907584636539
0.48 -0.249458904498483
0.49 -0.253954812961603
0.5 -0.258417142592573
0.51 -0.262825173216917
0.52 -0.267182915406546
0.53 -0.271493069471764
0.54 -0.275761090353615
0.55 -0.279980275239987
0.56 -0.284149327351064
0.57 -0.288262304669969
0.58 -0.292325313664288
0.59 -0.29632536029894
0.6 -0.300272039798776
0.61 -0.304144773020496
0.62 -0.307969691230571
0.63 -0.311731778686664
0.64 -0.315426066841515
0.65 -0.319035239860247
0.66 -0.322570690106122
0.67 -0.326027995191466
0.68 -0.329391029225198
0.69 -0.332653515190468
0.7 -0.335819752781257
0.71 -0.338894273365414
0.72 -0.341867106461703
0.73 -0.344712164255546
0.74 -0.347442019258413
0.75 -0.350042462198705
0.76 -0.352506244264271
0.77 -0.35482827653677
0.78 -0.356989472932059
0.79 -0.358975360215424
0.8 -0.360783927524686
0.81 -0.362390762585251
0.82 -0.363770233815086
0.83 -0.364887475224556
0.84 -0.365752808180314
0.85 -0.366324711309344
0.86 -0.366576167063343
0.87 -0.36646737161415
0.88 -0.365926242947569
0.89 -0.36490106857995
0.9 -0.363302584292819
0.91 -0.361050262606059
0.92 -0.357998480398041
0.93 -0.353999750140898
0.94 -0.348761585409873
0.95 -0.341933114512068
0.96 -0.332887586189922
0.97 -0.32058156946485
0.98 -0.302755887191686
0.99 -0.273026327779056
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 -0.00551883133637873
0.02 -0.0110912096171945
0.03 -0.0166701465141973
0.04 -0.0222383016934625
0.05 -0.0278088163461336
0.06 -0.0333751949596366
0.07 -0.0389211695321102
0.08 -0.044475400165616
0.09 -0.0500235504482998
0.1 -0.0555633445297281
0.11 -0.0610928790943133
0.12 -0.0666222094551336
0.13 -0.0721352075694582
0.14 -0.0776378018188902
0.15 -0.083124003798369
0.16 -0.0886012752382854
0.17 -0.0940705614679715
0.18 -0.0995276002644039
0.19 -0.104972534399297
0.2 -0.110384522135307
0.21 -0.115780300134362
0.22 -0.121167224904968
0.23 -0.126537351097039
0.24 -0.131885709736596
0.25 -0.137203670825617
0.26 -0.142504922047028
0.27 -0.147782501232924
0.28 -0.153034411323811
0.29 -0.15826017177173
0.3 -0.163458460450982
0.31 -0.168623289907026
0.32 -0.173762417285356
0.33 -0.178863687488621
0.34 -0.183934040239325
0.35 -0.188946098371213
0.36 -0.193932154430518
0.37 -0.198895832934034
0.38 -0.203830979849313
0.39 -0.208737159228497
0.4 -0.213617629252293
0.41 -0.218477513580345
0.42 -0.223315354023251
0.43 -0.228116241048001
0.44 -0.232893492935908
0.45 -0.237635645080863
0.46 -0.242343963283233
0.47 -0.24701714638628
0.48 -0.251650423654195
0.49 -0.256246015245142
0.5 -0.260796010071783
0.51 -0.265297532862409
0.52 -0.269759661168383
0.53 -0.274170190393011
0.54 -0.278532861329341
0.55 -0.282851865252039
0.56 -0.287117306836417
0.57 -0.291329524090201
0.58 -0.295493846314603
0.59 -0.299590033211382
0.6 -0.303635298177843
0.61 -0.307611896951069
0.62 -0.311527914552785
0.63 -0.315372767715889
0.64 -0.319151426408923
0.65 -0.322848835485954
0.66 -0.326469891300862
0.67 -0.330011655799315
0.68 -0.333472102147973
0.69 -0.336834408744048
0.7 -0.340104248916075
0.71 -0.343274202014527
0.72 -0.346342274218576
0.73 -0.349288553169895
0.74 -0.352121334414829
0.75 -0.354823163976118
0.76 -0.357390585129518
0.77 -0.359804633653704
0.78 -0.362060912009713
0.79 -0.364139948687844
0.8 -0.366031188971097
0.81 -0.367719373909421
0.82 -0.369186862408571
0.83 -0.370395813275483
0.84 -0.371346746209471
0.85 -0.371997387582623
0.86 -0.372319706481803
0.87 -0.372265293716258
0.88 -0.371777782969362
0.89 -0.370801387938205
0.9 -0.369254455211397
0.91 -0.367034159339143
0.92 -0.364012689818442
0.93 -0.360008695463651
0.94 -0.354767165921828
0.95 -0.347914904362735
0.96 -0.33883373234512
0.97 -0.326455927160431
0.98 -0.308531307435306
0.99 -0.278542406342017
};
\addplot [semithick, crimson2143940]
table {%
0.01 -0.00586378281199153
0.02 -0.011798941377253
0.03 -0.0177482955791439
0.04 -0.0236907604655101
0.05 -0.0296389540924103
0.06 -0.0355883906360483
0.07 -0.0415327393227296
0.08 -0.0474735609254494
0.09 -0.053407017836605
0.1 -0.059333613095039
0.11 -0.0652563099880324
0.12 -0.0711683486972714
0.13 -0.077069642743353
0.14 -0.0829513967921255
0.15 -0.0888377694600129
0.16 -0.0947097117290045
0.17 -0.100572389813402
0.18 -0.10642973926174
0.19 -0.112272006949417
0.2 -0.118100032233609
0.21 -0.123914776509054
0.22 -0.129712171233413
0.23 -0.135493940649453
0.24 -0.141256416010075
0.25 -0.147007310198272
0.26 -0.152731354615887
0.27 -0.158435089115279
0.28 -0.164119149758414
0.29 -0.169781205421582
0.3 -0.17541689446023
0.31 -0.181031294274232
0.32 -0.186629415199128
0.33 -0.192211699036985
0.34 -0.197758529120589
0.35 -0.203263481498336
0.36 -0.208752679961209
0.37 -0.214217341113592
0.38 -0.219649258333726
0.39 -0.225063517357636
0.4 -0.230457344965293
0.41 -0.235828142309201
0.42 -0.241170752473898
0.43 -0.246481708369192
0.44 -0.251771859697303
0.45 -0.257029298864028
0.46 -0.262244415711344
0.47 -0.267435668196289
0.48 -0.272580057190965
0.49 -0.277694769542819
0.5 -0.282770235548008
0.51 -0.287806728249894
0.52 -0.292791919488622
0.53 -0.297734323191188
0.54 -0.302637367833058
0.55 -0.307494611909211
0.56 -0.312293772903976
0.57 -0.317044149639777
0.58 -0.321741477257797
0.59 -0.32638356477726
0.6 -0.330974684309072
0.61 -0.335501710313522
0.62 -0.339967538104802
0.63 -0.344363675251042
0.64 -0.348691414311954
0.65 -0.352947766329383
0.66 -0.357133400635637
0.67 -0.361229360480439
0.68 -0.365248673186144
0.69 -0.369163850778745
0.7 -0.37299438081171
0.71 -0.376723113964251
0.72 -0.380342610476509
0.73 -0.383857738921773
0.74 -0.387251364924046
0.75 -0.39050727023198
0.76 -0.393624512804407
0.77 -0.396603716019781
0.78 -0.399414189306383
0.79 -0.402050789574927
0.8 -0.404495227597039
0.81 -0.406739170282853
0.82 -0.408744818498789
0.83 -0.410498942796597
0.84 -0.411977733959749
0.85 -0.413164028575083
0.86 -0.414000570982674
0.87 -0.414454475333099
0.88 -0.414477982803188
0.89 -0.413991760760111
0.9 -0.412917188727629
0.91 -0.411160652192543
0.92 -0.408575122216308
0.93 -0.404954652408812
0.94 -0.40006128881038
0.95 -0.393458849692442
0.96 -0.384493675562765
0.97 -0.372047255319721
0.98 -0.353663026995913
0.99 -0.322347238321399
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/ensemble-nerfacto/empirical_coverage_negative_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.0207238991401594, ymax=0.435201881943348,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.00545426244637817
0.02 0.0109827702916037
0.03 0.0165117881666864
0.04 0.0220373367569735
0.05 0.027552584848155
0.06 0.0330486121591958
0.07 0.0385546689444658
0.08 0.0440852039575104
0.09 0.0496200976964442
0.1 0.055155672112289
0.11 0.0606776778106263
0.12 0.0661919788706139
0.13 0.0716976528237734
0.14 0.0771974972761921
0.15 0.0826805672701667
0.16 0.088176631594813
0.17 0.0936658455014816
0.18 0.0991359907354775
0.19 0.104582027841033
0.2 0.110014044397783
0.21 0.11542987571812
0.22 0.120829155305535
0.23 0.126209772649125
0.24 0.131564916684232
0.25 0.136893620631882
0.26 0.142201181411661
0.27 0.147481459993487
0.28 0.15273431045615
0.29 0.15794750390671
0.3 0.163121994769578
0.31 0.16825358216596
0.32 0.173343467890253
0.33 0.178400420058677
0.34 0.183409927609851
0.35 0.188387943674909
0.36 0.193341267379409
0.37 0.198267868025529
0.38 0.203157139727068
0.39 0.208018050604767
0.4 0.212840746497726
0.41 0.217627410964747
0.42 0.222375403942677
0.43 0.227094369624887
0.44 0.231766937313905
0.45 0.236413003992908
0.46 0.241016674283658
0.47 0.245582650152859
0.48 0.250110544706917
0.49 0.254586750237902
0.5 0.259022139447897
0.51 0.263414278550511
0.52 0.267755083018333
0.53 0.272041844548172
0.54 0.276284430093958
0.55 0.280479054100274
0.56 0.284626136290635
0.57 0.288707815758207
0.58 0.292726347210393
0.59 0.296695689010003
0.6 0.300594215552751
0.61 0.304431817859977
0.62 0.308220040341535
0.63 0.311936140600997
0.64 0.315579973609368
0.65 0.319156239354889
0.66 0.322649023917884
0.67 0.326066864351882
0.68 0.329398165726235
0.69 0.332644019332595
0.7 0.335789860598172
0.71 0.338835762026399
0.72 0.341783644979759
0.73 0.344621174598818
0.74 0.347346452923021
0.75 0.349950147724622
0.76 0.352423679925227
0.77 0.354738966907041
0.78 0.356912320895635
0.79 0.358921094748899
0.8 0.360764829880542
0.81 0.362410188961195
0.82 0.363836803544854
0.83 0.365039955910206
0.84 0.365997586434892
0.85 0.366681809768327
0.86 0.367036582551705
0.87 0.367027353648364
0.88 0.366619376951111
0.89 0.365739025723467
0.9 0.364305411507837
0.91 0.362251335775675
0.92 0.359444429181582
0.93 0.355738494793598
0.94 0.350875648344961
0.95 0.344512064266486
0.96 0.33609570586921
0.97 0.3246466308043
0.98 0.308058461833016
0.99 0.280383596205249
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.00552296893332457
0.02 0.0110459106159321
0.03 0.0165675815099425
0.04 0.0220902778640661
0.05 0.0276036947862233
0.06 0.0331201998054668
0.07 0.0386457912006398
0.08 0.0441605362180465
0.09 0.0496795242180383
0.1 0.0551930353503874
0.11 0.060698795740112
0.12 0.0662019031034106
0.13 0.0716933543943081
0.14 0.0771696820617765
0.15 0.0826404642528001
0.16 0.0880981121889566
0.17 0.0935348834692374
0.18 0.0989631909703344
0.19 0.104382149016438
0.2 0.109779412611002
0.21 0.115160150025306
0.22 0.120516540807169
0.23 0.125851919146739
0.24 0.131170404062953
0.25 0.136467386940654
0.26 0.141732918353693
0.27 0.146964680937611
0.28 0.152158997397452
0.29 0.157329668183475
0.3 0.162476763601866
0.31 0.167584839040936
0.32 0.172662864260412
0.33 0.177698612297838
0.34 0.182682673592346
0.35 0.187631128107061
0.36 0.192560745571463
0.37 0.197467661548675
0.38 0.202344316318026
0.39 0.207197234467938
0.4 0.212022600979016
0.41 0.21681755211801
0.42 0.221583860425042
0.43 0.226318558041213
0.44 0.231019099246448
0.45 0.235684162815926
0.46 0.240311019609715
0.47 0.244907584636539
0.48 0.249458904498483
0.49 0.253954812961603
0.5 0.258417142592573
0.51 0.262825173216917
0.52 0.267182915406546
0.53 0.271493069471764
0.54 0.275761090353615
0.55 0.279980275239987
0.56 0.284149327351064
0.57 0.288262304669969
0.58 0.292325313664288
0.59 0.29632536029894
0.6 0.300272039798776
0.61 0.304144773020496
0.62 0.307969691230571
0.63 0.311731778686664
0.64 0.315426066841515
0.65 0.319035239860247
0.66 0.322570690106122
0.67 0.326027995191466
0.68 0.329391029225198
0.69 0.332653515190468
0.7 0.335819752781257
0.71 0.338894273365414
0.72 0.341867106461703
0.73 0.344712164255546
0.74 0.347442019258413
0.75 0.350042462198705
0.76 0.352506244264271
0.77 0.35482827653677
0.78 0.356989472932059
0.79 0.358975360215424
0.8 0.360783927524686
0.81 0.362390762585251
0.82 0.363770233815086
0.83 0.364887475224556
0.84 0.365752808180314
0.85 0.366324711309344
0.86 0.366576167063343
0.87 0.36646737161415
0.88 0.365926242947569
0.89 0.36490106857995
0.9 0.363302584292819
0.91 0.361050262606059
0.92 0.357998480398041
0.93 0.353999750140898
0.94 0.348761585409873
0.95 0.341933114512068
0.96 0.332887586189922
0.97 0.32058156946485
0.98 0.302755887191686
0.99 0.273026327779056
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.00554001088867734
0.02 0.0110917101353602
0.03 0.0166701465141973
0.04 0.0222383016934625
0.05 0.0278088163461336
0.06 0.0333751949596366
0.07 0.0389211695321102
0.08 0.044475400165616
0.09 0.0500235504482998
0.1 0.0555633445297281
0.11 0.0610928790943133
0.12 0.0666222094551336
0.13 0.0721352075694582
0.14 0.0776378018188902
0.15 0.083124003798369
0.16 0.0886012752382854
0.17 0.0940705614679715
0.18 0.0995276002644039
0.19 0.104972534399297
0.2 0.110384522135307
0.21 0.115780300134362
0.22 0.121167224904968
0.23 0.126537351097039
0.24 0.131885709736596
0.25 0.137203670825617
0.26 0.142504922047028
0.27 0.147782501232924
0.28 0.153034411323811
0.29 0.15826017177173
0.3 0.163458460450982
0.31 0.168623289907026
0.32 0.173762417285356
0.33 0.178863687488621
0.34 0.183934040239325
0.35 0.188946098371213
0.36 0.193932154430518
0.37 0.198895832934034
0.38 0.203830979849313
0.39 0.208737159228497
0.4 0.213617629252293
0.41 0.218477513580345
0.42 0.223315354023251
0.43 0.228116241048001
0.44 0.232893492935908
0.45 0.237635645080863
0.46 0.242343963283233
0.47 0.24701714638628
0.48 0.251650423654195
0.49 0.256246015245142
0.5 0.260796010071783
0.51 0.265297532862409
0.52 0.269759661168383
0.53 0.274170190393011
0.54 0.278532861329341
0.55 0.282851865252039
0.56 0.287117306836417
0.57 0.291329524090201
0.58 0.295493846314603
0.59 0.299590033211382
0.6 0.303635298177843
0.61 0.307611896951069
0.62 0.311527914552785
0.63 0.315372767715889
0.64 0.319151426408923
0.65 0.322848835485954
0.66 0.326469891300862
0.67 0.330011655799315
0.68 0.333472102147973
0.69 0.336834408744048
0.7 0.340104248916075
0.71 0.343274202014527
0.72 0.346342274218576
0.73 0.349288553169895
0.74 0.352121334414829
0.75 0.354823163976118
0.76 0.357390585129518
0.77 0.359804633653704
0.78 0.362060912009713
0.79 0.364139948687844
0.8 0.366031188971097
0.81 0.367719373909421
0.82 0.369186862408571
0.83 0.370395813275483
0.84 0.371346746209471
0.85 0.371997387582623
0.86 0.372319706481803
0.87 0.372265293716258
0.88 0.371777782969362
0.89 0.370801387938205
0.9 0.369254455211397
0.91 0.367034159339143
0.92 0.364012689818442
0.93 0.360008695463651
0.94 0.354767165921828
0.95 0.347914904362735
0.96 0.33883373234512
0.97 0.326455927160431
0.98 0.308531307435306
0.99 0.278542406342017
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.00588893433165284
0.02 0.0118157361792516
0.03 0.0177518043179079
0.04 0.0236907604655101
0.05 0.0296389540924103
0.06 0.0355883906360483
0.07 0.0415327393227296
0.08 0.0474735609254494
0.09 0.053407017836605
0.1 0.059333613095039
0.11 0.0652563099880324
0.12 0.0711683486972714
0.13 0.077069642743353
0.14 0.0829513967921255
0.15 0.0888377694600129
0.16 0.0947097117290045
0.17 0.100572389813402
0.18 0.10642973926174
0.19 0.112272006949417
0.2 0.118100032233609
0.21 0.123914776509054
0.22 0.129712171233413
0.23 0.135493940649453
0.24 0.141256416010075
0.25 0.147007310198272
0.26 0.152731354615887
0.27 0.158435089115279
0.28 0.164119149758414
0.29 0.169781205421582
0.3 0.17541689446023
0.31 0.181031294274232
0.32 0.186629415199128
0.33 0.192211699036985
0.34 0.197758529120589
0.35 0.203263481498336
0.36 0.208752679961209
0.37 0.214217341113592
0.38 0.219649258333726
0.39 0.225063517357636
0.4 0.230457344965293
0.41 0.235828142309201
0.42 0.241170752473898
0.43 0.246481708369192
0.44 0.251771859697303
0.45 0.257029298864028
0.46 0.262244415711344
0.47 0.267435668196289
0.48 0.272580057190965
0.49 0.277694769542819
0.5 0.282770235548008
0.51 0.287806728249894
0.52 0.292791919488622
0.53 0.297734323191188
0.54 0.302637367833058
0.55 0.307494611909211
0.56 0.312293772903976
0.57 0.317044149639777
0.58 0.321741477257797
0.59 0.32638356477726
0.6 0.330974684309072
0.61 0.335501710313522
0.62 0.339967538104802
0.63 0.344363675251042
0.64 0.348691414311954
0.65 0.352947766329383
0.66 0.357133400635637
0.67 0.361229360480439
0.68 0.365248673186144
0.69 0.369163850778745
0.7 0.37299438081171
0.71 0.376723113964251
0.72 0.380342610476509
0.73 0.383857738921773
0.74 0.387251364924046
0.75 0.39050727023198
0.76 0.393624512804407
0.77 0.396603716019781
0.78 0.399414189306383
0.79 0.402050789574927
0.8 0.404495227597039
0.81 0.406739170282853
0.82 0.408744818498789
0.83 0.410498942796597
0.84 0.411977733959749
0.85 0.413164028575083
0.86 0.414000570982674
0.87 0.414454475333099
0.88 0.414477982803188
0.89 0.413991760760111
0.9 0.412917188727629
0.91 0.411160652192543
0.92 0.408575122216308
0.93 0.404954652408812
0.94 0.40006128881038
0.95 0.393458849692442
0.96 0.384493675562765
0.97 0.372047255319721
0.98 0.353663026995913
0.99 0.322347238321399
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/ensemble-splatfacto/avg_length.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.039, xmax=1.039,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.0239020043699017, ymax=0.516354462873606,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.01 0.00239298735451606
0.02 0.00478635106396381
0.03 0.00718046723450307
0.04 0.00957571217655985
0.05 0.0119724648722113
0.06 0.0143711071769639
0.07 0.0167720199439722
0.08 0.0191755873556129
0.09 0.0215821967675666
0.1 0.0239922406372817
0.11 0.0264061141348215
0.12 0.0288242176211431
0.13 0.0312469505030967
0.14 0.033674726632426
0.15 0.0361079603315975
0.16 0.0385470738402902
0.17 0.0409924913116767
0.18 0.0434446561030254
0.19 0.0459040074681016
0.2 0.0483709978329047
0.21 0.0508460878538657
0.22 0.0533297637507434
0.23 0.0558224902617679
0.24 0.0583247627529547
0.25 0.0608371038492007
0.26 0.0633600196526008
0.27 0.0658940484888135
0.28 0.0684397397622431
0.29 0.0709976578055023
0.3 0.0735683751140479
0.31 0.0761525105351648
0.32 0.0787506685181353
0.33 0.0813634854678424
0.34 0.0839916410029137
0.35 0.0866358106066438
0.36 0.0892966977638697
0.37 0.0919750369368688
0.38 0.0946716013228697
0.39 0.0973871892613782
0.4 0.100122627115107
0.41 0.102878754309567
0.42 0.105656512035849
0.43 0.108456810154975
0.44 0.111280632624202
0.45 0.114129016459121
0.46 0.117003018718899
0.47 0.119903791905438
0.48 0.122832511949556
0.49 0.125790412256844
0.5 0.128778822614863
0.51 0.131799125663399
0.52 0.134852786539445
0.53 0.137941316485651
0.54 0.141066380467959
0.55 0.144229710990106
0.56 0.147433132592066
0.57 0.150678605465849
0.58 0.153968213425142
0.59 0.157304177448335
0.6 0.160688861353708
0.61 0.164124828679202
0.62 0.167614787012743
0.63 0.171161658513219
0.64 0.174768618791843
0.65 0.178439051859922
0.66 0.182176655491594
0.67 0.185985390809733
0.68 0.189869633969746
0.69 0.19383409071477
0.7 0.197883914737875
0.71 0.202024793989987
0.72 0.206262955877436
0.73 0.210605277936928
0.74 0.215059355531172
0.75 0.219633640286597
0.76 0.224337615206097
0.77 0.229181848944046
0.78 0.234178295006197
0.79 0.239340462950535
0.8 0.244683786911804
0.81 0.250225941585941
0.82 0.255987362015162
0.83 0.261991826561915
0.84 0.268267185289631
0.85 0.27484653191655
0.86 0.281769493713448
0.87 0.289084092513821
0.88 0.296849456553978
0.89 0.305139445148101
0.9 0.314048237343957
0.91 0.32369851576664
0.92 0.334254594382939
0.93 0.345944068749852
0.94 0.359095725972654
0.95 0.374211569257834
0.96 0.392117689421918
0.97 0.414330544760807
0.98 0.444164415913414
0.99 0.491797350726174
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.00145981087224249
0.02 0.00291985120357757
0.03 0.00438035050876197
0.04 0.00584153879067095
0.05 0.00730364716696042
0.06 0.00876690757870197
0.07 0.010231553032668
0.08 0.0116978177686392
0.09 0.0131659390739715
0.1 0.0146361547193154
0.11 0.0161087077886502
0.12 0.017583840368224
0.13 0.0190617962812943
0.14 0.0205428310552623
0.15 0.0220271927172242
0.16 0.023515141261805
0.17 0.0250069380864577
0.18 0.0265028496012893
0.19 0.0280031444980524
0.2 0.0295081001151176
0.21 0.031017997748935
0.22 0.0325331318419813
0.23 0.0340537861141172
0.24 0.0355802646503323
0.25 0.0371128838179473
0.26 0.0386519602234254
0.27 0.0401978084620495
0.28 0.0417507749940663
0.29 0.0433112024422755
0.3 0.0448794364671933
0.31 0.0464558492516009
0.32 0.0480408250559081
0.33 0.0496347417039906
0.34 0.0512380101229308
0.35 0.0528510498597522
0.36 0.0544742857964291
0.37 0.0561081761336526
0.38 0.0577531825138411
0.39 0.0594097925817987
0.4 0.0610785124822864
0.41 0.0627598529854262
0.42 0.0644543841822179
0.43 0.0661626717759439
0.44 0.0678853064823516
0.45 0.0696229262008014
0.46 0.0713761725126553
0.47 0.0731457538854542
0.48 0.0749323786859799
0.49 0.0767368064128395
0.5 0.0785598522060705
0.51 0.0804023447895601
0.52 0.0822651863852063
0.53 0.0841493106196155
0.54 0.0860557152391619
0.55 0.087985461276655
0.56 0.0899396716107603
0.57 0.0919195344225148
0.58 0.093926310773522
0.59 0.0959613677221092
0.6 0.0980261541995546
0.61 0.100122223632206
0.62 0.102251223053145
0.63 0.104414957938925
0.64 0.106615327833416
0.65 0.10885442592642
0.66 0.111134502019091
0.67 0.113457981999511
0.68 0.115827508523693
0.69 0.118245967207
0.7 0.120716513710846
0.71 0.12324260731766
0.72 0.125828039228836
0.73 0.12847701591216
0.74 0.13119417695409
0.75 0.133984650575849
0.76 0.13685425364951
0.77 0.139809409473613
0.78 0.142857435600967
0.79 0.146006546588804
0.8 0.149266174575853
0.81 0.15264709283742
0.82 0.156161773884791
0.83 0.159824707039211
0.84 0.163652923134275
0.85 0.16766657177282
0.86 0.171889827374702
0.87 0.176352003318019
0.88 0.181089160682715
0.89 0.186146372688437
0.9 0.191581049829293
0.91 0.197468077797861
0.92 0.203907678957203
0.93 0.211038688450285
0.94 0.219061691484012
0.95 0.228282910524851
0.96 0.239206317230698
0.97 0.252756961761014
0.98 0.270956740320828
0.99 0.300014598142249
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.000968120686550816
0.02 0.00193639367351022
0.03 0.00290497087008355
0.04 0.00387400505792078
0.05 0.0048436491907097
0.06 0.00581405791642025
0.07 0.00678538438281916
0.08 0.00775778587185797
0.09 0.00873141762428445
0.1 0.00970643829231935
0.11 0.0106830090441795
0.12 0.0116612902630223
0.13 0.0126414459638205
0.14 0.0136236405125217
0.15 0.014608043953522
0.16 0.0155948248274366
0.17 0.0165841582165957
0.18 0.0175762194275808
0.19 0.0185711888057419
0.2 0.0195692492053154
0.21 0.0205705851315708
0.22 0.0215753958705244
0.23 0.0225838676088971
0.24 0.0235962019185111
0.25 0.0246126095901786
0.26 0.0256332952093271
0.27 0.026658475046423
0.28 0.0276883739782793
0.29 0.0287232198918741
0.3 0.0297632460823199
0.31 0.0308086958380796
0.32 0.0318598235310528
0.33 0.0329168826439298
0.34 0.0339801367849158
0.35 0.035049879127834
0.36 0.0361263848451461
0.37 0.0372099475190802
0.38 0.0383008881633508
0.39 0.0393995229126678
0.4 0.040506184202261
0.41 0.0416212218263763
0.42 0.0427450057082023
0.43 0.0438779098552966
0.44 0.045020331381474
0.45 0.0461726884286717
0.46 0.0473354130568773
0.47 0.0485089677983074
0.48 0.0496938216729294
0.49 0.0508904907192108
0.5 0.0520995009390694
0.51 0.0533214109074679
0.52 0.0545568149664773
0.53 0.0558063322023626
0.54 0.0570706258845368
0.55 0.0583503962095237
0.56 0.0596463929418674
0.57 0.06095939819108
0.58 0.0622902657308018
0.59 0.0636398796286808
0.6 0.0650092065595024
0.61 0.0663992836258894
0.62 0.0678112033434354
0.63 0.0692461467827095
0.64 0.0707053995052176
0.65 0.0721903283532443
0.66 0.0737024305904873
0.67 0.0752433194999853
0.68 0.0768147528113419
0.69 0.0784186339416729
0.7 0.0800570553537697
0.71 0.0817323121707521
0.72 0.083446924373778
0.73 0.0852036776622171
0.74 0.0870056462269285
0.75 0.0888562443142756
0.76 0.0907593222428736
0.77 0.0927191264600034
0.78 0.0947405154803716
0.79 0.0968289511820659
0.8 0.098990678954155
0.81 0.101232850549313
0.82 0.103563721149184
0.83 0.105992918567122
0.84 0.108531719064529
0.85 0.11119349413474
0.86 0.113994280056273
0.87 0.116953523647175
0.88 0.120095121336662
0.89 0.123448979603005
0.9 0.127053158077882
0.91 0.130957322796936
0.92 0.135227962230564
0.93 0.139957118049573
0.94 0.145277830616038
0.95 0.151393184817061
0.96 0.15863738266967
0.97 0.167623942741457
0.98 0.179693703410492
0.99 0.198964361179378
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.000655107777530448
0.02 0.00131031854780589
0.03 0.00196573527182893
0.04 0.00262146135670515
0.05 0.00327759993208763
0.06 0.00393425569851873
0.07 0.00459153332586976
0.08 0.00524953726445613
0.09 0.00590837458367388
0.1 0.00656815128338035
0.11 0.00722897712714719
0.12 0.00789096061155433
0.13 0.00855421182293859
0.14 0.0092188437742246
0.15 0.00988496880497878
0.16 0.0105527039566143
0.17 0.0112221655030774
0.18 0.0118934739767346
0.19 0.0125667490028029
0.2 0.0132421166277014
0.21 0.013919701704499
0.22 0.0145996362122709
0.23 0.0152820480088827
0.24 0.0159670736085938
0.25 0.0166548564751651
0.26 0.0173455345020288
0.27 0.0180392538241342
0.28 0.018736164389256
0.29 0.0194364259902765
0.3 0.0201401882165269
0.31 0.0208476249838447
0.32 0.0215589012383417
0.33 0.0222741916992002
0.34 0.0229936762867525
0.35 0.0237175467229702
0.36 0.0244459946507892
0.37 0.0251792228164158
0.38 0.0259174398306495
0.39 0.0266608646234719
0.4 0.0274097210845578
0.41 0.0281642397718009
0.42 0.0289246854714078
0.43 0.0296912968202003
0.44 0.030464351542164
0.45 0.0312441283623642
0.46 0.0320309220173424
0.47 0.0328250418596265
0.48 0.0336268122326049
0.49 0.0344365695145339
0.5 0.0352546807828426
0.51 0.0360815248980337
0.52 0.0369174982259775
0.53 0.0377630191602241
0.54 0.0386185457951147
0.55 0.0394845383784043
0.56 0.0403615124075996
0.57 0.0412499968609724
0.58 0.042150567483519
0.59 0.0430638278154256
0.6 0.0439904232858503
0.61 0.044931057404682
0.62 0.0458864757960522
0.63 0.0468574732490596
0.64 0.0478449184122471
0.65 0.0488497387424132
0.66 0.049872952566964
0.67 0.0509156381087557
0.68 0.0519789938728725
0.69 0.0530643081301057
0.7 0.0541729985248711
0.71 0.0553066097856815
0.72 0.0564668531893465
0.73 0.0576556118859593
0.74 0.0588749653585092
0.75 0.0601272382345663
0.76 0.0614149999556543
0.77 0.0627411639910248
0.78 0.0641089975740438
0.79 0.0655221965608325
0.8 0.0669850030018049
0.81 0.0685022283869477
0.82 0.0700794790375939
0.83 0.0717232733877771
0.84 0.0734412226855899
0.85 0.0752423978318075
0.86 0.0771376368057536
0.87 0.0791400938150012
0.88 0.0812659474810682
0.89 0.0835354351757153
0.9 0.0859743171514724
0.91 0.0886161879191771
0.92 0.0915060307075596
0.93 0.094706165301878
0.94 0.0983065835961069
0.95 0.102444717907901
0.96 0.107346722937499
0.97 0.113427742111189
0.98 0.121595114589192
0.99 0.134635170449131
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/ensemble-splatfacto/empirical_coverage.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.05, ymax=1.05,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 1
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.0111830269671647
0.02 0.0185036270540961
0.03 0.0258399832329049
0.04 0.0331854631431448
0.05 0.0405385849617446
0.06 0.0479017575299325
0.07 0.0552736705718229
0.08 0.0626558172077136
0.09 0.070052145271522
0.1 0.0774678719535399
0.11 0.0849062668178605
0.12 0.0923590044171807
0.13 0.0998392533027929
0.14 0.107338123954105
0.15 0.114864224844058
0.16 0.122414811012434
0.17 0.129992461410386
0.18 0.137609174658311
0.19 0.14525234827164
0.2 0.152947650208148
0.21 0.160672251311355
0.22 0.168438460097693
0.23 0.17625248168169
0.24 0.184117063588816
0.25 0.192041433268742
0.26 0.200021490442841
0.27 0.208051403492051
0.28 0.216147659138734
0.29 0.224312332377054
0.3 0.232550011077935
0.31 0.240859682724755
0.32 0.249244019451275
0.33 0.257727987167886
0.34 0.266328905341275
0.35 0.274981796927798
0.36 0.283667522979357
0.37 0.292377280600304
0.38 0.301119111042104
0.39 0.309874388936178
0.4 0.318643682966449
0.41 0.327437704546069
0.42 0.336249006706663
0.43 0.345084628493836
0.44 0.353946914508558
0.45 0.362804901688229
0.46 0.371681470951168
0.47 0.380574592266196
0.48 0.38948814391887
0.49 0.398406830784735
0.5 0.407351284191774
0.51 0.41629866769723
0.52 0.425254223829473
0.53 0.43421042664189
0.54 0.443174095140235
0.55 0.452129419894751
0.56 0.461077116103798
0.57 0.470015446075659
0.58 0.478947758907118
0.59 0.487861544041732
0.6 0.496776504269074
0.61 0.505672714878407
0.62 0.514557478746098
0.63 0.523437019518522
0.64 0.532306239846337
0.65 0.541152439620447
0.66 0.549988115758721
0.67 0.558810099825991
0.68 0.567618596663027
0.69 0.576424109877841
0.7 0.585215166529868
0.71 0.593992912911964
0.72 0.602773695950178
0.73 0.611533723121232
0.74 0.62027182998817
0.75 0.629005145960896
0.76 0.637731969671287
0.77 0.646449276662984
0.78 0.655166743463548
0.79 0.663892091109144
0.8 0.672620185172107
0.81 0.681375809403619
0.82 0.690154569838244
0.83 0.699058172721717
0.84 0.707923486888336
0.85 0.716854502025126
0.86 0.725868791500899
0.87 0.734988537175021
0.88 0.744237311853042
0.89 0.753637427002558
0.9 0.763236792879076
0.91 0.773060942601884
0.92 0.783167155621227
0.93 0.793618085797566
0.94 0.804510532386776
0.95 0.815999100644442
0.96 0.82835639690874
0.97 0.84203038063733
0.98 0.857961484729378
0.99 0.878780446625464
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.0141789234665938
0.02 0.020976721362358
0.03 0.0277728270047734
0.04 0.0345870994977266
0.05 0.0414052673256149
0.06 0.0482349956000525
0.07 0.0550602369351901
0.08 0.0619096802913255
0.09 0.0687744357647346
0.1 0.0756415416982541
0.11 0.0825254851388997
0.12 0.0894317385035153
0.13 0.0963524914514597
0.14 0.103291482173698
0.15 0.110255156464289
0.16 0.117242542163129
0.17 0.124257998773981
0.18 0.131293275260212
0.19 0.138366683317248
0.2 0.145471405273741
0.21 0.152601138581274
0.22 0.159767350838674
0.23 0.166964298068583
0.24 0.174194192923956
0.25 0.181466170563598
0.26 0.18878544576619
0.27 0.19615425272085
0.28 0.203567221998198
0.29 0.211047774213129
0.3 0.218586154658205
0.31 0.226199681332909
0.32 0.233897303664052
0.33 0.241683222352974
0.34 0.249522880325653
0.35 0.257390657926998
0.36 0.265219278539776
0.37 0.273053720309517
0.38 0.280910892246861
0.39 0.28877812102277
0.4 0.29665296900619
0.41 0.304533621036889
0.42 0.31242277187093
0.43 0.320319987104646
0.44 0.328220729987512
0.45 0.336128215728248
0.46 0.344033470589256
0.47 0.351942053210882
0.48 0.359869047975613
0.49 0.367801258440028
0.5 0.375733622399299
0.51 0.38368640435696
0.52 0.391629084411146
0.53 0.399572085976561
0.54 0.40748860239651
0.55 0.415389522741688
0.56 0.423277692598124
0.57 0.431158282558136
0.58 0.439039671375833
0.59 0.446916714588007
0.6 0.454800210722986
0.61 0.462684111923555
0.62 0.470574554762055
0.63 0.478466108254021
0.64 0.486356475160836
0.65 0.494258190010277
0.66 0.502163368069138
0.67 0.510095690490924
0.68 0.518046798067724
0.69 0.52601039102699
0.7 0.533992136010133
0.71 0.541973596055106
0.72 0.549979331414842
0.73 0.557988184412008
0.74 0.566020690237188
0.75 0.574081104813242
0.76 0.582183131345232
0.77 0.590321549412639
0.78 0.598498085034951
0.79 0.606736855601238
0.8 0.615042814961523
0.81 0.623400332977494
0.82 0.63185772037115
0.83 0.640526778010895
0.84 0.649197300383299
0.85 0.657990682564301
0.86 0.666941942617439
0.87 0.676070840360625
0.88 0.685408869087586
0.89 0.695005257213002
0.9 0.70488967123219
0.91 0.71512308768021
0.92 0.725766039514549
0.93 0.736924573333529
0.94 0.74875065567344
0.95 0.761482747275298
0.96 0.775450366186326
0.97 0.791289927191425
0.98 0.810306516242946
0.99 0.836184350116417
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.0162465071149299
0.02 0.0223555149811846
0.03 0.0284643265965766
0.04 0.0345899241425188
0.05 0.0407078103069956
0.06 0.0468383157445703
0.07 0.0529725530002263
0.08 0.059118941554466
0.09 0.065277937426419
0.1 0.0714503215541226
0.11 0.0776264548611657
0.12 0.0838207430281207
0.13 0.0900276018746028
0.14 0.0962555898105497
0.15 0.102491677729248
0.16 0.108755751690357
0.17 0.115034592712428
0.18 0.121343020464084
0.19 0.12767502855887
0.2 0.134028912369214
0.21 0.14041092327201
0.22 0.14682284357281
0.23 0.153263235064886
0.24 0.159740416655953
0.25 0.166248837746219
0.26 0.172809902802839
0.27 0.179406040464265
0.28 0.186057611875877
0.29 0.19275584872827
0.3 0.199497908592454
0.31 0.206318243629316
0.32 0.213218604552121
0.33 0.220202262602106
0.34 0.227232418330119
0.35 0.234254099165335
0.36 0.241259972621777
0.37 0.248295426855842
0.38 0.255350008380414
0.39 0.26240186376932
0.4 0.269468922811198
0.41 0.276556433128152
0.42 0.283656201616351
0.43 0.290764248088273
0.44 0.297891881726219
0.45 0.305033963869171
0.46 0.312191322892413
0.47 0.319357196871742
0.48 0.326538601078537
0.49 0.333738646715748
0.5 0.340955588459294
0.51 0.348183038727047
0.52 0.355431670766205
0.53 0.362680247646811
0.54 0.369922138040567
0.55 0.377172298048817
0.56 0.384429664660586
0.57 0.391696144858375
0.58 0.398984199164954
0.59 0.406284204380481
0.6 0.413603081795395
0.61 0.420925322678483
0.62 0.428270360295603
0.63 0.435632350119161
0.64 0.4430261512356
0.65 0.450437862865358
0.66 0.457871748140817
0.67 0.465333800660208
0.68 0.472826707057526
0.69 0.480346091490267
0.7 0.48790018323852
0.71 0.495500826524538
0.72 0.503122495050655
0.73 0.510786649857632
0.74 0.518500995714239
0.75 0.526272862683249
0.76 0.534106434494542
0.77 0.541996382284744
0.78 0.549967090447565
0.79 0.558023280607714
0.8 0.56617623099978
0.81 0.574424105212723
0.82 0.5828041096733
0.83 0.591394808457602
0.84 0.600058175216836
0.85 0.608904537726925
0.86 0.617932618051637
0.87 0.627189296220796
0.88 0.636728970950722
0.89 0.646576874457823
0.9 0.656798354888994
0.91 0.667454596786118
0.92 0.678617491649317
0.93 0.690403668102091
0.94 0.703010988225333
0.95 0.716712617208843
0.96 0.731907003281257
0.97 0.749356301365558
0.98 0.770608648254026
0.99 0.800095410469444
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.0171067856154062
0.02 0.0225662225146674
0.03 0.0280310366677668
0.04 0.0335021146187659
0.05 0.0389825207321611
0.06 0.0444664113226023
0.07 0.0499510004005418
0.08 0.0554467003081891
0.09 0.0609502501261516
0.1 0.066459479574971
0.11 0.0719744974583186
0.12 0.0774974099861827
0.13 0.0830313206664257
0.14 0.0885776045104658
0.15 0.0941463533482942
0.16 0.0997260358396575
0.17 0.105316725050729
0.18 0.110921009316551
0.19 0.116548556814984
0.2 0.122187708065935
0.21 0.127844995658833
0.22 0.13352146212821
0.23 0.139223842616412
0.24 0.144955524420672
0.25 0.150703631055312
0.26 0.156481825906741
0.27 0.162283693810062
0.28 0.168116141843098
0.29 0.17399010671763
0.3 0.17990964526659
0.31 0.185884047195504
0.32 0.191920165519421
0.33 0.198000142789335
0.34 0.204109060230872
0.35 0.210191772764063
0.36 0.216263624928334
0.37 0.22234567765657
0.38 0.228437701444154
0.39 0.234551712984426
0.4 0.240677137473592
0.41 0.246814150585993
0.42 0.252963659499304
0.43 0.259127365428512
0.44 0.265317759286696
0.45 0.271529336565935
0.46 0.277766577462621
0.47 0.284037440063392
0.48 0.290333902727304
0.49 0.296663407281915
0.5 0.303017514813837
0.51 0.309398334038892
0.52 0.315797110642556
0.53 0.322202362562311
0.54 0.328622884794535
0.55 0.335077286814102
0.56 0.341554355667226
0.57 0.348073829352347
0.58 0.354620238138316
0.59 0.36119730623222
0.6 0.367801619459284
0.61 0.374451296744562
0.62 0.381146062643116
0.63 0.387872412082934
0.64 0.394641526719848
0.65 0.401466188129961
0.66 0.408343355606104
0.67 0.415259210421067
0.68 0.422236792536943
0.69 0.429271157751388
0.7 0.436370693047633
0.71 0.44352432286638
0.72 0.450743501391274
0.73 0.458040257547738
0.74 0.465424030299239
0.75 0.472889208112846
0.76 0.480447912959673
0.77 0.48810931117277
0.78 0.495889331861559
0.79 0.503791832349525
0.8 0.511829779435649
0.81 0.520015190962038
0.82 0.528366988252976
0.83 0.536984133079977
0.84 0.545722202720441
0.85 0.554677787731857
0.86 0.563890968396749
0.87 0.573411856635749
0.88 0.583260611143224
0.89 0.593486542701949
0.9 0.604162113337398
0.91 0.61535856857552
0.92 0.627190068928528
0.93 0.639786597875315
0.94 0.653374431591857
0.95 0.668265644813299
0.96 0.68494036545913
0.97 0.704269114844791
0.98 0.72810721490137
0.99 0.761616554943379
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/ensemble-splatfacto/empirical_coverage_absolute_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.0148369694428388, ymax=0.311576358299615,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.00571714760783168
0.02 0.00789868951415463
0.03 0.0101247176012628
0.04 0.0123985398591318
0.05 0.0147242112836913
0.06 0.017052988596167
0.07 0.0193736071215381
0.08 0.0216863853427799
0.09 0.0240378179998427
0.1 0.0264308775521813
0.11 0.0288269831932186
0.12 0.0312353337671783
0.13 0.0336183199854069
0.14 0.0359842474727268
0.15 0.038324026948519
0.16 0.0406410054798958
0.17 0.0429412280368094
0.18 0.0452238141425723
0.19 0.0474927665285174
0.2 0.04973162375988
0.21 0.0519396099155398
0.22 0.054118829064326
0.23 0.0562752742434612
0.24 0.0584001121941205
0.25 0.0604721379404156
0.26 0.0624954986593566
0.27 0.0644709112102759
0.28 0.0663871373015476
0.29 0.0682435140356384
0.3 0.070044787321432
0.31 0.0718489383767215
0.32 0.0735947816393709
0.33 0.0752596075555779
0.34 0.0768208631352122
0.35 0.0783680487215625
0.36 0.0799135006328802
0.37 0.0814229659421227
0.38 0.082891235056527
0.39 0.0843527197228387
0.4 0.0858243513568767
0.41 0.0872680582825638
0.42 0.0886984815052744
0.43 0.090096480730804
0.44 0.09145576298605
0.45 0.0928038754548355
0.46 0.0941334525887391
0.47 0.0954753161005305
0.48 0.0967938806252944
0.49 0.0980923543535531
0.5 0.0993515596889042
0.51 0.100597885319794
0.52 0.101838552215583
0.53 0.103068230092063
0.54 0.104281234063765
0.55 0.105506978225128
0.56 0.106701299734652
0.57 0.107871876450142
0.58 0.109038142153492
0.59 0.110192714673561
0.6 0.111325141586966
0.61 0.112444861737329
0.62 0.113551633714435
0.63 0.114638894214391
0.64 0.115709590075195
0.65 0.116775253389978
0.66 0.11780961602655
0.67 0.118847060128536
0.68 0.119862156276446
0.69 0.120907617891152
0.7 0.121941699878954
0.71 0.122968162847251
0.72 0.123979093870555
0.73 0.124975062615158
0.74 0.125968027233727
0.75 0.126952028968691
0.76 0.127920600050678
0.77 0.128888511782639
0.78 0.129846000925931
0.79 0.13076688515338
0.8 0.131677638191095
0.81 0.132577361107943
0.82 0.133458344454094
0.83 0.134208863844044
0.84 0.135012737209794
0.85 0.135775960727734
0.86 0.136446848763436
0.87 0.13701465662967
0.88 0.137473170454555
0.89 0.137788078077403
0.9 0.137945312363723
0.91 0.137885754070543
0.92 0.137542253289573
0.93 0.13688627859622
0.94 0.135789664968212
0.95 0.134104201580869
0.96 0.13164360309126
0.97 0.12796961936267
0.98 0.122038515270622
0.99 0.111219553374536
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.00903012821301622
0.02 0.0112497708006173
0.03 0.0136729355145319
0.04 0.0161750183710214
0.05 0.0187391147530804
0.06 0.0213373968308405
0.07 0.0240446884253885
0.08 0.0267748039543336
0.09 0.0294913429167766
0.1 0.0323108310558632
0.11 0.0351423477957296
0.12 0.0379528242366669
0.13 0.0407541999907894
0.14 0.0435573881421973
0.15 0.0463502594381656
0.16 0.0491247786818251
0.17 0.0518721074035021
0.18 0.054602273111645
0.19 0.0573022845737673
0.2 0.0599934789909105
0.21 0.0626775269733873
0.22 0.0653649230099254
0.23 0.0680351816311808
0.24 0.0706731699840023
0.25 0.0732754466652578
0.26 0.0758341006769585
0.27 0.0783460984140132
0.28 0.0808394542580859
0.29 0.0832903914934668
0.3 0.0857112482539024
0.31 0.0880786009303794
0.32 0.0903817392750809
0.33 0.092609627610586
0.34 0.0948095936466037
0.35 0.0969953174297556
0.36 0.0992398516298942
0.37 0.101515018535319
0.38 0.103777830120972
0.39 0.10605840038709
0.4 0.108339698589688
0.41 0.110615915587765
0.42 0.112881862147114
0.43 0.115126951761205
0.44 0.117339648709253
0.45 0.119524954199455
0.46 0.121672889826135
0.47 0.123796534520835
0.48 0.125889556564152
0.49 0.127953034582654
0.5 0.129999967342907
0.51 0.132008857775239
0.52 0.134013430255111
0.53 0.135995795585276
0.54 0.137983164746088
0.55 0.139968483051233
0.56 0.141944567477299
0.57 0.14391858999356
0.58 0.145888722505737
0.59 0.147849485805054
0.6 0.149809014776884
0.61 0.151759006402313
0.62 0.153696210471367
0.63 0.155647080783438
0.64 0.157599817925361
0.65 0.159537868902882
0.66 0.161467630022362
0.67 0.163365892146484
0.68 0.165241111198532
0.69 0.167105818247175
0.7 0.168952847895193
0.71 0.170790124400108
0.72 0.172606447450806
0.73 0.174424281984396
0.74 0.176218935027617
0.75 0.177980446143589
0.76 0.179715674638065
0.77 0.181414878886203
0.78 0.183093145192417
0.79 0.184712262772586
0.8 0.186263735061304
0.81 0.187795178338259
0.82 0.189254976560437
0.83 0.190502393034032
0.84 0.191746145046422
0.85 0.192866432473094
0.86 0.193827834065763
0.87 0.194638068470018
0.88 0.195241796623201
0.89 0.19558695192718
0.9 0.195643790807201
0.91 0.195351016552083
0.92 0.194648220717275
0.93 0.193429540509265
0.94 0.191544509476191
0.95 0.188752787324611
0.96 0.184725727597862
0.97 0.178827300908223
0.98 0.169753079443153
0.99 0.153820221998612
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.0119405701113678
0.02 0.0143276712065788
0.03 0.0169664572942186
0.04 0.0197080998246859
0.05 0.022583530544771
0.06 0.0256118074144333
0.07 0.0286785115226352
0.08 0.0318084485594728
0.09 0.0349331101501761
0.1 0.0380439000809933
0.11 0.0411804819770065
0.12 0.0443819577255965
0.13 0.04768907004091
0.14 0.0510057637978132
0.15 0.0543647393522431
0.16 0.057732150853697
0.17 0.0610847642161477
0.18 0.0644106376040135
0.19 0.0677206882625973
0.2 0.0710463246024882
0.21 0.0744098677947552
0.22 0.0777780825425904
0.23 0.0811234400832442
0.24 0.0844375690944875
0.25 0.0877218548780738
0.26 0.0909706077897598
0.27 0.0942280933187521
0.28 0.0974345396098814
0.29 0.100600815841127
0.3 0.103775191336469
0.31 0.106886874375416
0.32 0.109921435569009
0.33 0.112885359663011
0.34 0.115810848505315
0.35 0.118743227156846
0.36 0.121725432769131
0.37 0.124740771028629
0.38 0.127757791931941
0.39 0.130771431587091
0.4 0.133768431811156
0.41 0.136737565430957
0.42 0.139693656581081
0.43 0.142637562258697
0.44 0.145626276096031
0.45 0.148575264766639
0.46 0.151494114625215
0.47 0.154383966472721
0.48 0.157250703339952
0.49 0.160082971746755
0.5 0.162883231348639
0.51 0.165669555517904
0.52 0.168424647221574
0.53 0.171166007167969
0.54 0.173907897313673
0.55 0.17663149026825
0.56 0.179335614735471
0.57 0.182015090492618
0.58 0.184670838565483
0.59 0.187320390456221
0.6 0.189941617190107
0.61 0.192545023356359
0.62 0.195117074190741
0.63 0.19766000149221
0.64 0.200163125424478
0.65 0.202634895818656
0.66 0.205073637418375
0.67 0.207477565023216
0.68 0.209835574909474
0.69 0.2121557126457
0.7 0.214429019675103
0.71 0.216684248036862
0.72 0.218954101828601
0.73 0.221171952366627
0.74 0.223360807740604
0.75 0.225497201374409
0.76 0.22756452923391
0.77 0.229567528075422
0.78 0.231488282709054
0.79 0.233333334072852
0.8 0.235074892210804
0.81 0.236718708401028
0.82 0.238223598778091
0.83 0.239512132948232
0.84 0.240725327376509
0.85 0.241757440006924
0.86 0.242645759866304
0.87 0.243302650432088
0.88 0.243675924286979
0.89 0.243739349232595
0.9 0.243429009603331
0.91 0.242720516310465
0.92 0.241525609052702
0.93 0.239709530996099
0.94 0.237073382451955
0.95 0.233343482391166
0.96 0.22812031533135
0.97 0.220643698634442
0.98 0.209391351745974
0.99 0.189904589530556
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.0135905361121251
0.02 0.0163237181691565
0.03 0.019340429394193
0.04 0.0225240728026391
0.05 0.0258107089220991
0.06 0.029312429996275
0.07 0.0328909890591599
0.08 0.0364568117006499
0.09 0.0400192631221009
0.1 0.0435756974301447
0.11 0.0472032836484081
0.12 0.0509816588318367
0.13 0.0549073608986515
0.14 0.0588234713080189
0.15 0.0627210367960385
0.16 0.0667017182634681
0.17 0.0706953053852874
0.18 0.0746791599951867
0.19 0.0787379798863
0.2 0.0828209350089901
0.21 0.0868891273030907
0.22 0.09093893518455
0.23 0.094965292062119
0.24 0.0989689751823719
0.25 0.10300919522437
0.26 0.107023814046815
0.27 0.111016142309183
0.28 0.114982339625999
0.29 0.118909838362056
0.3 0.122846884125213
0.31 0.126772832303549
0.32 0.130672135482583
0.33 0.134550137927457
0.34 0.138401504124199
0.35 0.1422742694315
0.36 0.146155285607707
0.37 0.150022453412313
0.38 0.153878189771764
0.39 0.157706402202823
0.4 0.161519932674327
0.41 0.165317370497284
0.42 0.169098816382758
0.43 0.172862749813715
0.44 0.176595317217354
0.45 0.180303224856227
0.46 0.18398269746444
0.47 0.18762554703991
0.48 0.191239618337988
0.49 0.194818147218915
0.5 0.198368936245993
0.51 0.201892212992043
0.52 0.205393435600131
0.53 0.208887638145877
0.54 0.212360168708459
0.55 0.215798823095371
0.56 0.219212808227931
0.57 0.222593036817693
0.58 0.22597095099229
0.59 0.229318603893655
0.6 0.232639028421217
0.61 0.235914533013498
0.62 0.239144555147637
0.63 0.242343291219081
0.64 0.245500104251067
0.65 0.248601789493751
0.66 0.251656644393896
0.67 0.254740789578933
0.68 0.257763207463057
0.69 0.260728842248612
0.7 0.263629306952367
0.71 0.26647567713362
0.72 0.269256498608726
0.73 0.271959742452262
0.74 0.274575969700761
0.75 0.277110791887154
0.76 0.279552087040327
0.77 0.28189068882723
0.78 0.284110668138441
0.79 0.286208167650475
0.8 0.288170220564351
0.81 0.289984809037962
0.82 0.291633011747023
0.83 0.293015866920023
0.84 0.294277797279559
0.85 0.295322212268143
0.86 0.296109031603251
0.87 0.296588143364251
0.88 0.296739388856776
0.89 0.296513457298051
0.9 0.295837886662601
0.91 0.29464143142448
0.92 0.292809931071472
0.93 0.290213402124685
0.94 0.286625568408143
0.95 0.281734355186701
0.96 0.27505963454087
0.97 0.265730885155208
0.98 0.25189278509863
0.99 0.228383445056621
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/ensemble-splatfacto/empirical_coverage_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.311931697580386, ymax=0.0222990943390153,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.0011830269671647
0.02 -0.00149637294590388
0.03 -0.0041600167670951
0.04 -0.00681453685685512
0.05 -0.00946141503825538
0.06 -0.0120982424700674
0.07 -0.0147263294281771
0.08 -0.0173441827922863
0.09 -0.019947854728478
0.1 -0.0225321280464601
0.11 -0.0250937331821395
0.12 -0.0276409955828193
0.13 -0.0301607466972071
0.14 -0.0326618760458954
0.15 -0.0351357751559424
0.16 -0.0375851889875664
0.17 -0.0400075385896136
0.18 -0.042390825341689
0.19 -0.0447476517283598
0.2 -0.0470523497918514
0.21 -0.0493277486886455
0.22 -0.051561539902307
0.23 -0.0537475183183103
0.24 -0.055882936411184
0.25 -0.0579585667312575
0.26 -0.0599785095571586
0.27 -0.0619485965079488
0.28 -0.0638523408612665
0.29 -0.065687667622946
0.3 -0.067449988922065
0.31 -0.0691403172752454
0.32 -0.0707559805487255
0.33 -0.0722720128321135
0.34 -0.0736710946587245
0.35 -0.0750182030722017
0.36 -0.0763324770206426
0.37 -0.0776227193996955
0.38 -0.0788808889578963
0.39 -0.0801256110638222
0.4 -0.081356317033551
0.41 -0.0825622954539307
0.42 -0.083750993293337
0.43 -0.0849153715061642
0.44 -0.0860530854914421
0.45 -0.0871950983117714
0.46 -0.0883185290488316
0.47 -0.0894254077338042
0.48 -0.09051185608113
0.49 -0.0915931692152654
0.5 -0.0926487158082255
0.51 -0.0937013323027705
0.52 -0.0947457761705268
0.53 -0.0957895733581104
0.54 -0.0968259048597652
0.55 -0.0978705801052487
0.56 -0.0989228838962024
0.57 -0.0999845539243414
0.58 -0.101052241092882
0.59 -0.102138455958268
0.6 -0.103223495730926
0.61 -0.104327285121593
0.62 -0.105442521253902
0.63 -0.106562980481478
0.64 -0.107693760153663
0.65 -0.108847560379552
0.66 -0.110011884241279
0.67 -0.111189900174009
0.68 -0.112381403336973
0.69 -0.113575890122159
0.7 -0.114784833470132
0.71 -0.116007087088036
0.72 -0.117226304049822
0.73 -0.118466276878768
0.74 -0.11972817001183
0.75 -0.120994854039104
0.76 -0.122268030328713
0.77 -0.123550723337016
0.78 -0.124833256536452
0.79 -0.126107908890856
0.8 -0.127379814827893
0.81 -0.128624190596381
0.82 -0.129845430161756
0.83 -0.130941827278283
0.84 -0.132076513111664
0.85 -0.133145497974873
0.86 -0.1341312084991
0.87 -0.135011462824979
0.88 -0.135762688146958
0.89 -0.136362572997442
0.9 -0.136763207120924
0.91 -0.136939057398116
0.92 -0.136832844378773
0.93 -0.136381914202434
0.94 -0.135489467613224
0.95 -0.134000899355558
0.96 -0.13164360309126
0.97 -0.12796961936267
0.98 -0.122038515270622
0.99 -0.111219553374536
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.0041789234665938
0.02 0.000976721362357993
0.03 -0.00222717299522667
0.04 -0.00541290050227332
0.05 -0.00859473267438501
0.06 -0.0117650043999474
0.07 -0.0149397630648098
0.08 -0.0180903197086745
0.09 -0.0212255642352654
0.1 -0.0243584583017459
0.11 -0.0274745148611003
0.12 -0.0305682614964847
0.13 -0.0336475085485403
0.14 -0.0367085178263018
0.15 -0.0397448435357106
0.16 -0.0427574578368709
0.17 -0.0457420012260188
0.18 -0.0487067247397882
0.19 -0.0516333166827518
0.2 -0.0545285947262587
0.21 -0.0573988614187262
0.22 -0.0602326491613257
0.23 -0.0630357019314174
0.24 -0.0658058070760436
0.25 -0.0685338294364021
0.26 -0.0712145542338097
0.27 -0.0738457472791497
0.28 -0.0764327780018018
0.29 -0.0789522257868712
0.3 -0.0814138453417951
0.31 -0.0838003186670913
0.32 -0.0861026963359479
0.33 -0.0883167776470258
0.34 -0.0904771196743472
0.35 -0.0926093420730017
0.36 -0.0947807214602242
0.37 -0.0969462796904829
0.38 -0.099089107753139
0.39 -0.10122187897723
0.4 -0.10334703099381
0.41 -0.105466378963111
0.42 -0.10757722812907
0.43 -0.109680012895354
0.44 -0.111779270012488
0.45 -0.113871784271752
0.46 -0.115966529410744
0.47 -0.118057946789118
0.48 -0.120130952024387
0.49 -0.122198741559972
0.5 -0.124266377600701
0.51 -0.12631359564304
0.52 -0.128370915588854
0.53 -0.130427914023439
0.54 -0.13251139760349
0.55 -0.134610477258312
0.56 -0.136722307401876
0.57 -0.138841717441864
0.58 -0.140960328624167
0.59 -0.143083285411993
0.6 -0.145199789277014
0.61 -0.147315888076445
0.62 -0.149425445237945
0.63 -0.151533891745979
0.64 -0.153643524839163
0.65 -0.155741809989723
0.66 -0.157836631930862
0.67 -0.159904309509076
0.68 -0.161953201932276
0.69 -0.16398960897301
0.7 -0.166007863989867
0.71 -0.168026403944894
0.72 -0.170020668585158
0.73 -0.172011815587992
0.74 -0.173979309762812
0.75 -0.175918895186758
0.76 -0.177816868654768
0.77 -0.179678450587361
0.78 -0.181501914965049
0.79 -0.183263144398762
0.8 -0.184957185038478
0.81 -0.186599667022506
0.82 -0.18814227962885
0.83 -0.189473221989105
0.84 -0.190802699616701
0.85 -0.192009317435699
0.86 -0.193058057382561
0.87 -0.193929159639375
0.88 -0.194591130912414
0.89 -0.194994742786998
0.9 -0.19511032876781
0.91 -0.19487691231979
0.92 -0.194233960485451
0.93 -0.193075426666471
0.94 -0.19124934432656
0.95 -0.188517252724702
0.96 -0.184549633813674
0.97 -0.178710072808575
0.98 -0.169693483757054
0.99 -0.153815649883583
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.00624650711492989
0.02 0.00235551498118456
0.03 -0.00153567340342346
0.04 -0.00541007585748112
0.05 -0.00929218969300433
0.06 -0.0131616842554296
0.07 -0.0170274469997736
0.08 -0.020881058445534
0.09 -0.0247220625735809
0.1 -0.0285496784458773
0.11 -0.0323735451388343
0.12 -0.0361792569718793
0.13 -0.0399723981253972
0.14 -0.0437444101894503
0.15 -0.0475083222707523
0.16 -0.0512442483096426
0.17 -0.054965407287572
0.18 -0.058656979535916
0.19 -0.0623249714411301
0.2 -0.0659710876307858
0.21 -0.0695890767279898
0.22 -0.0731771564271895
0.23 -0.0767367649351144
0.24 -0.0802595833440472
0.25 -0.0837511622537814
0.26 -0.0871900971971612
0.27 -0.0905939595357354
0.28 -0.093942388124123
0.29 -0.0972441512717298
0.3 -0.100502091407546
0.31 -0.103681756370684
0.32 -0.106781395447879
0.33 -0.109797737397894
0.34 -0.112767581669881
0.35 -0.115745900834665
0.36 -0.118740027378223
0.37 -0.121704573144158
0.38 -0.124649991619586
0.39 -0.127598136230681
0.4 -0.130531077188802
0.41 -0.133443566871848
0.42 -0.136343798383649
0.43 -0.139235751911727
0.44 -0.142108118273781
0.45 -0.144966036130829
0.46 -0.147808677107587
0.47 -0.150642803128258
0.48 -0.153461398921463
0.49 -0.156261353284252
0.5 -0.159044411540706
0.51 -0.161816961272953
0.52 -0.164568329233795
0.53 -0.167319752353189
0.54 -0.170077861959433
0.55 -0.172827701951183
0.56 -0.175570335339414
0.57 -0.178303855141625
0.58 -0.181015800835046
0.59 -0.183715795619519
0.6 -0.186396918204605
0.61 -0.189074677321517
0.62 -0.191729639704397
0.63 -0.194367649880839
0.64 -0.1969738487644
0.65 -0.199562137134642
0.66 -0.202128251859183
0.67 -0.204666199339792
0.68 -0.207173292942473
0.69 -0.209653908509733
0.7 -0.212099816761481
0.71 -0.214499173475462
0.72 -0.216877504949345
0.73 -0.219213350142368
0.74 -0.221499004285761
0.75 -0.223727137316751
0.76 -0.225893565505458
0.77 -0.228003617715256
0.78 -0.230032909552435
0.79 -0.231976719392286
0.8 -0.23382376900022
0.81 -0.235575894787277
0.82 -0.2371958903267
0.83 -0.238605191542398
0.84 -0.239941824783164
0.85 -0.241095462273075
0.86 -0.242067381948363
0.87 -0.242810703779204
0.88 -0.243271029049278
0.89 -0.243423125542177
0.9 -0.243201645111006
0.91 -0.242545403213883
0.92 -0.241382508350683
0.93 -0.239596331897909
0.94 -0.236989011774667
0.95 -0.233287382791157
0.96 -0.228092996718743
0.97 -0.220643698634442
0.98 -0.209391351745974
0.99 -0.189904589530556
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.00710678561540618
0.02 0.00256622251466736
0.03 -0.00196896333223325
0.04 -0.00649788538123399
0.05 -0.0110174792678388
0.06 -0.0155335886773977
0.07 -0.0200489995994582
0.08 -0.0245532996918108
0.09 -0.0290497498738484
0.1 -0.033540520425029
0.11 -0.0380255025416814
0.12 -0.0425025900138173
0.13 -0.0469686793335743
0.14 -0.0514223954895342
0.15 -0.0558536466517058
0.16 -0.0602739641603424
0.17 -0.0646832749492707
0.18 -0.0690789906834486
0.19 -0.0734514431850161
0.2 -0.0778122919340648
0.21 -0.0821550043411669
0.22 -0.0864785378717897
0.23 -0.0907761573835884
0.24 -0.0950444755793275
0.25 -0.0992963689446883
0.26 -0.103518174093259
0.27 -0.107716306189938
0.28 -0.111883858156902
0.29 -0.11600989328237
0.3 -0.12009035473341
0.31 -0.124115952804496
0.32 -0.128079834480579
0.33 -0.131999857210665
0.34 -0.135890939769128
0.35 -0.139808227235937
0.36 -0.143736375071666
0.37 -0.14765432234343
0.38 -0.151562298555846
0.39 -0.155448287015574
0.4 -0.159322862526408
0.41 -0.163185849414007
0.42 -0.167036340500695
0.43 -0.170872634571488
0.44 -0.174682240713304
0.45 -0.178470663434065
0.46 -0.182233422537379
0.47 -0.185962559936608
0.48 -0.189666097272696
0.49 -0.193336592718085
0.5 -0.196982485186163
0.51 -0.200601665961108
0.52 -0.204202889357444
0.53 -0.207797637437689
0.54 -0.211377115205465
0.55 -0.214922713185898
0.56 -0.218445644332774
0.57 -0.221926170647653
0.58 -0.225379761861684
0.59 -0.22880269376778
0.6 -0.232198380540716
0.61 -0.235548703255438
0.62 -0.238853937356883
0.63 -0.242127587917066
0.64 -0.245358473280152
0.65 -0.248533811870039
0.66 -0.251656644393896
0.67 -0.254740789578933
0.68 -0.257763207463057
0.69 -0.260728842248612
0.7 -0.263629306952367
0.71 -0.26647567713362
0.72 -0.269256498608726
0.73 -0.271959742452262
0.74 -0.274575969700761
0.75 -0.277110791887154
0.76 -0.279552087040327
0.77 -0.28189068882723
0.78 -0.284110668138441
0.79 -0.286208167650475
0.8 -0.288170220564351
0.81 -0.289984809037962
0.82 -0.291633011747023
0.83 -0.293015866920023
0.84 -0.294277797279559
0.85 -0.295322212268143
0.86 -0.296109031603251
0.87 -0.296588143364251
0.88 -0.296739388856776
0.89 -0.296513457298051
0.9 -0.295837886662601
0.91 -0.29464143142448
0.92 -0.292809931071472
0.93 -0.290213402124685
0.94 -0.286625568408143
0.95 -0.281734355186701
0.96 -0.27505963454087
0.97 -0.265730885155208
0.98 -0.25189278509863
0.99 -0.228383445056621
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/ensemble-splatfacto/empirical_coverage_negative_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.0148369694428388, ymax=0.311576358299615,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.00226706032033349
0.02 0.00469753123002925
0.03 0.00714236718417897
0.04 0.00960653835799346
0.05 0.0120928131609733
0.06 0.0145756155331172
0.07 0.0170499682748576
0.08 0.0195152840675331
0.09 0.0219928363641603
0.1 0.0244815027993207
0.11 0.026960358187679
0.12 0.0294381646749988
0.13 0.031889533341307
0.14 0.0343230617593111
0.15 0.0367299010522307
0.16 0.0391130972337311
0.17 0.0414743833132115
0.18 0.0438073197421307
0.19 0.0461202091284386
0.2 0.0483919867758657
0.21 0.0506336793020926
0.22 0.0528401844833165
0.23 0.0550113962808858
0.24 0.0571415243026522
0.25 0.0592153523358366
0.26 0.0612370041082576
0.27 0.0632097538591124
0.28 0.0651197390814071
0.29 0.0669655908292922
0.3 0.0687473881217485
0.31 0.0704946278259835
0.32 0.0721753810940482
0.33 0.0737658101938457
0.34 0.0752459788969683
0.35 0.0766931258968821
0.36 0.0781229888267614
0.37 0.0795228426709091
0.38 0.0808860620072117
0.39 0.0822391653933305
0.4 0.0835903341952138
0.41 0.0849151768682473
0.42 0.0862247373993057
0.43 0.0875059261184841
0.44 0.088754424238746
0.45 0.0899994868833034
0.46 0.0912259908187854
0.47 0.0924503619171674
0.48 0.0936528683532122
0.49 0.0948427617844093
0.5 0.0960001377485649
0.51 0.0971496088112823
0.52 0.098292164193055
0.53 0.0994289017250867
0.54 0.100553569461765
0.55 0.101688779165188
0.56 0.102812091815427
0.57 0.103928215187242
0.58 0.105045191623187
0.59 0.106165585315915
0.6 0.107274318658946
0.61 0.108386073429461
0.62 0.109497077484168
0.63 0.110600937347935
0.64 0.111701675114429
0.65 0.112811406884765
0.66 0.113910750133914
0.67 0.115018480151272
0.68 0.11612177980671
0.69 0.117241754006656
0.7 0.118363266674543
0.71 0.119487624967644
0.72 0.120602698960188
0.73 0.121720669746963
0.74 0.122848098622778
0.75 0.123973441503898
0.76 0.125094315189695
0.77 0.126219617559828
0.78 0.127339628731191
0.79 0.128437397022118
0.8 0.129528726509494
0.81 0.130600775852162
0.82 0.131651887307925
0.83 0.132575345561164
0.84 0.133544625160729
0.85 0.134460729351304
0.86 0.135289028631268
0.87 0.136013059727325
0.88 0.136617929300756
0.89 0.137075325537422
0.9 0.137354259742324
0.91 0.13741240573433
0.92 0.137187548834173
0.93 0.136634096399327
0.94 0.135639566290718
0.95 0.134052550468213
0.96 0.13164360309126
0.97 0.12796961936267
0.98 0.122038515270622
0.99 0.111219553374536
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.00242560237321121
0.02 0.00513652471912964
0.03 0.00795005425487926
0.04 0.0107939594366474
0.05 0.0136669237137327
0.06 0.016551200615394
0.07 0.0194922257450991
0.08 0.022432561831504
0.09 0.025358453576021
0.1 0.0283346446788045
0.11 0.0313084313284149
0.12 0.0342605428665758
0.13 0.0372008542696648
0.14 0.0401329529842496
0.15 0.0430475514869381
0.16 0.045941118259348
0.17 0.0488070543147604
0.18 0.0516544989257166
0.19 0.0544678006282595
0.2 0.0572610368585846
0.21 0.0600381941960567
0.22 0.0627987860856256
0.23 0.0655354417812991
0.24 0.0682394885300229
0.25 0.0709046380508299
0.26 0.0735243274553841
0.27 0.0760959228465814
0.28 0.0786361161299439
0.29 0.081121308640169
0.3 0.0835625467978488
0.31 0.0859394597987354
0.32 0.0882422178055144
0.33 0.0904632026288059
0.34 0.0926433566604754
0.35 0.0948023297513787
0.36 0.0970102865450592
0.37 0.0992306491129007
0.38 0.101433468937055
0.39 0.10364013968216
0.4 0.105843364791749
0.41 0.108041147275438
0.42 0.110229545138092
0.43 0.112403482328279
0.44 0.11455945936087
0.45 0.116698369235603
0.46 0.118819709618439
0.47 0.120927240654977
0.48 0.123010254294269
0.49 0.125075888071313
0.5 0.127133172471804
0.51 0.12916122670914
0.52 0.131192172921982
0.53 0.133211854804357
0.54 0.135247281174789
0.55 0.137289480154772
0.56 0.139333437439587
0.57 0.141380153717712
0.58 0.143424525564952
0.59 0.145466385608523
0.6 0.147504402026949
0.61 0.149537447239379
0.62 0.151560827854656
0.63 0.153590486264709
0.64 0.155621671382262
0.65 0.157639839446302
0.66 0.159652130976612
0.67 0.16163510082778
0.68 0.163597156565404
0.69 0.165547713610092
0.7 0.16748035594253
0.71 0.169408264172501
0.72 0.171313558017982
0.73 0.173218048786194
0.74 0.175099122395215
0.75 0.176949670665173
0.76 0.178766271646417
0.77 0.180546664736782
0.78 0.182297530078733
0.79 0.183987703585674
0.8 0.185610460049891
0.81 0.187197422680383
0.82 0.188698628094644
0.83 0.189987807511568
0.84 0.191274422331562
0.85 0.192437874954397
0.86 0.193442945724162
0.87 0.194283614054697
0.88 0.194916463767807
0.89 0.195290847357089
0.9 0.195377059787505
0.91 0.195113964435936
0.92 0.194441090601363
0.93 0.193252483587868
0.94 0.191396926901376
0.95 0.188635020024656
0.96 0.184637680705768
0.97 0.178768686858399
0.98 0.169723281600104
0.99 0.153817935941098
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.00284703149821894
0.02 0.00598607811269711
0.03 0.00925106534882105
0.04 0.0125590878410835
0.05 0.0159378601188877
0.06 0.0193867458349315
0.07 0.0228529792612044
0.08 0.0263447535025034
0.09 0.0298275863618785
0.1 0.0332967892634353
0.11 0.0367770135579204
0.12 0.0402806073487379
0.13 0.0438307340831536
0.14 0.0473750869936318
0.15 0.0509365308114977
0.16 0.0544881995816698
0.17 0.0580250857518598
0.18 0.0615338085699647
0.19 0.0650228298518637
0.2 0.068508706116637
0.21 0.0719994722613725
0.22 0.07547761948489
0.23 0.0789301025091793
0.24 0.0823485762192674
0.25 0.0857365085659276
0.26 0.0890803524934605
0.27 0.0924110264272438
0.28 0.0956884638670022
0.29 0.0989224835564282
0.3 0.102138641372008
0.31 0.10528431537305
0.32 0.108351415508444
0.33 0.111341548530452
0.34 0.114289215087598
0.35 0.117244563995756
0.36 0.120232730073677
0.37 0.123222672086393
0.38 0.126203891775763
0.39 0.129184783908886
0.4 0.132149754499979
0.41 0.135090566151403
0.42 0.138018727482365
0.43 0.140936657085212
0.44 0.143867197184906
0.45 0.146770650448734
0.46 0.149651395866401
0.47 0.15251338480049
0.48 0.155356051130707
0.49 0.158172162515504
0.5 0.160963821444672
0.51 0.163743258395429
0.52 0.166496488227684
0.53 0.169242879760579
0.54 0.171992879636553
0.55 0.174729596109716
0.56 0.177452975037443
0.57 0.180159472817121
0.58 0.182843319700265
0.59 0.18551809303787
0.6 0.188169267697356
0.61 0.190809850338938
0.62 0.193423356947569
0.63 0.196013825686525
0.64 0.198568487094439
0.65 0.201098516476649
0.66 0.203600944638779
0.67 0.206071882181504
0.68 0.208504433925974
0.69 0.210904810577716
0.7 0.213264418218291
0.71 0.215591710756162
0.72 0.217915803388973
0.73 0.220192651254498
0.74 0.222429906013183
0.75 0.22461216934558
0.76 0.226729047369684
0.77 0.228785572895339
0.78 0.230760596130744
0.79 0.232655026732569
0.8 0.234449330605512
0.81 0.236147301594152
0.82 0.237709744552395
0.83 0.239058662245315
0.84 0.240333576079836
0.85 0.241426451139999
0.86 0.242356570907334
0.87 0.243056677105646
0.88 0.243473476668129
0.89 0.243581237387386
0.9 0.243315327357168
0.91 0.242632959762174
0.92 0.241454058701693
0.93 0.239652931447004
0.94 0.237031197113311
0.95 0.233315432591161
0.96 0.228106656025047
0.97 0.220643698634442
0.98 0.209391351745974
0.99 0.189904589530556
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.00324187524835944
0.02 0.00687874782724455
0.03 0.0106546963632131
0.04 0.0145109790919365
0.05 0.018414094094969
0.06 0.0224230093368363
0.07 0.026469994329309
0.08 0.0305050556962304
0.09 0.0345345064979747
0.1 0.0385581089275868
0.11 0.0426143930950447
0.12 0.046742124422827
0.13 0.0509380201161129
0.14 0.0551229333987765
0.15 0.0592873417238721
0.16 0.0634878412119053
0.17 0.067689290167279
0.18 0.0718790753393177
0.19 0.076094711535658
0.2 0.0803166134715275
0.21 0.0845220658221288
0.22 0.0887087365281699
0.23 0.0928707247228537
0.24 0.0970067253808497
0.25 0.101152782084529
0.26 0.105270994070037
0.27 0.109366224249561
0.28 0.11343309889145
0.29 0.117459865822213
0.3 0.121468619429312
0.31 0.125444392554022
0.32 0.129375984981581
0.33 0.133274997569061
0.34 0.137146221946663
0.35 0.141041248333719
0.36 0.144945830339686
0.37 0.148838387877871
0.38 0.152720244163805
0.39 0.156577344609198
0.4 0.160421397600368
0.41 0.164251609955645
0.42 0.168067578441727
0.43 0.171867692192602
0.44 0.175638778965329
0.45 0.179386944145146
0.46 0.18310806000091
0.47 0.186794053488259
0.48 0.190452857805342
0.49 0.1940773699685
0.5 0.197675710716078
0.51 0.201246939476575
0.52 0.204798162478788
0.53 0.208342637791783
0.54 0.211868641956962
0.55 0.215360768140635
0.56 0.218829226280352
0.57 0.222259603732673
0.58 0.225675356426987
0.59 0.229060648830717
0.6 0.232418704480967
0.61 0.235731618134468
0.62 0.23899924625226
0.63 0.242235439568074
0.64 0.24542928876561
0.65 0.248567800681895
0.66 0.251656644393896
0.67 0.254740789578933
0.68 0.257763207463057
0.69 0.260728842248612
0.7 0.263629306952367
0.71 0.26647567713362
0.72 0.269256498608726
0.73 0.271959742452262
0.74 0.274575969700761
0.75 0.277110791887154
0.76 0.279552087040327
0.77 0.28189068882723
0.78 0.284110668138441
0.79 0.286208167650475
0.8 0.288170220564351
0.81 0.289984809037962
0.82 0.291633011747023
0.83 0.293015866920023
0.84 0.294277797279559
0.85 0.295322212268143
0.86 0.296109031603251
0.87 0.296588143364251
0.88 0.296739388856776
0.89 0.296513457298051
0.9 0.295837886662601
0.91 0.29464143142448
0.92 0.292809931071472
0.93 0.290213402124685
0.94 0.286625568408143
0.95 0.281734355186701
0.96 0.27505963454087
0.97 0.265730885155208
0.98 0.25189278509863
0.99 0.228383445056621
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/nerfacto-laplace/avg_length.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.039, xmax=1.039,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.00165693941625625, ymax=0.0362041220783851,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.01 0.000167788162840328
0.02 0.000335602710765223
0.03 0.000503470026405738
0.04 0.000671416500406064
0.05 0.000839468710430125
0.06 0.00100765335811675
0.07 0.00117599725580434
0.08 0.00134452721958549
0.09 0.00151327057307293
0.1 0.00168225470189252
0.11 0.00185150723985064
0.12 0.00202105654349925
0.13 0.00219093043089159
0.14 0.00236115772676313
0.15 0.00253176793309258
0.16 0.00270279017619781
0.17 0.00287425449727996
0.18 0.00304619216294638
0.19 0.0032186334959334
0.2 0.0033916103586208
0.21 0.00356515549494546
0.22 0.00373930248328832
0.23 0.00391408396836689
0.24 0.00408953482384033
0.25 0.00426569172904825
0.26 0.00444259020868875
0.27 0.00462026756463394
0.28 0.00479876280749746
0.29 0.0049781153599018
0.3 0.00515836545416449
0.31 0.00533955576541934
0.32 0.00552173008596777
0.33 0.00570493209361536
0.34 0.00588920908212118
0.35 0.00607460920553233
0.36 0.00626118176153469
0.37 0.00644897800494267
0.38 0.0066380524246715
0.39 0.00682846054819434
0.4 0.0070202593421598
0.41 0.00721351012021851
0.42 0.00740827684406585
0.43 0.00760462419645058
0.44 0.00780262134544392
0.45 0.00800233994533151
0.46 0.00820385561881327
0.47 0.00840724789352936
0.48 0.00861259946232811
0.49 0.0088199977278637
0.5 0.00902953466701748
0.51 0.00924130831868263
0.52 0.0094554199463763
0.53 0.00967197785878883
0.54 0.00989109641151175
0.55 0.0101128987181404
0.56 0.0103375115844189
0.57 0.0105650734827838
0.58 0.0107957291131499
0.59 0.0110296352776155
0.6 0.0112669589216672
0.61 0.0115078765593948
0.62 0.0117525808904299
0.63 0.0120012765182836
0.64 0.0122541829897168
0.65 0.0125115413030497
0.66 0.0127736093964875
0.67 0.0130406661673206
0.68 0.0133130150705265
0.69 0.0135909894324407
0.7 0.0138749494281768
0.71 0.0141652942360309
0.72 0.0144624594058439
0.73 0.0147669283299845
0.74 0.0150792341024669
0.75 0.0153999681492956
0.76 0.0157297951042581
0.77 0.0160694549244764
0.78 0.016419789496325
0.79 0.016781742716145
0.8 0.0171563996235665
0.81 0.0175449959057802
0.82 0.0179489670403055
0.83 0.0183699785173422
0.84 0.0188099868825889
0.85 0.0192713087564682
0.86 0.0197567228501304
0.87 0.0202695980918703
0.88 0.020814078245101
0.89 0.021395345498231
0.9 0.0220199992080746
0.91 0.0226966433777501
0.92 0.0234367996313446
0.93 0.0242564264527
0.94 0.0251785765368751
0.95 0.0262384475359882
0.96 0.027493964144768
0.97 0.0290514538408907
0.98 0.0311433048094409
0.99 0.0344831647377196
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.000106788657740006
0.02 0.000213594105531419
0.03 0.000320433128931434
0.04 0.00042732255428371
0.05 0.000534279272522385
0.06 0.000641320242755093
0.07 0.000748462593821304
0.08 0.000855723344402745
0.09 0.000963119986287995
0.1 0.00107066978239644
0.11 0.00117839054252974
0.12 0.00128629991454235
0.13 0.00139441604499476
0.14 0.00150275730492885
0.15 0.00161134184178626
0.16 0.00172018895595923
0.17 0.00182931738858239
0.18 0.00193874685154773
0.19 0.00204849702605918
0.2 0.00215858813750203
0.21 0.00226904072186569
0.22 0.00237987627367528
0.23 0.00249111584755916
0.24 0.00260278170306985
0.25 0.00271489648241272
0.26 0.00282748349936647
0.27 0.00294056590010432
0.28 0.00305416895608897
0.29 0.00316831778314153
0.3 0.00328303799203783
0.31 0.00339835660016803
0.32 0.00351430105073702
0.33 0.00363090014115476
0.34 0.00374818291158027
0.35 0.0038661808062331
0.36 0.0039849246713876
0.37 0.00410444746710865
0.38 0.00422478381472946
0.39 0.00434596868043388
0.4 0.00446803928497843
0.41 0.00459103334736948
0.42 0.00471499234106441
0.43 0.00483995770626334
0.44 0.00496597254003579
0.45 0.00509308353554005
0.46 0.00522133811119648
0.47 0.00535078710554121
0.48 0.00548148273486606
0.49 0.0056134810136462
0.5 0.00574684128136015
0.51 0.00588162386751932
0.52 0.00601789541240524
0.53 0.00615572371166324
0.54 0.00629518161499356
0.55 0.00643634707164407
0.56 0.00657930170848212
0.57 0.00672413389714266
0.58 0.00687093413740588
0.59 0.00701980421019363
0.6 0.0071708480956538
0.61 0.00732417978190055
0.62 0.00747992163139919
0.63 0.00763820330921517
0.64 0.0077991667336799
0.65 0.00796296174057026
0.66 0.0081297543809602
0.67 0.00829972229584705
0.68 0.00847305939319842
0.69 0.00864997582774955
0.7 0.00883070159308392
0.71 0.00901549178973683
0.72 0.00920462174578933
0.73 0.00939840092142088
0.74 0.00959716795574932
0.75 0.00980129832556852
0.76 0.0100112162479998
0.77 0.0102273933073606
0.78 0.0104503625821093
0.79 0.0106807278843353
0.8 0.0109191776064596
0.81 0.0111664999974286
0.82 0.0114236079395713
0.83 0.011691559499453
0.84 0.0119716036125646
0.85 0.0122652096091018
0.86 0.0125741506890382
0.87 0.0129005708181485
0.88 0.0132471048714545
0.89 0.0136170525268988
0.9 0.0140146123184398
0.91 0.0144452625048971
0.92 0.0149163344683054
0.93 0.0154379852724437
0.94 0.0160248867469395
0.95 0.0166994406260456
0.96 0.0174985142721893
0.97 0.0184897771468976
0.98 0.0198211344425246
0.99 0.0219467843289148
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 6.97958182699385e-05
0.02 0.000139602607891579
0.03 0.000209431338301142
0.04 0.000279293022304417
0.05 0.000349198653110238
0.06 0.000419159409160239
0.07 0.000489186364494626
0.08 0.000559290748487836
0.09 0.000629483896211866
0.1 0.00069977718054405
0.11 0.000770182196942541
0.12 0.00084071056054806
0.13 0.00091137393541289
0.14 0.000982184554221975
0.15 0.00105315418881409
0.16 0.00112429529642417
0.17 0.00119562040162534
0.18 0.00126714224926586
0.19 0.00133887368920432
0.2 0.00141082788853319
0.21 0.0014830183299986
0.22 0.00155545930471824
0.23 0.00162816410719719
0.24 0.00170114756014352
0.25 0.00177442446160704
0.26 0.00184800999911177
0.27 0.00192191945378808
0.28 0.00199616904708506
0.29 0.00207077534095057
0.3 0.00214575503181706
0.31 0.00222112609435436
0.32 0.00229690601149449
0.33 0.00237311382916322
0.34 0.00244976851040732
0.35 0.00252689054665084
0.36 0.00260450002461468
0.37 0.00268261877957424
0.38 0.00276126912218902
0.39 0.00284047427405681
0.4 0.00292025795375498
0.41 0.00300064557527006
0.42 0.00308166378651599
0.43 0.0031633397021638
0.44 0.00324570155741858
0.45 0.00332877960854228
0.46 0.00341260534636693
0.47 0.00349721161474343
0.48 0.00358263284049727
0.49 0.00366890536089219
0.5 0.00375606795837605
0.51 0.00384416026781128
0.52 0.00393322595445826
0.53 0.00402330864741586
0.54 0.00411445682770905
0.55 0.00420672103203885
0.56 0.00430015452141124
0.57 0.00439481478033847
0.58 0.00449076203237899
0.59 0.00458806158866707
0.6 0.00468678208118939
0.61 0.0047869983409298
0.62 0.00488878925664499
0.63 0.00499224036643187
0.64 0.00509744412959769
0.65 0.00520449828008624
0.66 0.005313512568048
0.67 0.00542460140235569
0.68 0.00553789211946747
0.69 0.00565352280542125
0.7 0.00577164326581155
0.71 0.0058924195833732
0.72 0.0060160331498435
0.73 0.00614268487462321
0.74 0.00627259646363112
0.75 0.006406013587333
0.76 0.00654321381878198
0.77 0.00668450408151641
0.78 0.00683023475821897
0.79 0.00698079873696145
0.8 0.00713664649207236
0.81 0.00729829363549444
0.82 0.00746633569959152
0.83 0.00764146649156714
0.84 0.00782449890667157
0.85 0.00801639747459626
0.86 0.00821831762842404
0.87 0.00843166174574166
0.88 0.00865815272055738
0.89 0.00889994570604359
0.9 0.00915978610936693
0.91 0.00944125403346305
0.92 0.00974914164285686
0.93 0.0100900856202186
0.94 0.0104736787701513
0.95 0.0109145595305245
0.96 0.0114368242421633
0.97 0.0120847020521609
0.98 0.0129548607076581
0.99 0.0143441617655253
};
\addplot [semithick, crimson2143940]
table {%
0.01 6.40179244092634e-05
0.02 0.000128045917713182
0.03 0.000192094025372801
0.04 0.00025617234129957
0.05 0.000320291019662528
0.06 0.000384460237405445
0.07 0.000448690146993023
0.08 0.000512991102957829
0.09 0.000577373495551935
0.1 0.000641847697534503
0.11 0.000706424389047783
0.12 0.000771114212729756
0.13 0.000835927929126782
0.14 0.000900876512821126
0.15 0.00096597113252449
0.16 0.00103122296881756
0.17 0.0010966435120972
0.18 0.00116224466022191
0.19 0.00122803791484688
0.2 0.00129403562242964
0.21 0.00136024999346988
0.22 0.00142669396183819
0.23 0.00149338025713868
0.24 0.00156032175897243
0.25 0.00162753266200206
0.26 0.00169502651720157
0.27 0.00176281751646398
0.28 0.00183092052073246
0.29 0.00189935070530808
0.3 0.00196812347416099
0.31 0.00203725498705661
0.32 0.00210676180027322
0.33 0.00217666071219875
0.34 0.0022469698950653
0.35 0.00231770732971331
0.36 0.0023888922100922
0.37 0.00246054396054256
0.38 0.00253268341188519
0.39 0.00260533170174918
0.4 0.00267851099718521
0.41 0.00275224369799634
0.42 0.00282655523490165
0.43 0.00290146945509093
0.44 0.00297701310113782
0.45 0.00305321403203195
0.46 0.00313010025361819
0.47 0.00320770248891833
0.48 0.00328605245191685
0.49 0.00336518318895861
0.5 0.00344513007525578
0.51 0.00352593010833996
0.52 0.00360762239287592
0.53 0.00369024782920512
0.54 0.00377385078677915
0.55 0.00385847679917894
0.56 0.00394417561389351
0.57 0.0040309998134345
0.58 0.00411900425200529
0.59 0.0042082488205794
0.6 0.0042987972665508
0.61 0.0043907172321031
0.62 0.0044840816364296
0.63 0.00457896878394596
0.64 0.00467546332899997
0.65 0.00477365534123985
0.66 0.00487364491283184
0.67 0.00497553764410542
0.68 0.00507944988777602
0.69 0.0051855082771061
0.7 0.00529385036585484
0.71 0.00540462839409624
0.72 0.00551800931002598
0.73 0.00563417595725804
0.74 0.0057533332070977
0.75 0.00587570599787072
0.76 0.00600154811548212
0.77 0.006131142192196
0.78 0.00626480886514647
0.79 0.00640290801897514
0.8 0.00654585536962483
0.81 0.00669412026537959
0.82 0.00684825147182285
0.83 0.0070088842813009
0.84 0.00717676538653959
0.85 0.0073527781396163
0.86 0.0075379825811029
0.87 0.0077336653135785
0.88 0.00794140680068795
0.89 0.00816318303083285
0.9 0.00840151358101758
0.91 0.00865968110607471
0.92 0.00894208043772987
0.93 0.00925480016651537
0.94 0.00960663781743114
0.95 0.0100110213342725
0.96 0.0104900519254981
0.97 0.0110842956709516
0.98 0.0118824213662506
0.99 0.0131567111846551
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/nerfacto-laplace/empirical_coverage.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.05, ymax=1.05,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 1
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.00037814116432142
0.02 0.000755830072978924
0.03 0.00113508577811896
0.04 0.00151648856357501
0.05 0.00189657743076169
0.06 0.00227717089708319
0.07 0.00265780913654432
0.08 0.00303860534041014
0.09 0.00342183387054013
0.1 0.00380477980971366
0.11 0.00418972169344814
0.12 0.00457369911411319
0.13 0.00495966701966969
0.14 0.00534637628044907
0.15 0.00573245638684873
0.16 0.00611962798806919
0.17 0.00650844294764526
0.18 0.00689655514256927
0.19 0.00728710976353989
0.2 0.00767991025093654
0.21 0.00807396784341517
0.22 0.00846986813409657
0.23 0.00886613805425555
0.24 0.00926369037266561
0.25 0.00966167795763392
0.26 0.0100623295639596
0.27 0.0104646666798409
0.28 0.0108701491522219
0.29 0.0112746522208668
0.3 0.0116842561761544
0.31 0.0120956643291291
0.32 0.0125080534130468
0.33 0.012922104295638
0.34 0.0133398949581346
0.35 0.0137599705744872
0.36 0.014182174784157
0.37 0.0146074027843263
0.38 0.0150363304255627
0.39 0.0154690443191752
0.4 0.0159035022321058
0.41 0.0163417659170245
0.42 0.0167807535330627
0.43 0.0172247013304841
0.44 0.0176705300251886
0.45 0.0181201375359193
0.46 0.018579505717125
0.47 0.0190402411434762
0.48 0.0195046400641149
0.49 0.0199730459274289
0.5 0.0204449030953921
0.51 0.0209238373011609
0.52 0.0214094981814623
0.53 0.021898984262113
0.54 0.0223935614756317
0.55 0.0228930035756236
0.56 0.0234003889846543
0.57 0.0239151918566123
0.58 0.0244364996844491
0.59 0.0249621319121638
0.6 0.025497858156186
0.61 0.0260413092170158
0.62 0.0265931233904107
0.63 0.0271511917772153
0.64 0.0277212146657906
0.65 0.0283021252606194
0.66 0.0288913989953861
0.67 0.0294935516327465
0.68 0.0301065133143786
0.69 0.030729421659424
0.7 0.0313682204263831
0.71 0.0320190630408676
0.72 0.0326866752858394
0.73 0.0333725944561305
0.74 0.0340740210230203
0.75 0.0347933381130718
0.76 0.035531522562002
0.77 0.0362936529947803
0.78 0.037078859508242
0.79 0.0378879293799339
0.8 0.0387247121822133
0.81 0.0395938971054823
0.82 0.0404962453221044
0.83 0.0414341403226066
0.84 0.0424149999951745
0.85 0.0434449153170604
0.86 0.0445249525785814
0.87 0.0456685875068438
0.88 0.0468788491575007
0.89 0.0481697381524294
0.9 0.049556016733883
0.91 0.0510543153575168
0.92 0.0526942357360444
0.93 0.0545028219064909
0.94 0.0565400637169898
0.95 0.058874485512515
0.96 0.0616351359371941
0.97 0.0650407875706055
0.98 0.0696064021987781
0.99 0.0768584644315835
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.000367399761573194
0.02 0.000734639363036068
0.03 0.00110068286481864
0.04 0.00147006224598053
0.05 0.00183935001781382
0.06 0.00220936644719233
0.07 0.00258018805330974
0.08 0.00294963840561582
0.09 0.00332230088227562
0.1 0.00369687278125201
0.11 0.00407024454830951
0.12 0.00444408261701103
0.13 0.00481776989701158
0.14 0.00519500044025068
0.15 0.00557187012738393
0.16 0.00595044968804241
0.17 0.00632986366318033
0.18 0.00671094090464243
0.19 0.00709323744943637
0.2 0.00747632247936251
0.21 0.00786066230500273
0.22 0.00824843727927873
0.23 0.00863513879257546
0.24 0.00902383705725219
0.25 0.00941524452753146
0.26 0.00980762808085219
0.27 0.0102019292250128
0.28 0.0105981175250476
0.29 0.0109972904362339
0.3 0.0113974475884176
0.31 0.0118001000817758
0.32 0.0122054986826166
0.33 0.0126117268950529
0.34 0.0130205773969011
0.35 0.0134333535736006
0.36 0.0138480303585429
0.37 0.0142670942739217
0.38 0.0146880211738294
0.39 0.015110944394286
0.4 0.0155376912610065
0.41 0.015970071533617
0.42 0.0164057482621382
0.43 0.0168429785354559
0.44 0.0172833980188511
0.45 0.0177284283111697
0.46 0.0181769309946237
0.47 0.0186299475513865
0.48 0.0190856432511017
0.49 0.0195488921188858
0.5 0.0200134472442111
0.51 0.0204823242163775
0.52 0.0209590748764448
0.53 0.021440188254017
0.54 0.0219285468117416
0.55 0.0224234878798114
0.56 0.02292774780785
0.57 0.0234349829708261
0.58 0.0239489673721557
0.59 0.0244709231800082
0.6 0.0249971603513484
0.61 0.0255345434309736
0.62 0.0260790241927983
0.63 0.0266302437820226
0.64 0.0271916641226985
0.65 0.0277649494432454
0.66 0.0283502774366046
0.67 0.028943852089906
0.68 0.0295504782606683
0.69 0.0301690585437528
0.7 0.0308012253797921
0.71 0.0314467637415632
0.72 0.0321091569073335
0.73 0.0327869263905576
0.74 0.033478735018497
0.75 0.0341893605041789
0.76 0.0349216157928015
0.77 0.0356749844269135
0.78 0.0364539537461675
0.79 0.0372573540485744
0.8 0.0380875874835936
0.81 0.0389481134360232
0.82 0.0398456789230327
0.83 0.0407796291913894
0.84 0.0417543700362452
0.85 0.0427724057490737
0.86 0.0438465497071009
0.87 0.0449796424034933
0.88 0.0461828867018365
0.89 0.0474662575320832
0.9 0.0488463988768952
0.91 0.0503404545738154
0.92 0.051969118713226
0.93 0.0537676869301953
0.94 0.0557920268334033
0.95 0.0581138878375881
0.96 0.0608603886828259
0.97 0.0642570078249221
0.98 0.068812500182422
0.99 0.0760548082832234
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.00036294166697893
0.02 0.000727815427616006
0.03 0.00109240214627246
0.04 0.00145681456575261
0.05 0.00182276229963349
0.06 0.00218861653820055
0.07 0.00255558775185035
0.08 0.00292307681561652
0.09 0.00329085272314208
0.1 0.00365898618568347
0.11 0.00402791143914605
0.12 0.00439726606502977
0.13 0.00476876352691428
0.14 0.00514066190601282
0.15 0.00551292166293093
0.16 0.00588758057338353
0.17 0.00626419143654949
0.18 0.00664070342148719
0.19 0.00701978250113672
0.2 0.00739862914673728
0.21 0.00777869316281234
0.22 0.00816057526440596
0.23 0.00854269789459294
0.24 0.00892724552376211
0.25 0.00931660954478444
0.26 0.00970749349069052
0.27 0.0100988023710972
0.28 0.0104921547430835
0.29 0.0108873273409469
0.3 0.0112857300372856
0.31 0.0116846736192747
0.32 0.0120863645963318
0.33 0.012491116303367
0.34 0.0128997041623894
0.35 0.0133105358044971
0.36 0.0137234353622244
0.37 0.0141395760245488
0.38 0.0145566255945641
0.39 0.014976842605047
0.4 0.0154001120679971
0.41 0.0158273077393794
0.42 0.0162581521648454
0.43 0.0166918363171446
0.44 0.017129634553383
0.45 0.0175732436586831
0.46 0.0180186261452719
0.47 0.0184671846539683
0.48 0.0189213538679008
0.49 0.0193799227069413
0.5 0.0198439209024855
0.51 0.0203124793994768
0.52 0.0207853162609908
0.53 0.0212632119824677
0.54 0.0217484570313494
0.55 0.0222407212147017
0.56 0.022738292694581
0.57 0.0232402682224687
0.58 0.0237489514932626
0.59 0.0242653160222867
0.6 0.0247868862377942
0.61 0.0253171422186502
0.62 0.0258582699884766
0.63 0.026407035684893
0.64 0.0269647991427731
0.65 0.0275311120477582
0.66 0.028106682602247
0.67 0.0286962106998856
0.68 0.0292959894675004
0.69 0.0299084812771661
0.7 0.0305351250363721
0.71 0.0311769635158924
0.72 0.0318334501996377
0.73 0.0325045547780485
0.74 0.0331935556705175
0.75 0.0338998603015756
0.76 0.0346274086193956
0.77 0.0353738922891186
0.78 0.0361476235296986
0.79 0.0369425453389707
0.8 0.0377698871869566
0.81 0.0386231540363454
0.82 0.0395140913970654
0.83 0.0404401092023593
0.84 0.0414110746605409
0.85 0.0424272312767468
0.86 0.0434963709928338
0.87 0.0446288541737136
0.88 0.045827312333098
0.89 0.0471040607797234
0.9 0.0484791087135136
0.91 0.0499677873930057
0.92 0.0515933408784352
0.93 0.0533900751639236
0.94 0.0554143866329746
0.95 0.0577367773743174
0.96 0.0604855340504448
0.97 0.0638842879981031
0.98 0.0684349060374093
0.99 0.0756619299154587
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.000385586052893187
0.02 0.000774830072292603
0.03 0.00116455055085382
0.04 0.00155553540760761
0.05 0.00194318751669756
0.06 0.00233201250332926
0.07 0.00272182094237123
0.08 0.00311121426337346
0.09 0.00350099009275276
0.1 0.00389053692647368
0.11 0.00428193346315669
0.12 0.00467094957911745
0.13 0.005063805035165
0.14 0.0054536975193775
0.15 0.00584624036350607
0.16 0.00623889986294819
0.17 0.00663321176732662
0.18 0.00702906964083998
0.19 0.0074240118326079
0.2 0.00781990814005725
0.21 0.00821853761675287
0.22 0.00861654389984682
0.23 0.0090180704138172
0.24 0.00941928896393027
0.25 0.00982375325137267
0.26 0.0102283296035882
0.27 0.0106341242087553
0.28 0.0110427184068576
0.29 0.011454929551935
0.3 0.0118678274000244
0.31 0.0122821636321762
0.32 0.0126989818797356
0.33 0.0131183333461411
0.34 0.0135405105554278
0.35 0.0139641647731716
0.36 0.0143896830727589
0.37 0.0148185364329378
0.38 0.0152511982514773
0.39 0.0156860192555346
0.4 0.0161260068501778
0.41 0.0165673791305803
0.42 0.0170133403649031
0.43 0.0174591448288839
0.44 0.0179122010348539
0.45 0.0183659027876156
0.46 0.0188245954336037
0.47 0.0192893184182572
0.48 0.019756865326766
0.49 0.0202284524928598
0.5 0.0207060647745485
0.51 0.0211883113718295
0.52 0.021674103620478
0.53 0.022166491107505
0.54 0.0226627580808503
0.55 0.0231683375143624
0.56 0.0236784909368926
0.57 0.0241942887288913
0.58 0.0247166271764182
0.59 0.0252482934655241
0.6 0.0257846571616771
0.61 0.0263289649747943
0.62 0.0268810776750544
0.63 0.0274421591442911
0.64 0.0280130974709845
0.65 0.0285943333603039
0.66 0.0291870599836927
0.67 0.029790602226117
0.68 0.0304018172589419
0.69 0.0310314549496127
0.7 0.0316730655200731
0.71 0.0323259894288187
0.72 0.0329940555450008
0.73 0.0336790096213287
0.74 0.0343793595715194
0.75 0.035097152255645
0.76 0.0358368132374494
0.77 0.0365971560206097
0.78 0.0373814333405415
0.79 0.0381887186302942
0.8 0.0390285948121841
0.81 0.0398956974772409
0.82 0.0407994879664862
0.83 0.0417366725379284
0.84 0.0427174576890422
0.85 0.0437461177633586
0.86 0.0448264960276913
0.87 0.0459697241145058
0.88 0.047179470230338
0.89 0.0484698570591677
0.9 0.0498529461541185
0.91 0.0513601004716673
0.92 0.0529993782812271
0.93 0.0548150314916762
0.94 0.0568535227194623
0.95 0.0591977351136427
0.96 0.0619684340389412
0.97 0.0653955031044428
0.98 0.0699835240404794
0.99 0.0772547304734061
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/nerfacto-laplace/empirical_coverage_absolute_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.0457169035042271, ymax=0.960054973588768,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.00962185883567859
0.02 0.0192441699270211
0.03 0.0288649142218811
0.04 0.0384835114364249
0.05 0.0481034225692382
0.06 0.0577228291029167
0.07 0.0673421908634556
0.08 0.0769613946595898
0.09 0.0865781661294598
0.1 0.0961952201902863
0.11 0.105810278306552
0.12 0.115426300885887
0.13 0.12504033298033
0.14 0.134653623719551
0.15 0.144267543613151
0.16 0.153880372011931
0.17 0.163491557052355
0.18 0.173103444857431
0.19 0.18271289023646
0.2 0.192320089749063
0.21 0.201926032156585
0.22 0.211530131865903
0.23 0.221133861945744
0.24 0.230736309627334
0.25 0.240338322042366
0.26 0.24993767043604
0.27 0.259535333320159
0.28 0.269129850847778
0.29 0.278725347779133
0.3 0.288315743823846
0.31 0.297904335670871
0.32 0.307491946586953
0.33 0.317077895704362
0.34 0.326660105041865
0.35 0.336240029425513
0.36 0.345817825215843
0.37 0.355392597215674
0.38 0.364963669574437
0.39 0.374530955680825
0.4 0.384096497767894
0.41 0.393658234082976
0.42 0.403219246466937
0.43 0.412775298669516
0.44 0.422329469974811
0.45 0.431879862464081
0.46 0.441420494282875
0.47 0.450959758856524
0.48 0.460495359935885
0.49 0.470026954072571
0.5 0.479555096904608
0.51 0.489076162698839
0.52 0.498590501818538
0.53 0.508101015737887
0.54 0.517606438524368
0.55 0.527106996424376
0.56 0.536599611015346
0.57 0.546084808143388
0.58 0.555563500315551
0.59 0.565037868087836
0.6 0.574502141843814
0.61 0.583958690782984
0.62 0.593406876609589
0.63 0.602848808222785
0.64 0.612278785334209
0.65 0.621697874739381
0.66 0.631108601004614
0.67 0.640506448367253
0.68 0.649893486685621
0.69 0.659270578340576
0.7 0.668631779573617
0.71 0.677980936959132
0.72 0.687313324714161
0.73 0.696627405543869
0.74 0.70592597897698
0.75 0.715206661886928
0.76 0.724468477437998
0.77 0.73370634700522
0.78 0.742921140491758
0.79 0.752112070620066
0.8 0.761275287817787
0.81 0.770406102894518
0.82 0.779503754677896
0.83 0.788565859677393
0.84 0.797585000004825
0.85 0.80655508468294
0.86 0.815475047421419
0.87 0.824331412493156
0.88 0.833121150842499
0.89 0.841830261847571
0.9 0.850443983266117
0.91 0.858945684642483
0.92 0.867305764263956
0.93 0.875497178093509
0.94 0.88345993628301
0.95 0.891125514487485
0.96 0.898364864062806
0.97 0.904959212429394
0.98 0.910393597801222
0.99 0.913141535568416
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.00963260023842682
0.02 0.0192653606369639
0.03 0.0288993171351814
0.04 0.0385299377540194
0.05 0.0481606499821861
0.06 0.0577906335528076
0.07 0.0674198119466902
0.08 0.0770503615943841
0.09 0.0866776991177243
0.1 0.096303127218748
0.11 0.10592975545169
0.12 0.115555917382989
0.13 0.125182230102988
0.14 0.134804999559749
0.15 0.144428129872616
0.16 0.154049550311958
0.17 0.16367013633682
0.18 0.173289059095358
0.19 0.182906762550564
0.2 0.192523677520637
0.21 0.202139337694997
0.22 0.211751562720721
0.23 0.221364861207425
0.24 0.230976162942748
0.25 0.240584755472469
0.26 0.250192371919148
0.27 0.259798070774987
0.28 0.269401882474952
0.29 0.279002709563766
0.3 0.288602552411582
0.31 0.298199899918224
0.32 0.307794501317383
0.33 0.317388273104947
0.34 0.326979422603099
0.35 0.336566646426399
0.36 0.346151969641457
0.37 0.355732905726078
0.38 0.365311978826171
0.39 0.374889055605714
0.4 0.384462308738994
0.41 0.394029928466383
0.42 0.403594251737862
0.43 0.413157021464544
0.44 0.422716601981149
0.45 0.43227157168883
0.46 0.441823069005376
0.47 0.451370052448614
0.48 0.460914356748898
0.49 0.470451107881114
0.5 0.479986552755789
0.51 0.489517675783623
0.52 0.499040925123555
0.53 0.508559811745983
0.54 0.518071453188259
0.55 0.527576512120189
0.56 0.53707225219215
0.57 0.546565017029174
0.58 0.556051032627844
0.59 0.565529076819992
0.6 0.575002839648652
0.61 0.584465456569026
0.62 0.593920975807202
0.63 0.603369756217977
0.64 0.612808335877301
0.65 0.622235050556755
0.66 0.631649722563395
0.67 0.641056147910094
0.68 0.650449521739332
0.69 0.659830941456247
0.7 0.669198774620208
0.71 0.678553236258437
0.72 0.687890843092667
0.73 0.697213073609442
0.74 0.706521264981503
0.75 0.715810639495821
0.76 0.725078384207199
0.77 0.734325015573087
0.78 0.743546046253833
0.79 0.752742645951426
0.8 0.761912412516406
0.81 0.771051886563977
0.82 0.780154321076967
0.83 0.789220370808611
0.84 0.798245629963755
0.85 0.807227594250926
0.86 0.816153450292899
0.87 0.825020357596507
0.88 0.833817113298163
0.89 0.842533742467917
0.9 0.851153601123105
0.91 0.859659545426185
0.92 0.868030881286774
0.93 0.876232313069805
0.94 0.884207973166597
0.95 0.891886112162412
0.96 0.899139611317174
0.97 0.905742992175078
0.98 0.911187499817578
0.99 0.913945191716777
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.00963705833302108
0.02 0.019272184572384
0.03 0.0289075978537276
0.04 0.0385431854342473
0.05 0.0481772377003665
0.06 0.0578113834617994
0.07 0.0674444122481496
0.08 0.0770769231843834
0.09 0.0867091472768579
0.1 0.0963410138143165
0.11 0.105972088560854
0.12 0.11560273393497
0.13 0.125231236473086
0.14 0.134859338093987
0.15 0.144487078337069
0.16 0.154112419426616
0.17 0.16373580856345
0.18 0.173359296578513
0.19 0.182980217498863
0.2 0.192601370853263
0.21 0.202221306837188
0.22 0.211839424735594
0.23 0.221457302105407
0.24 0.231072754476238
0.25 0.240683390455216
0.26 0.250292506509309
0.27 0.259901197628903
0.28 0.269507845256917
0.29 0.279112672659053
0.3 0.288714269962714
0.31 0.298315326380725
0.32 0.307913635403668
0.33 0.317508883696633
0.34 0.327100295837611
0.35 0.336689464195503
0.36 0.346276564637776
0.37 0.355860423975451
0.38 0.365443374405436
0.39 0.375023157394953
0.4 0.384599887932003
0.41 0.394172692260621
0.42 0.403741847835154
0.43 0.413308163682855
0.44 0.422870365446617
0.45 0.432426756341317
0.46 0.441981373854728
0.47 0.451532815346032
0.48 0.461078646132099
0.49 0.470620077293059
0.5 0.480156079097514
0.51 0.489687520600523
0.52 0.499214683739009
0.53 0.508736788017532
0.54 0.518251542968651
0.55 0.527759278785298
0.56 0.537261707305419
0.57 0.546759731777531
0.58 0.556251048506737
0.59 0.565734683977713
0.6 0.575213113762206
0.61 0.58468285778135
0.62 0.594141730011523
0.63 0.603592964315107
0.64 0.613035200857227
0.65 0.622468887952242
0.66 0.631893317397753
0.67 0.641303789300114
0.68 0.650704010532499
0.69 0.660091518722834
0.7 0.669464874963628
0.71 0.678823036484108
0.72 0.688166549800362
0.73 0.697495445221952
0.74 0.706806444329483
0.75 0.716100139698424
0.76 0.725372591380604
0.77 0.734626107710881
0.78 0.743852376470301
0.79 0.753057454661029
0.8 0.762230112813043
0.81 0.771376845963655
0.82 0.780485908602935
0.83 0.789559890797641
0.84 0.798588925339459
0.85 0.807572768723253
0.86 0.816503629007166
0.87 0.825371145826286
0.88 0.834172687666902
0.89 0.842895939220277
0.9 0.851520891286486
0.91 0.860032212606994
0.92 0.868406659121565
0.93 0.876609924836076
0.94 0.884585613367025
0.95 0.892263222625682
0.96 0.899514465949555
0.97 0.906115712001897
0.98 0.911565093962591
0.99 0.914338070084541
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.00961441394710682
0.02 0.0192251699277074
0.03 0.0288354494491462
0.04 0.0384444645923923
0.05 0.0480568124833024
0.06 0.0576679874966707
0.07 0.0672781790576287
0.08 0.0768887857366265
0.09 0.0864990099072472
0.1 0.0961094630735263
0.11 0.105718066536843
0.12 0.115329050420883
0.13 0.124936194964835
0.14 0.134546302480622
0.15 0.144153759636494
0.16 0.153761100137052
0.17 0.163366788232673
0.18 0.17297093035916
0.19 0.182575988167392
0.2 0.192180091859943
0.21 0.201781462383247
0.22 0.211383456100153
0.23 0.220981929586183
0.24 0.23058071103607
0.25 0.240176246748627
0.26 0.249771670396412
0.27 0.259365875791245
0.28 0.268957281593142
0.29 0.278545070448065
0.3 0.288132172599975
0.31 0.297717836367824
0.32 0.307301018120264
0.33 0.316881666653859
0.34 0.326459489444572
0.35 0.336035835226828
0.36 0.345610316927241
0.37 0.355181463567062
0.38 0.364748801748523
0.39 0.374313980744465
0.4 0.383873993149822
0.41 0.39343262086942
0.42 0.402986659635097
0.43 0.412540855171116
0.44 0.422087798965146
0.45 0.431634097212384
0.46 0.441175404566396
0.47 0.450710681581743
0.48 0.460243134673234
0.49 0.46977154750714
0.5 0.479293935225452
0.51 0.48881168862817
0.52 0.498325896379522
0.53 0.507833508892495
0.54 0.51733724191915
0.55 0.526831662485638
0.56 0.536321509063107
0.57 0.545805711271109
0.58 0.555283372823582
0.59 0.564751706534476
0.6 0.574215342838323
0.61 0.583671035025206
0.62 0.593118922324946
0.63 0.602557840855709
0.64 0.611986902529015
0.65 0.621405666639696
0.66 0.630812940016307
0.67 0.640209397773883
0.68 0.649598182741058
0.69 0.658968545050387
0.7 0.668326934479927
0.71 0.677674010571181
0.72 0.687005944454999
0.73 0.696320990378671
0.74 0.705620640428481
0.75 0.714902847744355
0.76 0.724163186762551
0.77 0.73340284397939
0.78 0.742618566659458
0.79 0.751811281369706
0.8 0.760971405187816
0.81 0.770104302522759
0.82 0.779200512033514
0.83 0.788263327462072
0.84 0.797282542310958
0.85 0.806253882236641
0.86 0.815173503972309
0.87 0.824030275885494
0.88 0.832820529769662
0.89 0.841530142940833
0.9 0.850147053845881
0.91 0.858639899528333
0.92 0.867000621718773
0.93 0.875184968508324
0.94 0.883146477280538
0.95 0.890802264886357
0.96 0.898031565961059
0.97 0.904604496895557
0.98 0.910016475959521
0.99 0.912745269526594
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/nerfacto-laplace/empirical_coverage_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.960054973588768, ymax=0.0457169035042271,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 -0.00962185883567859
0.02 -0.0192441699270211
0.03 -0.0288649142218811
0.04 -0.0384835114364249
0.05 -0.0481034225692382
0.06 -0.0577228291029167
0.07 -0.0673421908634556
0.08 -0.0769613946595898
0.09 -0.0865781661294598
0.1 -0.0961952201902863
0.11 -0.105810278306552
0.12 -0.115426300885887
0.13 -0.12504033298033
0.14 -0.134653623719551
0.15 -0.144267543613151
0.16 -0.153880372011931
0.17 -0.163491557052355
0.18 -0.173103444857431
0.19 -0.18271289023646
0.2 -0.192320089749063
0.21 -0.201926032156585
0.22 -0.211530131865903
0.23 -0.221133861945744
0.24 -0.230736309627334
0.25 -0.240338322042366
0.26 -0.24993767043604
0.27 -0.259535333320159
0.28 -0.269129850847778
0.29 -0.278725347779133
0.3 -0.288315743823846
0.31 -0.297904335670871
0.32 -0.307491946586953
0.33 -0.317077895704362
0.34 -0.326660105041865
0.35 -0.336240029425513
0.36 -0.345817825215843
0.37 -0.355392597215674
0.38 -0.364963669574437
0.39 -0.374530955680825
0.4 -0.384096497767894
0.41 -0.393658234082976
0.42 -0.403219246466937
0.43 -0.412775298669516
0.44 -0.422329469974811
0.45 -0.431879862464081
0.46 -0.441420494282875
0.47 -0.450959758856524
0.48 -0.460495359935885
0.49 -0.470026954072571
0.5 -0.479555096904608
0.51 -0.489076162698839
0.52 -0.498590501818538
0.53 -0.508101015737887
0.54 -0.517606438524368
0.55 -0.527106996424376
0.56 -0.536599611015346
0.57 -0.546084808143388
0.58 -0.555563500315551
0.59 -0.565037868087836
0.6 -0.574502141843814
0.61 -0.583958690782984
0.62 -0.593406876609589
0.63 -0.602848808222785
0.64 -0.612278785334209
0.65 -0.621697874739381
0.66 -0.631108601004614
0.67 -0.640506448367253
0.68 -0.649893486685621
0.69 -0.659270578340576
0.7 -0.668631779573617
0.71 -0.677980936959132
0.72 -0.687313324714161
0.73 -0.696627405543869
0.74 -0.70592597897698
0.75 -0.715206661886928
0.76 -0.724468477437998
0.77 -0.73370634700522
0.78 -0.742921140491758
0.79 -0.752112070620066
0.8 -0.761275287817787
0.81 -0.770406102894518
0.82 -0.779503754677896
0.83 -0.788565859677393
0.84 -0.797585000004825
0.85 -0.80655508468294
0.86 -0.815475047421419
0.87 -0.824331412493156
0.88 -0.833121150842499
0.89 -0.841830261847571
0.9 -0.850443983266117
0.91 -0.858945684642483
0.92 -0.867305764263956
0.93 -0.875497178093509
0.94 -0.88345993628301
0.95 -0.891125514487485
0.96 -0.898364864062806
0.97 -0.904959212429394
0.98 -0.910393597801222
0.99 -0.913141535568416
};
\addplot [semithick, darkorange25512714]
table {%
0.01 -0.00963260023842682
0.02 -0.0192653606369639
0.03 -0.0288993171351814
0.04 -0.0385299377540194
0.05 -0.0481606499821861
0.06 -0.0577906335528076
0.07 -0.0674198119466902
0.08 -0.0770503615943841
0.09 -0.0866776991177243
0.1 -0.096303127218748
0.11 -0.10592975545169
0.12 -0.115555917382989
0.13 -0.125182230102988
0.14 -0.134804999559749
0.15 -0.144428129872616
0.16 -0.154049550311958
0.17 -0.16367013633682
0.18 -0.173289059095358
0.19 -0.182906762550564
0.2 -0.192523677520637
0.21 -0.202139337694997
0.22 -0.211751562720721
0.23 -0.221364861207425
0.24 -0.230976162942748
0.25 -0.240584755472469
0.26 -0.250192371919148
0.27 -0.259798070774987
0.28 -0.269401882474952
0.29 -0.279002709563766
0.3 -0.288602552411582
0.31 -0.298199899918224
0.32 -0.307794501317383
0.33 -0.317388273104947
0.34 -0.326979422603099
0.35 -0.336566646426399
0.36 -0.346151969641457
0.37 -0.355732905726078
0.38 -0.365311978826171
0.39 -0.374889055605714
0.4 -0.384462308738994
0.41 -0.394029928466383
0.42 -0.403594251737862
0.43 -0.413157021464544
0.44 -0.422716601981149
0.45 -0.43227157168883
0.46 -0.441823069005376
0.47 -0.451370052448614
0.48 -0.460914356748898
0.49 -0.470451107881114
0.5 -0.479986552755789
0.51 -0.489517675783623
0.52 -0.499040925123555
0.53 -0.508559811745983
0.54 -0.518071453188259
0.55 -0.527576512120189
0.56 -0.53707225219215
0.57 -0.546565017029174
0.58 -0.556051032627844
0.59 -0.565529076819992
0.6 -0.575002839648652
0.61 -0.584465456569026
0.62 -0.593920975807202
0.63 -0.603369756217977
0.64 -0.612808335877301
0.65 -0.622235050556755
0.66 -0.631649722563395
0.67 -0.641056147910094
0.68 -0.650449521739332
0.69 -0.659830941456247
0.7 -0.669198774620208
0.71 -0.678553236258437
0.72 -0.687890843092667
0.73 -0.697213073609442
0.74 -0.706521264981503
0.75 -0.715810639495821
0.76 -0.725078384207199
0.77 -0.734325015573087
0.78 -0.743546046253833
0.79 -0.752742645951426
0.8 -0.761912412516406
0.81 -0.771051886563977
0.82 -0.780154321076967
0.83 -0.789220370808611
0.84 -0.798245629963755
0.85 -0.807227594250926
0.86 -0.816153450292899
0.87 -0.825020357596507
0.88 -0.833817113298163
0.89 -0.842533742467917
0.9 -0.851153601123105
0.91 -0.859659545426185
0.92 -0.868030881286774
0.93 -0.876232313069805
0.94 -0.884207973166597
0.95 -0.891886112162412
0.96 -0.899139611317174
0.97 -0.905742992175078
0.98 -0.911187499817578
0.99 -0.913945191716777
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 -0.00963705833302108
0.02 -0.019272184572384
0.03 -0.0289075978537276
0.04 -0.0385431854342473
0.05 -0.0481772377003665
0.06 -0.0578113834617994
0.07 -0.0674444122481496
0.08 -0.0770769231843834
0.09 -0.0867091472768579
0.1 -0.0963410138143165
0.11 -0.105972088560854
0.12 -0.11560273393497
0.13 -0.125231236473086
0.14 -0.134859338093987
0.15 -0.144487078337069
0.16 -0.154112419426616
0.17 -0.16373580856345
0.18 -0.173359296578513
0.19 -0.182980217498863
0.2 -0.192601370853263
0.21 -0.202221306837188
0.22 -0.211839424735594
0.23 -0.221457302105407
0.24 -0.231072754476238
0.25 -0.240683390455216
0.26 -0.250292506509309
0.27 -0.259901197628903
0.28 -0.269507845256917
0.29 -0.279112672659053
0.3 -0.288714269962714
0.31 -0.298315326380725
0.32 -0.307913635403668
0.33 -0.317508883696633
0.34 -0.327100295837611
0.35 -0.336689464195503
0.36 -0.346276564637776
0.37 -0.355860423975451
0.38 -0.365443374405436
0.39 -0.375023157394953
0.4 -0.384599887932003
0.41 -0.394172692260621
0.42 -0.403741847835154
0.43 -0.413308163682855
0.44 -0.422870365446617
0.45 -0.432426756341317
0.46 -0.441981373854728
0.47 -0.451532815346032
0.48 -0.461078646132099
0.49 -0.470620077293059
0.5 -0.480156079097514
0.51 -0.489687520600523
0.52 -0.499214683739009
0.53 -0.508736788017532
0.54 -0.518251542968651
0.55 -0.527759278785298
0.56 -0.537261707305419
0.57 -0.546759731777531
0.58 -0.556251048506737
0.59 -0.565734683977713
0.6 -0.575213113762206
0.61 -0.58468285778135
0.62 -0.594141730011523
0.63 -0.603592964315107
0.64 -0.613035200857227
0.65 -0.622468887952242
0.66 -0.631893317397753
0.67 -0.641303789300114
0.68 -0.650704010532499
0.69 -0.660091518722834
0.7 -0.669464874963628
0.71 -0.678823036484108
0.72 -0.688166549800362
0.73 -0.697495445221952
0.74 -0.706806444329483
0.75 -0.716100139698424
0.76 -0.725372591380604
0.77 -0.734626107710881
0.78 -0.743852376470301
0.79 -0.753057454661029
0.8 -0.762230112813043
0.81 -0.771376845963655
0.82 -0.780485908602935
0.83 -0.789559890797641
0.84 -0.798588925339459
0.85 -0.807572768723253
0.86 -0.816503629007166
0.87 -0.825371145826286
0.88 -0.834172687666902
0.89 -0.842895939220277
0.9 -0.851520891286486
0.91 -0.860032212606994
0.92 -0.868406659121565
0.93 -0.876609924836076
0.94 -0.884585613367025
0.95 -0.892263222625682
0.96 -0.899514465949555
0.97 -0.906115712001897
0.98 -0.911565093962591
0.99 -0.914338070084541
};
\addplot [semithick, crimson2143940]
table {%
0.01 -0.00961441394710682
0.02 -0.0192251699277074
0.03 -0.0288354494491462
0.04 -0.0384444645923923
0.05 -0.0480568124833024
0.06 -0.0576679874966707
0.07 -0.0672781790576287
0.08 -0.0768887857366265
0.09 -0.0864990099072472
0.1 -0.0961094630735263
0.11 -0.105718066536843
0.12 -0.115329050420883
0.13 -0.124936194964835
0.14 -0.134546302480622
0.15 -0.144153759636494
0.16 -0.153761100137052
0.17 -0.163366788232673
0.18 -0.17297093035916
0.19 -0.182575988167392
0.2 -0.192180091859943
0.21 -0.201781462383247
0.22 -0.211383456100153
0.23 -0.220981929586183
0.24 -0.23058071103607
0.25 -0.240176246748627
0.26 -0.249771670396412
0.27 -0.259365875791245
0.28 -0.268957281593142
0.29 -0.278545070448065
0.3 -0.288132172599975
0.31 -0.297717836367824
0.32 -0.307301018120264
0.33 -0.316881666653859
0.34 -0.326459489444572
0.35 -0.336035835226828
0.36 -0.345610316927241
0.37 -0.355181463567062
0.38 -0.364748801748523
0.39 -0.374313980744465
0.4 -0.383873993149822
0.41 -0.39343262086942
0.42 -0.402986659635097
0.43 -0.412540855171116
0.44 -0.422087798965146
0.45 -0.431634097212384
0.46 -0.441175404566396
0.47 -0.450710681581743
0.48 -0.460243134673234
0.49 -0.46977154750714
0.5 -0.479293935225452
0.51 -0.48881168862817
0.52 -0.498325896379522
0.53 -0.507833508892495
0.54 -0.51733724191915
0.55 -0.526831662485638
0.56 -0.536321509063107
0.57 -0.545805711271109
0.58 -0.555283372823582
0.59 -0.564751706534476
0.6 -0.574215342838323
0.61 -0.583671035025206
0.62 -0.593118922324946
0.63 -0.602557840855709
0.64 -0.611986902529015
0.65 -0.621405666639696
0.66 -0.630812940016307
0.67 -0.640209397773883
0.68 -0.649598182741058
0.69 -0.658968545050387
0.7 -0.668326934479927
0.71 -0.677674010571181
0.72 -0.687005944454999
0.73 -0.696320990378671
0.74 -0.705620640428481
0.75 -0.714902847744355
0.76 -0.724163186762551
0.77 -0.73340284397939
0.78 -0.742618566659458
0.79 -0.751811281369706
0.8 -0.760971405187816
0.81 -0.770104302522759
0.82 -0.779200512033514
0.83 -0.788263327462072
0.84 -0.797282542310958
0.85 -0.806253882236641
0.86 -0.815173503972309
0.87 -0.824030275885494
0.88 -0.832820529769662
0.89 -0.841530142940833
0.9 -0.850147053845881
0.91 -0.858639899528333
0.92 -0.867000621718773
0.93 -0.875184968508324
0.94 -0.883146477280538
0.95 -0.890802264886357
0.96 -0.898031565961059
0.97 -0.904604496895557
0.98 -0.910016475959521
0.99 -0.912745269526594
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/nerfacto-laplace/empirical_coverage_negative_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.0457169035042271, ymax=0.960054973588768,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.00962185883567859
0.02 0.0192441699270211
0.03 0.0288649142218811
0.04 0.0384835114364249
0.05 0.0481034225692382
0.06 0.0577228291029167
0.07 0.0673421908634556
0.08 0.0769613946595898
0.09 0.0865781661294598
0.1 0.0961952201902863
0.11 0.105810278306552
0.12 0.115426300885887
0.13 0.12504033298033
0.14 0.134653623719551
0.15 0.144267543613151
0.16 0.153880372011931
0.17 0.163491557052355
0.18 0.173103444857431
0.19 0.18271289023646
0.2 0.192320089749063
0.21 0.201926032156585
0.22 0.211530131865903
0.23 0.221133861945744
0.24 0.230736309627334
0.25 0.240338322042366
0.26 0.24993767043604
0.27 0.259535333320159
0.28 0.269129850847778
0.29 0.278725347779133
0.3 0.288315743823846
0.31 0.297904335670871
0.32 0.307491946586953
0.33 0.317077895704362
0.34 0.326660105041865
0.35 0.336240029425513
0.36 0.345817825215843
0.37 0.355392597215674
0.38 0.364963669574437
0.39 0.374530955680825
0.4 0.384096497767894
0.41 0.393658234082976
0.42 0.403219246466937
0.43 0.412775298669516
0.44 0.422329469974811
0.45 0.431879862464081
0.46 0.441420494282875
0.47 0.450959758856524
0.48 0.460495359935885
0.49 0.470026954072571
0.5 0.479555096904608
0.51 0.489076162698839
0.52 0.498590501818538
0.53 0.508101015737887
0.54 0.517606438524368
0.55 0.527106996424376
0.56 0.536599611015346
0.57 0.546084808143388
0.58 0.555563500315551
0.59 0.565037868087836
0.6 0.574502141843814
0.61 0.583958690782984
0.62 0.593406876609589
0.63 0.602848808222785
0.64 0.612278785334209
0.65 0.621697874739381
0.66 0.631108601004614
0.67 0.640506448367253
0.68 0.649893486685621
0.69 0.659270578340576
0.7 0.668631779573617
0.71 0.677980936959132
0.72 0.687313324714161
0.73 0.696627405543869
0.74 0.70592597897698
0.75 0.715206661886928
0.76 0.724468477437998
0.77 0.73370634700522
0.78 0.742921140491758
0.79 0.752112070620066
0.8 0.761275287817787
0.81 0.770406102894518
0.82 0.779503754677896
0.83 0.788565859677393
0.84 0.797585000004825
0.85 0.80655508468294
0.86 0.815475047421419
0.87 0.824331412493156
0.88 0.833121150842499
0.89 0.841830261847571
0.9 0.850443983266117
0.91 0.858945684642483
0.92 0.867305764263956
0.93 0.875497178093509
0.94 0.88345993628301
0.95 0.891125514487485
0.96 0.898364864062806
0.97 0.904959212429394
0.98 0.910393597801222
0.99 0.913141535568416
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.00963260023842682
0.02 0.0192653606369639
0.03 0.0288993171351814
0.04 0.0385299377540194
0.05 0.0481606499821861
0.06 0.0577906335528076
0.07 0.0674198119466902
0.08 0.0770503615943841
0.09 0.0866776991177243
0.1 0.096303127218748
0.11 0.10592975545169
0.12 0.115555917382989
0.13 0.125182230102988
0.14 0.134804999559749
0.15 0.144428129872616
0.16 0.154049550311958
0.17 0.16367013633682
0.18 0.173289059095358
0.19 0.182906762550564
0.2 0.192523677520637
0.21 0.202139337694997
0.22 0.211751562720721
0.23 0.221364861207425
0.24 0.230976162942748
0.25 0.240584755472469
0.26 0.250192371919148
0.27 0.259798070774987
0.28 0.269401882474952
0.29 0.279002709563766
0.3 0.288602552411582
0.31 0.298199899918224
0.32 0.307794501317383
0.33 0.317388273104947
0.34 0.326979422603099
0.35 0.336566646426399
0.36 0.346151969641457
0.37 0.355732905726078
0.38 0.365311978826171
0.39 0.374889055605714
0.4 0.384462308738994
0.41 0.394029928466383
0.42 0.403594251737862
0.43 0.413157021464544
0.44 0.422716601981149
0.45 0.43227157168883
0.46 0.441823069005376
0.47 0.451370052448614
0.48 0.460914356748898
0.49 0.470451107881114
0.5 0.479986552755789
0.51 0.489517675783623
0.52 0.499040925123555
0.53 0.508559811745983
0.54 0.518071453188259
0.55 0.527576512120189
0.56 0.53707225219215
0.57 0.546565017029174
0.58 0.556051032627844
0.59 0.565529076819992
0.6 0.575002839648652
0.61 0.584465456569026
0.62 0.593920975807202
0.63 0.603369756217977
0.64 0.612808335877301
0.65 0.622235050556755
0.66 0.631649722563395
0.67 0.641056147910094
0.68 0.650449521739332
0.69 0.659830941456247
0.7 0.669198774620208
0.71 0.678553236258437
0.72 0.687890843092667
0.73 0.697213073609442
0.74 0.706521264981503
0.75 0.715810639495821
0.76 0.725078384207199
0.77 0.734325015573087
0.78 0.743546046253833
0.79 0.752742645951426
0.8 0.761912412516406
0.81 0.771051886563977
0.82 0.780154321076967
0.83 0.789220370808611
0.84 0.798245629963755
0.85 0.807227594250926
0.86 0.816153450292899
0.87 0.825020357596507
0.88 0.833817113298163
0.89 0.842533742467917
0.9 0.851153601123105
0.91 0.859659545426185
0.92 0.868030881286774
0.93 0.876232313069805
0.94 0.884207973166597
0.95 0.891886112162412
0.96 0.899139611317174
0.97 0.905742992175078
0.98 0.911187499817578
0.99 0.913945191716777
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.00963705833302108
0.02 0.019272184572384
0.03 0.0289075978537276
0.04 0.0385431854342473
0.05 0.0481772377003665
0.06 0.0578113834617994
0.07 0.0674444122481496
0.08 0.0770769231843834
0.09 0.0867091472768579
0.1 0.0963410138143165
0.11 0.105972088560854
0.12 0.11560273393497
0.13 0.125231236473086
0.14 0.134859338093987
0.15 0.144487078337069
0.16 0.154112419426616
0.17 0.16373580856345
0.18 0.173359296578513
0.19 0.182980217498863
0.2 0.192601370853263
0.21 0.202221306837188
0.22 0.211839424735594
0.23 0.221457302105407
0.24 0.231072754476238
0.25 0.240683390455216
0.26 0.250292506509309
0.27 0.259901197628903
0.28 0.269507845256917
0.29 0.279112672659053
0.3 0.288714269962714
0.31 0.298315326380725
0.32 0.307913635403668
0.33 0.317508883696633
0.34 0.327100295837611
0.35 0.336689464195503
0.36 0.346276564637776
0.37 0.355860423975451
0.38 0.365443374405436
0.39 0.375023157394953
0.4 0.384599887932003
0.41 0.394172692260621
0.42 0.403741847835154
0.43 0.413308163682855
0.44 0.422870365446617
0.45 0.432426756341317
0.46 0.441981373854728
0.47 0.451532815346032
0.48 0.461078646132099
0.49 0.470620077293059
0.5 0.480156079097514
0.51 0.489687520600523
0.52 0.499214683739009
0.53 0.508736788017532
0.54 0.518251542968651
0.55 0.527759278785298
0.56 0.537261707305419
0.57 0.546759731777531
0.58 0.556251048506737
0.59 0.565734683977713
0.6 0.575213113762206
0.61 0.58468285778135
0.62 0.594141730011523
0.63 0.603592964315107
0.64 0.613035200857227
0.65 0.622468887952242
0.66 0.631893317397753
0.67 0.641303789300114
0.68 0.650704010532499
0.69 0.660091518722834
0.7 0.669464874963628
0.71 0.678823036484108
0.72 0.688166549800362
0.73 0.697495445221952
0.74 0.706806444329483
0.75 0.716100139698424
0.76 0.725372591380604
0.77 0.734626107710881
0.78 0.743852376470301
0.79 0.753057454661029
0.8 0.762230112813043
0.81 0.771376845963655
0.82 0.780485908602935
0.83 0.789559890797641
0.84 0.798588925339459
0.85 0.807572768723253
0.86 0.816503629007166
0.87 0.825371145826286
0.88 0.834172687666902
0.89 0.842895939220277
0.9 0.851520891286486
0.91 0.860032212606994
0.92 0.868406659121565
0.93 0.876609924836076
0.94 0.884585613367025
0.95 0.892263222625682
0.96 0.899514465949555
0.97 0.906115712001897
0.98 0.911565093962591
0.99 0.914338070084541
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.00961441394710682
0.02 0.0192251699277074
0.03 0.0288354494491462
0.04 0.0384444645923923
0.05 0.0480568124833024
0.06 0.0576679874966707
0.07 0.0672781790576287
0.08 0.0768887857366265
0.09 0.0864990099072472
0.1 0.0961094630735263
0.11 0.105718066536843
0.12 0.115329050420883
0.13 0.124936194964835
0.14 0.134546302480622
0.15 0.144153759636494
0.16 0.153761100137052
0.17 0.163366788232673
0.18 0.17297093035916
0.19 0.182575988167392
0.2 0.192180091859943
0.21 0.201781462383247
0.22 0.211383456100153
0.23 0.220981929586183
0.24 0.23058071103607
0.25 0.240176246748627
0.26 0.249771670396412
0.27 0.259365875791245
0.28 0.268957281593142
0.29 0.278545070448065
0.3 0.288132172599975
0.31 0.297717836367824
0.32 0.307301018120264
0.33 0.316881666653859
0.34 0.326459489444572
0.35 0.336035835226828
0.36 0.345610316927241
0.37 0.355181463567062
0.38 0.364748801748523
0.39 0.374313980744465
0.4 0.383873993149822
0.41 0.39343262086942
0.42 0.402986659635097
0.43 0.412540855171116
0.44 0.422087798965146
0.45 0.431634097212384
0.46 0.441175404566396
0.47 0.450710681581743
0.48 0.460243134673234
0.49 0.46977154750714
0.5 0.479293935225452
0.51 0.48881168862817
0.52 0.498325896379522
0.53 0.507833508892495
0.54 0.51733724191915
0.55 0.526831662485638
0.56 0.536321509063107
0.57 0.545805711271109
0.58 0.555283372823582
0.59 0.564751706534476
0.6 0.574215342838323
0.61 0.583671035025206
0.62 0.593118922324946
0.63 0.602557840855709
0.64 0.611986902529015
0.65 0.621405666639696
0.66 0.630812940016307
0.67 0.640209397773883
0.68 0.649598182741058
0.69 0.658968545050387
0.7 0.668326934479927
0.71 0.677674010571181
0.72 0.687005944454999
0.73 0.696320990378671
0.74 0.705620640428481
0.75 0.714902847744355
0.76 0.724163186762551
0.77 0.73340284397939
0.78 0.742618566659458
0.79 0.751811281369706
0.8 0.760971405187816
0.81 0.770104302522759
0.82 0.779200512033514
0.83 0.788263327462072
0.84 0.797282542310958
0.85 0.806253882236641
0.86 0.815173503972309
0.87 0.824030275885494
0.88 0.832820529769662
0.89 0.841530142940833
0.9 0.850147053845881
0.91 0.858639899528333
0.92 0.867000621718773
0.93 0.875184968508324
0.94 0.883146477280538
0.95 0.890802264886357
0.96 0.898031565961059
0.97 0.904604496895557
0.98 0.910016475959521
0.99 0.912745269526594
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/nerfacto-mcdropout/avg_length.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.039, xmax=1.039,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.00462847360129746, ymax=0.102565193180104,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.01 0.000475353356115454
0.02 0.000950781458091979
0.03 0.00142635896197614
0.04 0.00190216087725041
0.05 0.00237826218445331
0.06 0.00285473895877646
0.07 0.00333166646590267
0.08 0.00380912177340553
0.09 0.00428718086019102
0.1 0.00476592250676205
0.11 0.00524542497627891
0.12 0.00572576713274926
0.13 0.00620702955387107
0.14 0.00668929370128853
0.15 0.00717264127047273
0.16 0.00765715755687993
0.17 0.00814292614224347
0.18 0.00863003455074312
0.19 0.0091185709160218
0.2 0.00960862472465661
0.21 0.0101002874725481
0.22 0.0105936550292721
0.23 0.0110888213475554
0.24 0.0115858838779171
0.25 0.0120849451634893
0.26 0.0125861088833884
0.27 0.0130894791625037
0.28 0.0135951656407098
0.29 0.0141032821129133
0.3 0.0146139411419874
0.31 0.0151272640572666
0.32 0.0156433734838543
0.33 0.0161623953904358
0.34 0.0166844612916784
0.35 0.0172097123213132
0.36 0.0177382809355283
0.37 0.0182703191562774
0.38 0.0188059773594706
0.39 0.0193454138348
0.4 0.0198887915276117
0.41 0.0204362815140978
0.42 0.0209880659111812
0.43 0.0215443305091246
0.44 0.0221052664743525
0.45 0.0226710808501736
0.46 0.0232419862938817
0.47 0.0238182094529316
0.48 0.024399981051317
0.49 0.0249875514755805
0.5 0.0255811832850967
0.51 0.0261811486397259
0.52 0.0267877402938963
0.53 0.0274012593363514
0.54 0.0280220357786204
0.55 0.0286504133886639
0.56 0.0292867542182167
0.57 0.0299314504970421
0.58 0.0305849108685564
0.59 0.0312475820589983
0.6 0.0319199303029379
0.61 0.0326024662928553
0.62 0.0332957273856148
0.63 0.0340002931025876
0.64 0.0347167955700952
0.65 0.035445904184201
0.66 0.036188357938853
0.67 0.0369449433516974
0.68 0.0377165239651962
0.69 0.0385040414531669
0.7 0.0393085160545669
0.71 0.0401310769191793
0.72 0.0409729664910427
0.73 0.0418355402066896
0.74 0.0427203216575024
0.75 0.0436289786860104
0.76 0.0445633938818611
0.77 0.0455256733724745
0.78 0.0465181881927949
0.79 0.0475436252909931
0.8 0.0486050455192531
0.81 0.0497059652007772
0.82 0.0508504399539815
0.83 0.0520431879555189
0.84 0.0532897577325713
0.85 0.054596702646466
0.86 0.0559719096941042
0.87 0.0574249133060542
0.88 0.0589674624501697
0.89 0.0606142259887884
0.9 0.062383897679986
0.91 0.0643008737496959
0.92 0.066397780295281
0.93 0.0687198243653044
0.94 0.0713323298226568
0.95 0.074335005255034
0.96 0.0778919579918198
0.97 0.0823044090962245
0.98 0.0882307412723209
0.99 0.0976927537809492
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.000361792070745338
0.02 0.000723641000286808
0.03 0.00108560367977364
0.04 0.00144773712918834
0.05 0.00181009852172886
0.06 0.00217274556602542
0.07 0.00253573581891842
0.08 0.00289912742854148
0.09 0.00326297904006452
0.1 0.00362734970253011
0.11 0.00399229931108182
0.12 0.00435788907950059
0.13 0.004724178325078
0.14 0.00509123004029179
0.15 0.00545910684501847
0.16 0.00582787247043714
0.17 0.00619759153415478
0.18 0.00656833058208406
0.19 0.0069401560697931
0.2 0.00731313641576923
0.21 0.00768734187945803
0.22 0.00806284486002355
0.23 0.00843971616058812
0.24 0.00881803070928463
0.25 0.009197868471775
0.26 0.00957930422815031
0.27 0.00996241907940465
0.28 0.0103472982508662
0.29 0.0107340264459447
0.3 0.0111226890173281
0.31 0.011513380107996
0.32 0.0119061913311185
0.33 0.0123012200886192
0.34 0.0126985665314058
0.35 0.013098333666796
0.36 0.0135006298724742
0.37 0.013905563601139
0.38 0.0143132537750933
0.39 0.014723819376803
0.4 0.0151373856854608
0.41 0.0155540813276242
0.42 0.015974044930213
0.43 0.0163974181278497
0.44 0.0168243463201057
0.45 0.0172549884702993
0.46 0.0176895061926809
0.47 0.0181280699671166
0.48 0.0185708575601976
0.49 0.0190180574620861
0.5 0.019469872079873
0.51 0.0199265064604318
0.52 0.0203881836473418
0.53 0.0208551344641506
0.54 0.0213276081849687
0.55 0.0218058666095125
0.56 0.0222901867247497
0.57 0.0227808662798089
0.58 0.0232782152456968
0.59 0.0237825761948249
0.6 0.0242943016857602
0.61 0.0248137797474087
0.62 0.0253414204609845
0.63 0.0258776672203249
0.64 0.0264229975092793
0.65 0.0269779247725482
0.66 0.027543007360406
0.67 0.0281188442440372
0.68 0.0287060968287464
0.69 0.0293054774601529
0.7 0.0299177635110853
0.71 0.0305438156041563
0.72 0.031184578058591
0.73 0.0318410859238541
0.74 0.0325144929164664
0.75 0.0332060712351049
0.76 0.033917257185402
0.77 0.034649649141975
0.78 0.0354050562075475
0.79 0.0361855151675117
0.8 0.0369933650430712
0.81 0.0378312741484788
0.82 0.0387023345634977
0.83 0.0396101388768906
0.84 0.0405589011284212
0.85 0.0415536235294406
0.86 0.0426002932516876
0.87 0.0437061784990696
0.88 0.0448802111687648
0.89 0.0461335632120762
0.9 0.0474804687059858
0.91 0.0489394779951958
0.92 0.0505354353411185
0.93 0.0523027489641329
0.94 0.054291127197094
0.95 0.0565764677991222
0.96 0.0592836698780621
0.97 0.0626419946991111
0.98 0.0671525314658709
0.99 0.0743540810091088
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.000279654942978416
0.02 0.000559353887735316
0.03 0.000839140767268592
0.04 0.00111905951399359
0.05 0.00139915459277964
0.06 0.00167947046604843
0.07 0.00196005156419384
0.08 0.00224094292694391
0.09 0.00252218987503518
0.1 0.00280383803752034
0.11 0.00308593391797509
0.12 0.00336852395609945
0.13 0.00365165521403891
0.14 0.0039353755412051
0.15 0.0042197342362594
0.16 0.0045047796001968
0.17 0.00479056172384127
0.18 0.00507713265348348
0.19 0.00536454327697361
0.2 0.00565284608553853
0.21 0.00594209667988419
0.22 0.00623234920903996
0.23 0.00652366031977081
0.24 0.0068160872749842
0.25 0.0071096899006069
0.26 0.00740452939992696
0.27 0.00770066641760389
0.28 0.00799816709601524
0.29 0.00829709660942914
0.3 0.00859752210348217
0.31 0.00889951526147723
0.32 0.00920314770660441
0.33 0.00950849344031205
0.34 0.00981563034813409
0.35 0.0101246392776137
0.36 0.0104356021526235
0.37 0.0107486048377711
0.38 0.0110637378513579
0.39 0.0113810934926844
0.4 0.0117007676369944
0.41 0.0120228619032439
0.42 0.0123474824844183
0.43 0.0126747377620689
0.44 0.0130047416029051
0.45 0.013337615911393
0.46 0.0136734845808894
0.47 0.0140124819087184
0.48 0.0143547447634979
0.49 0.0147004181520092
0.5 0.0150496564210874
0.51 0.0154026220652148
0.52 0.0157594865248544
0.53 0.0161204253529192
0.54 0.0164856345042597
0.55 0.0168553155567207
0.56 0.0172296806843581
0.57 0.0176089618347612
0.58 0.0179933984896692
0.59 0.01838325352415
0.6 0.0187788039361631
0.61 0.019180345406897
0.62 0.0195881973248225
0.63 0.0200027001420539
0.64 0.0204242253615677
0.65 0.0208531678572596
0.66 0.0212899605107575
0.67 0.0217350667726424
0.68 0.0221889958232356
0.69 0.0226523001949093
0.7 0.0231255790381152
0.71 0.0236095020077268
0.72 0.0241047918819752
0.73 0.0246122536191307
0.74 0.0251327776769529
0.75 0.0256673485818569
0.76 0.0262170748577847
0.77 0.0267831932706978
0.78 0.0273671007983924
0.79 0.0279703721211083
0.8 0.0285948182682348
0.81 0.0292424966306621
0.82 0.0299158048729829
0.83 0.0306175102949453
0.84 0.0313508768510264
0.85 0.0321197667740599
0.86 0.0329288142815302
0.87 0.0337836310727057
0.88 0.0346911255215249
0.89 0.0356599307203032
0.9 0.0367010497757991
0.91 0.037828823627316
0.92 0.0390624524034278
0.93 0.0404285363696385
0.94 0.0419654991737018
0.95 0.0437320005318399
0.96 0.0458245879894349
0.97 0.0484204796328003
0.98 0.0519069926907193
0.99 0.0574735872814102
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.000243965797857146
0.02 0.000487969964188514
0.03 0.000732050861389501
0.04 0.000976246839761334
0.05 0.00122059656359114
0.06 0.00146513893997482
0.07 0.00170991280450259
0.08 0.00195495732046925
0.09 0.00220031172840102
0.1 0.0024460165449652
0.11 0.0026921116373039
0.12 0.00293863803777392
0.13 0.00318563653690077
0.14 0.00343314908486062
0.15 0.00368121804395257
0.16 0.00392988612059482
0.17 0.00417919755909296
0.18 0.00442919656031018
0.19 0.00467992825976311
0.2 0.00493143833451044
0.21 0.005183774953603
0.22 0.00543698639818836
0.23 0.00569112044927224
0.24 0.00594622825643982
0.25 0.00620236218025092
0.26 0.00645957456218122
0.27 0.00671791900717055
0.28 0.00697745309386876
0.29 0.00723823345085356
0.3 0.00750031960978363
0.31 0.00776377241504153
0.32 0.00802865547117633
0.33 0.00829503343580968
0.34 0.00856297417927415
0.35 0.00883254793782451
0.36 0.00910382617902136
0.37 0.00937688406900725
0.38 0.00965179982464883
0.39 0.0099286553776832
0.4 0.0102075331056209
0.41 0.0104885220128715
0.42 0.0107717147040801
0.43 0.0110572066347021
0.44 0.0113450957011228
0.45 0.0116354894961228
0.46 0.011928494857061
0.47 0.0122242301474908
0.48 0.0125228132297946
0.49 0.0128243725513633
0.5 0.0131290414970553
0.51 0.0134369619975037
0.52 0.0137482836319946
0.53 0.0140631612022012
0.54 0.0143817624902192
0.55 0.0147042643156951
0.56 0.0150308537403372
0.57 0.0153617312694324
0.58 0.015697107748025
0.59 0.0160372102094764
0.6 0.0163822807449046
0.61 0.0167325791377894
0.62 0.0170883803824987
0.63 0.0174499851075954
0.64 0.017817716242501
0.65 0.0181919185060038
0.66 0.0185729674643546
0.67 0.0189612699789044
0.68 0.0193572700925242
0.69 0.019761447028996
0.7 0.0201743275949716
0.71 0.0205964921111079
0.72 0.0210285741803215
0.73 0.0214712736861024
0.74 0.021925370622285
0.75 0.0223917200926093
0.76 0.0228712921029779
0.77 0.0233651632679686
0.78 0.0238745504063801
0.79 0.0244008360498691
0.8 0.0249455904389751
0.81 0.0255106146869988
0.82 0.0260979922132209
0.83 0.0267101494733363
0.84 0.027349925677907
0.85 0.0280206922505853
0.86 0.0287264884152962
0.87 0.0294722155907218
0.88 0.0302638949954428
0.89 0.0311090652005388
0.9 0.0320173177981032
0.91 0.0330011669497062
0.92 0.0340773624698616
0.93 0.0352691074569091
0.94 0.0366099238540987
0.95 0.0381509886456028
0.96 0.039976522691476
0.97 0.0422411282724196
0.98 0.0452827016565689
0.99 0.0501388950554981
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/nerfacto-mcdropout/empirical_coverage.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.05, ymax=1.05,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 1
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.00109300901222881
0.02 0.00217971071370254
0.03 0.00326732378166644
0.04 0.00435579714893314
0.05 0.00544210788340257
0.06 0.0065319228323264
0.07 0.00761824680971003
0.08 0.00870736236339196
0.09 0.0097952385048846
0.1 0.0108880973233545
0.11 0.0119830545156304
0.12 0.0130764064794331
0.13 0.0141750233188692
0.14 0.0152746702622769
0.15 0.0163796629388865
0.16 0.0174852978660286
0.17 0.0185935258362347
0.18 0.0197059716315143
0.19 0.0208226825284992
0.2 0.0219408521468941
0.21 0.0230609247709025
0.22 0.024186136232048
0.23 0.0253170141636427
0.24 0.0264477668016951
0.25 0.0275867675485842
0.26 0.02872716887182
0.27 0.0298761843008669
0.28 0.0310290980316266
0.29 0.032183336560087
0.3 0.033347219368137
0.31 0.0345177817505761
0.32 0.03569119922835
0.33 0.0368729147632807
0.34 0.0380630387283896
0.35 0.0392616262338124
0.36 0.0404650424553336
0.37 0.0416763415795921
0.38 0.0428950199147615
0.39 0.044124186472933
0.4 0.0453605496380127
0.41 0.0466052738602312
0.42 0.0478571904617093
0.43 0.0491208644441051
0.44 0.0503947663807217
0.45 0.0516773006091374
0.46 0.0529720786404276
0.47 0.0542779412679284
0.48 0.0555959198820947
0.49 0.0569277949496417
0.5 0.0582720363768674
0.51 0.0596308557376566
0.52 0.0610006168720089
0.53 0.0623888493235491
0.54 0.0637958530907719
0.55 0.0652165249109784
0.56 0.0666530691437181
0.57 0.0681130105762512
0.58 0.0695868710467541
0.59 0.0710837281217761
0.6 0.0725989836568631
0.61 0.0741340672283297
0.62 0.0756954317469741
0.63 0.0772821882712487
0.64 0.0788950915755934
0.65 0.0805325535002703
0.66 0.0821953173118713
0.67 0.0838879240658052
0.68 0.0856184632704655
0.69 0.0873844341711065
0.7 0.0891823730240835
0.71 0.0910206109121701
0.72 0.0928979413404045
0.73 0.094822416820929
0.74 0.0967922616280104
0.75 0.098814090669217
0.76 0.100888296368559
0.77 0.103024699309039
0.78 0.105225031277153
0.79 0.107492372494217
0.8 0.109835934921424
0.81 0.11226158743121
0.82 0.114782491715812
0.83 0.117401228884167
0.84 0.120131848931718
0.85 0.12299302110906
0.86 0.125999075722861
0.87 0.129170624115522
0.88 0.132525096633262
0.89 0.136101622657191
0.9 0.139926442942648
0.91 0.144059773787428
0.92 0.148559961392467
0.93 0.153537130281561
0.94 0.159101125212734
0.95 0.165459241468442
0.96 0.172944845293944
0.97 0.182150129061739
0.98 0.194380573840001
0.99 0.213576252218674
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.00110953540041035
0.02 0.00222038430190046
0.03 0.00332791727421956
0.04 0.00443958589145554
0.05 0.0055540351772983
0.06 0.00666937974505028
0.07 0.00778408908532483
0.08 0.00890328862519913
0.09 0.0100216455645269
0.1 0.0111438679633077
0.11 0.0122704512938929
0.12 0.0133943474638181
0.13 0.0145214226955066
0.14 0.0156523249708181
0.15 0.0167873750331505
0.16 0.017922438040264
0.17 0.0190636415663093
0.18 0.0202096978245487
0.19 0.0213547964135601
0.2 0.0225078824611743
0.21 0.0236627007993472
0.22 0.0248178616067636
0.23 0.0259801242381147
0.24 0.0271483647441691
0.25 0.0283176379373465
0.26 0.0294907883665664
0.27 0.0306755383317633
0.28 0.0318625161533389
0.29 0.0330594161310542
0.3 0.0342594458933949
0.31 0.0354672002428207
0.32 0.0366821490096841
0.33 0.037906070945896
0.34 0.0391347904297107
0.35 0.040370742376453
0.36 0.0416142660874585
0.37 0.0428646232757939
0.38 0.0441242950220349
0.39 0.0453899770811507
0.4 0.0466667756188042
0.41 0.0479522241395451
0.42 0.0492474910667338
0.43 0.0505543687229333
0.44 0.0518696713799294
0.45 0.0531982522284875
0.46 0.05453967666404
0.47 0.0558903037080472
0.48 0.0572527997630426
0.49 0.0586293970429032
0.5 0.0600178964831634
0.51 0.0614216496006821
0.52 0.062841865005707
0.53 0.0642770587331854
0.54 0.0657250778289238
0.55 0.0671946066019727
0.56 0.0686773750062947
0.57 0.0701808536473198
0.58 0.0717036601635601
0.59 0.073244083092022
0.6 0.0748076888264147
0.61 0.0763943650146626
0.62 0.0780086905678564
0.63 0.0796459494301939
0.64 0.0813049742656454
0.65 0.0829937866846527
0.66 0.0847119267121834
0.67 0.0864645981496395
0.68 0.0882489371195407
0.69 0.0900628083985954
0.7 0.0919182374939594
0.71 0.0938122101833794
0.72 0.0957489195687272
0.73 0.0977289652470782
0.74 0.0997587184871615
0.75 0.101838145300961
0.76 0.103972994630334
0.77 0.106170585585525
0.78 0.10843341183733
0.79 0.110763466780479
0.8 0.113168315910164
0.81 0.115655584402542
0.82 0.118243822669714
0.83 0.120932556287789
0.84 0.12373963756387
0.85 0.12667100029471
0.86 0.12974609799476
0.87 0.132988098138169
0.88 0.136422765773795
0.89 0.140077496748081
0.9 0.143981340808704
0.91 0.148200226320794
0.92 0.152787153223059
0.93 0.15784442020525
0.94 0.163505830455204
0.95 0.169964223174389
0.96 0.17756003013218
0.97 0.186886680879192
0.98 0.199247534131495
0.99 0.218590315126864
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.00316537781416682
0.02 0.004756127822959
0.03 0.00634612138562118
0.04 0.00793741643282517
0.05 0.00952946187447106
0.06 0.0111196305057652
0.07 0.0127131944702895
0.08 0.0143055770471324
0.09 0.0159037702406656
0.1 0.0175019838312005
0.11 0.0191009178131625
0.12 0.0207029175725869
0.13 0.0223061559229535
0.14 0.0239130477763979
0.15 0.0255231172656994
0.16 0.0271396344234935
0.17 0.0287629836328378
0.18 0.0303878641325008
0.19 0.032017805034956
0.2 0.0336525426510715
0.21 0.0352959679798495
0.22 0.0369430694778898
0.23 0.0386013172189139
0.24 0.0402682748398071
0.25 0.0419426877045159
0.26 0.0436267817237407
0.27 0.0453210671587974
0.28 0.0470228435975193
0.29 0.0487405116017623
0.3 0.0504721694741557
0.31 0.052216992057133
0.32 0.0539755483177592
0.33 0.0557400004194598
0.34 0.0574984991552493
0.35 0.0592569429668116
0.36 0.0610179747107388
0.37 0.0627837659155299
0.38 0.0645675658930783
0.39 0.0663562193360551
0.4 0.068158510496084
0.41 0.0699747528946967
0.42 0.0718058498572605
0.43 0.0736462165234518
0.44 0.0755019923958541
0.45 0.0773672872243511
0.46 0.0792491545861715
0.47 0.0811456006678339
0.48 0.0830568227266463
0.49 0.0849847863535769
0.5 0.086929643217981
0.51 0.0888907452888612
0.52 0.0908712547607768
0.53 0.0928747254412838
0.54 0.094900430202795
0.55 0.096947856619258
0.56 0.0990126120211637
0.57 0.101108160504671
0.58 0.103226615773999
0.59 0.105369866479215
0.6 0.107547213959588
0.61 0.109756362803069
0.62 0.111994213040246
0.63 0.11426812778252
0.64 0.116579245911218
0.65 0.118922791197199
0.66 0.121308140185172
0.67 0.123729569711802
0.68 0.126201435324509
0.69 0.128719198477195
0.7 0.131287215196801
0.71 0.133910292785836
0.72 0.136583626168368
0.73 0.139323566725891
0.74 0.142130174724481
0.75 0.145004927932407
0.76 0.147956408648868
0.77 0.150990454617564
0.78 0.154118986510208
0.79 0.157346035186616
0.8 0.160668257565637
0.81 0.164109165245279
0.82 0.167678891847272
0.83 0.171395230231913
0.84 0.175258813777722
0.85 0.179292418780845
0.86 0.183516537289132
0.87 0.187959317412973
0.88 0.192658497786485
0.89 0.197653128692536
0.9 0.20298927694211
0.91 0.208747162857745
0.92 0.2149998991839
0.93 0.221878816232159
0.94 0.22955913054402
0.95 0.23830577797946
0.96 0.248569095881467
0.97 0.261136202896557
0.98 0.277720271876664
0.99 0.303471697267542
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.00469960536354181
0.02 0.00642655960281116
0.03 0.00815435226578558
0.04 0.00988608098817103
0.05 0.0116202812088228
0.06 0.0133561258802317
0.07 0.0150944073851411
0.08 0.0168339121932732
0.09 0.0185771241651057
0.1 0.0203252942362732
0.11 0.0220762169880818
0.12 0.0238214625797949
0.13 0.025573439102436
0.14 0.0273323000165146
0.15 0.0290912798326214
0.16 0.0308556260094729
0.17 0.0326219660679284
0.18 0.0343979846294874
0.19 0.0361805771449961
0.2 0.0379679248787496
0.21 0.039767663285751
0.22 0.0415727819505683
0.23 0.043382241287209
0.24 0.0452023513444993
0.25 0.0470259554494309
0.26 0.0488590644148831
0.27 0.0507083962762454
0.28 0.0525622635730496
0.29 0.0544273753311283
0.3 0.0562997921679049
0.31 0.0581810139242054
0.32 0.0600802895034209
0.33 0.0619856986989884
0.34 0.0638977250093474
0.35 0.0658256245479467
0.36 0.0677662293903825
0.37 0.0697144217445628
0.38 0.0716733917392084
0.39 0.0736370251294637
0.4 0.0756180499309055
0.41 0.0776035846787253
0.42 0.079602814103612
0.43 0.0816273388564095
0.44 0.0836605977856735
0.45 0.0857005518694346
0.46 0.0877643446411578
0.47 0.0898374440482898
0.48 0.0919341606815205
0.49 0.0940487738037853
0.5 0.0961873074301877
0.51 0.0983385265274653
0.52 0.100511595683803
0.53 0.102707536029901
0.54 0.104924922623684
0.55 0.10716999970051
0.56 0.109440360396999
0.57 0.111731389130133
0.58 0.114053323809394
0.59 0.11640004119882
0.6 0.118777825012228
0.61 0.121197060162219
0.62 0.12364440358026
0.63 0.126126683040307
0.64 0.128644731444673
0.65 0.131203755417093
0.66 0.133805743696851
0.67 0.136451530532088
0.68 0.139141740265162
0.69 0.141884052820827
0.7 0.144680707144204
0.71 0.147536797640635
0.72 0.150451670225845
0.73 0.15342567398404
0.74 0.156474737882421
0.75 0.15959790790831
0.76 0.162798895101844
0.77 0.166089255088235
0.78 0.169468253138857
0.79 0.172950075975018
0.8 0.17654832683432
0.81 0.180270622377508
0.82 0.184130545370772
0.83 0.18814704481123
0.84 0.192309901979969
0.85 0.196653813885792
0.86 0.201204553303425
0.87 0.205990933309552
0.88 0.211046363003448
0.89 0.216403635932808
0.9 0.222129197678801
0.91 0.228293804838358
0.92 0.234982310558846
0.93 0.242336563319486
0.94 0.250531784180623
0.95 0.259850717077832
0.96 0.270752566438148
0.97 0.284064304800328
0.98 0.301571915883828
0.99 0.328641956389794
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/nerfacto-mcdropout/empirical_coverage_absolute_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.039392493546913, ymax=0.827242364485174,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.0089069909877712
0.02 0.0178202892862975
0.03 0.0267326762183336
0.04 0.0356442028510668
0.05 0.0445578921165974
0.06 0.0534680771676735
0.07 0.0623817531902899
0.08 0.071292637636608
0.09 0.0802047614951154
0.1 0.0891119026766454
0.11 0.0980169454843696
0.12 0.106923593520567
0.13 0.115824976681131
0.14 0.124725329737723
0.15 0.133620337061113
0.16 0.142514702133971
0.17 0.151406474163765
0.18 0.160294028368486
0.19 0.169177317471501
0.2 0.178059147853106
0.21 0.186939075229097
0.22 0.195813863767952
0.23 0.204682985836357
0.24 0.213552233198305
0.25 0.222413232451416
0.26 0.23127283112818
0.27 0.240123815699133
0.28 0.248970901968373
0.29 0.257816663439913
0.3 0.266652780631863
0.31 0.275482218249424
0.32 0.28430880077165
0.33 0.293127085236719
0.34 0.30193696127161
0.35 0.310738373766188
0.36 0.319534957544666
0.37 0.328323658420408
0.38 0.337104980085239
0.39 0.345875813527067
0.4 0.354639450361987
0.41 0.363394726139769
0.42 0.372142809538291
0.43 0.380879135555895
0.44 0.389605233619278
0.45 0.398322699390863
0.46 0.407027921359572
0.47 0.415722058732072
0.48 0.424404080117905
0.49 0.433072205050358
0.5 0.441727963623133
0.51 0.450369144262343
0.52 0.458999383127991
0.53 0.467611150676451
0.54 0.476204146909228
0.55 0.484783475089022
0.56 0.493346930856282
0.57 0.501886989423749
0.58 0.510413128953246
0.59 0.518916271878224
0.6 0.527401016343137
0.61 0.53586593277167
0.62 0.544304568253026
0.63 0.552717811728751
0.64 0.561104908424407
0.65 0.56946744649973
0.66 0.577804682688129
0.67 0.586112075934195
0.68 0.594381536729534
0.69 0.602615565828893
0.7 0.610817626975916
0.71 0.61897938908783
0.72 0.627102058659596
0.73 0.635177583179071
0.74 0.64320773837199
0.75 0.651185909330783
0.76 0.659111703631441
0.77 0.666975300690961
0.78 0.674774968722847
0.79 0.682507627505783
0.8 0.690164065078576
0.81 0.69773841256879
0.82 0.705217508284188
0.83 0.712598771115833
0.84 0.719868151068282
0.85 0.72700697889094
0.86 0.734000924277139
0.87 0.740829375884478
0.88 0.747474903366738
0.89 0.753898377342809
0.9 0.760073557057352
0.91 0.765940226212572
0.92 0.771440038607534
0.93 0.776462869718439
0.94 0.780898874787266
0.95 0.784540758531558
0.96 0.787055154706056
0.97 0.787849870938261
0.98 0.785619426159999
0.99 0.776423747781326
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.00889046459958966
0.02 0.0177796156980996
0.03 0.0266720827257805
0.04 0.0355604141085444
0.05 0.0444459648227016
0.06 0.0533306202549497
0.07 0.0622159109146751
0.08 0.0710967113748008
0.09 0.0799783544354731
0.1 0.0888561320366923
0.11 0.097729548706107
0.12 0.106605652536182
0.13 0.115478577304493
0.14 0.124347675029182
0.15 0.13321262496685
0.16 0.142077561959736
0.17 0.150936358433691
0.18 0.159790302175451
0.19 0.16864520358644
0.2 0.177492117538826
0.21 0.186337299200653
0.22 0.195182138393236
0.23 0.204019875761885
0.24 0.212851635255831
0.25 0.221682362062653
0.26 0.230509211633434
0.27 0.239324461668237
0.28 0.248137483846661
0.29 0.256940583868946
0.3 0.265740554106605
0.31 0.274532799757179
0.32 0.283317850990316
0.33 0.292093929054104
0.34 0.300865209570289
0.35 0.309629257623547
0.36 0.318385733912542
0.37 0.327135376724206
0.38 0.335875704977965
0.39 0.344610022918849
0.4 0.353333224381196
0.41 0.362047775860455
0.42 0.370752508933266
0.43 0.379445631277067
0.44 0.388130328620071
0.45 0.396801747771512
0.46 0.40546032333596
0.47 0.414109696291953
0.48 0.422747200236957
0.49 0.431370602957097
0.5 0.439982103516837
0.51 0.448578350399318
0.52 0.457158134994293
0.53 0.465722941266815
0.54 0.474274922171076
0.55 0.482805393398027
0.56 0.491322624993705
0.57 0.49981914635268
0.58 0.50829633983644
0.59 0.516755916907978
0.6 0.525192311173585
0.61 0.533605634985337
0.62 0.541991309432144
0.63 0.550354050569806
0.64 0.558695025734355
0.65 0.567006213315347
0.66 0.575288073287817
0.67 0.58353540185036
0.68 0.591751062880459
0.69 0.599937191601405
0.7 0.608081762506041
0.71 0.616187789816621
0.72 0.624251080431273
0.73 0.632271034752922
0.74 0.640241281512838
0.75 0.648161854699039
0.76 0.656027005369666
0.77 0.663829414414475
0.78 0.67156658816267
0.79 0.679236533219521
0.8 0.686831684089836
0.81 0.694344415597458
0.82 0.701756177330285
0.83 0.70906744371221
0.84 0.71626036243613
0.85 0.72332899970529
0.86 0.73025390200524
0.87 0.737011901861832
0.88 0.743577234226205
0.89 0.749922503251919
0.9 0.756018659191296
0.91 0.761799773679206
0.92 0.767212846776941
0.93 0.77215557979475
0.94 0.776494169544796
0.95 0.780035776825611
0.96 0.782439969867819
0.97 0.783113319120809
0.98 0.780752465868505
0.99 0.771409684873136
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.00940538940434523
0.02 0.0174648545421093
0.03 0.0255918913207862
0.04 0.0337620905270336
0.05 0.0420882383115108
0.06 0.0504171343928497
0.07 0.0587426016222465
0.08 0.0670702558006824
0.09 0.0753916636191729
0.1 0.083712108326889
0.11 0.092029226563326
0.12 0.100342110057223
0.13 0.108653432342574
0.14 0.116960020146389
0.15 0.125264012701966
0.16 0.133559684731022
0.17 0.141851105649346
0.18 0.150141200579462
0.19 0.158427278376694
0.2 0.166709443516292
0.21 0.174985858020361
0.22 0.183258596355167
0.23 0.191521839243551
0.24 0.199780394497496
0.25 0.208057312295484
0.26 0.216373218276259
0.27 0.224678932841203
0.28 0.232977156402481
0.29 0.241259488398238
0.3 0.249527830525844
0.31 0.257783007942867
0.32 0.266024451682241
0.33 0.27425999958054
0.34 0.282501500844751
0.35 0.290743057033188
0.36 0.298982025289261
0.37 0.30721623408447
0.38 0.315432434106922
0.39 0.323643780663945
0.4 0.331841489503916
0.41 0.340025247105303
0.42 0.348194150142739
0.43 0.356353783476548
0.44 0.364498007604146
0.45 0.372632712775649
0.46 0.380750845413828
0.47 0.388854399332166
0.48 0.396943177273354
0.49 0.405015213646423
0.5 0.413070356782019
0.51 0.421109254711139
0.52 0.429128745239223
0.53 0.437125274558716
0.54 0.445099569797205
0.55 0.453052143380742
0.56 0.460987387978836
0.57 0.468891839495329
0.58 0.476773384226001
0.59 0.484630133520785
0.6 0.492452786040412
0.61 0.500243637196931
0.62 0.508005786959754
0.63 0.51573187221748
0.64 0.523420754088782
0.65 0.531077208802801
0.66 0.538691859814828
0.67 0.546270430288198
0.68 0.553798564675491
0.69 0.561280801522805
0.7 0.568712784803199
0.71 0.576089707214165
0.72 0.583416373831632
0.73 0.590676433274109
0.74 0.597869825275519
0.75 0.604995072067593
0.76 0.612043591351132
0.77 0.619009545382436
0.78 0.625881013489792
0.79 0.632653964813384
0.8 0.639331742434363
0.81 0.645890834754721
0.82 0.652321108152728
0.83 0.658604769768087
0.84 0.664741186222278
0.85 0.670707581219155
0.86 0.676483462710868
0.87 0.682040682587027
0.88 0.687341502213515
0.89 0.692346871307464
0.9 0.69701072305789
0.91 0.701252837142256
0.92 0.7050001008161
0.93 0.708121183767841
0.94 0.710440869455979
0.95 0.71169422202054
0.96 0.711430904118533
0.97 0.708863797103443
0.98 0.702279728123336
0.99 0.686528302732458
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.0103196028695119
0.02 0.01806390737385
0.03 0.0259290460435708
0.04 0.0338646399155255
0.05 0.0418290556938511
0.06 0.0498251833351817
0.07 0.0578905195517762
0.08 0.0660213276629422
0.09 0.0741860605710628
0.1 0.0823445072008885
0.11 0.0904990279951558
0.12 0.0986588698132045
0.13 0.106810937430417
0.14 0.114955927923598
0.15 0.123101004816861
0.16 0.13124017486015
0.17 0.139378482278362
0.18 0.147509009190534
0.19 0.155631902119491
0.2 0.163749834528092
0.21 0.171857446043908
0.22 0.179959819756432
0.23 0.188059331810297
0.24 0.196148448723691
0.25 0.204232282528195
0.26 0.2123086770628
0.27 0.220371710361526
0.28 0.228425435998199
0.29 0.23646973556372
0.3 0.24450616023244
0.31 0.252530805195954
0.32 0.260541112723737
0.33 0.268543195905511
0.34 0.276532963791468
0.35 0.284504746770333
0.36 0.292461716956349
0.37 0.300412633111692
0.38 0.308349872257988
0.39 0.316362974870536
0.4 0.324381950069095
0.41 0.332396415321275
0.42 0.340397185896388
0.43 0.34837266114359
0.44 0.356339402214327
0.45 0.364299448130565
0.46 0.372235655358842
0.47 0.38016255595171
0.48 0.388065839318479
0.49 0.395951226196215
0.5 0.403812692569812
0.51 0.411661473472535
0.52 0.419488404316197
0.53 0.427292463970099
0.54 0.435075077376316
0.55 0.44283000029949
0.56 0.450559639603001
0.57 0.458268610869867
0.58 0.465946676190606
0.59 0.47359995880118
0.6 0.481222174987772
0.61 0.488802939837781
0.62 0.49635559641974
0.63 0.503873316959693
0.64 0.511355268555327
0.65 0.518796244582907
0.66 0.526194256303149
0.67 0.533548469467912
0.68 0.540858259734838
0.69 0.548115947179173
0.7 0.555319292855796
0.71 0.562463202359365
0.72 0.569548329774155
0.73 0.57657432601596
0.74 0.583525262117579
0.75 0.59040209209169
0.76 0.597201104898156
0.77 0.603910744911765
0.78 0.610531746861143
0.79 0.617049924024982
0.8 0.623451673165681
0.81 0.629729377622492
0.82 0.635869454629228
0.83 0.64185295518877
0.84 0.647690098020031
0.85 0.653346186114208
0.86 0.658795446696575
0.87 0.664009066690448
0.88 0.668953636996552
0.89 0.673596364067192
0.9 0.6778708023212
0.91 0.681706195161642
0.92 0.685017689441154
0.93 0.687663436680514
0.94 0.689468215819377
0.95 0.690149282922168
0.96 0.689247433561852
0.97 0.685935695199672
0.98 0.678428084116172
0.99 0.661358043610206
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/nerfacto-mcdropout/empirical_coverage_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.827242364485174, ymax=0.039392493546913,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 -0.0089069909877712
0.02 -0.0178202892862975
0.03 -0.0267326762183336
0.04 -0.0356442028510668
0.05 -0.0445578921165974
0.06 -0.0534680771676735
0.07 -0.0623817531902899
0.08 -0.071292637636608
0.09 -0.0802047614951154
0.1 -0.0891119026766454
0.11 -0.0980169454843696
0.12 -0.106923593520567
0.13 -0.115824976681131
0.14 -0.124725329737723
0.15 -0.133620337061113
0.16 -0.142514702133971
0.17 -0.151406474163765
0.18 -0.160294028368486
0.19 -0.169177317471501
0.2 -0.178059147853106
0.21 -0.186939075229097
0.22 -0.195813863767952
0.23 -0.204682985836357
0.24 -0.213552233198305
0.25 -0.222413232451416
0.26 -0.23127283112818
0.27 -0.240123815699133
0.28 -0.248970901968373
0.29 -0.257816663439913
0.3 -0.266652780631863
0.31 -0.275482218249424
0.32 -0.28430880077165
0.33 -0.293127085236719
0.34 -0.30193696127161
0.35 -0.310738373766188
0.36 -0.319534957544666
0.37 -0.328323658420408
0.38 -0.337104980085239
0.39 -0.345875813527067
0.4 -0.354639450361987
0.41 -0.363394726139769
0.42 -0.372142809538291
0.43 -0.380879135555895
0.44 -0.389605233619278
0.45 -0.398322699390863
0.46 -0.407027921359572
0.47 -0.415722058732072
0.48 -0.424404080117905
0.49 -0.433072205050358
0.5 -0.441727963623133
0.51 -0.450369144262343
0.52 -0.458999383127991
0.53 -0.467611150676451
0.54 -0.476204146909228
0.55 -0.484783475089022
0.56 -0.493346930856282
0.57 -0.501886989423749
0.58 -0.510413128953246
0.59 -0.518916271878224
0.6 -0.527401016343137
0.61 -0.53586593277167
0.62 -0.544304568253026
0.63 -0.552717811728751
0.64 -0.561104908424407
0.65 -0.56946744649973
0.66 -0.577804682688129
0.67 -0.586112075934195
0.68 -0.594381536729534
0.69 -0.602615565828893
0.7 -0.610817626975916
0.71 -0.61897938908783
0.72 -0.627102058659596
0.73 -0.635177583179071
0.74 -0.64320773837199
0.75 -0.651185909330783
0.76 -0.659111703631441
0.77 -0.666975300690961
0.78 -0.674774968722847
0.79 -0.682507627505783
0.8 -0.690164065078576
0.81 -0.69773841256879
0.82 -0.705217508284188
0.83 -0.712598771115833
0.84 -0.719868151068282
0.85 -0.72700697889094
0.86 -0.734000924277139
0.87 -0.740829375884478
0.88 -0.747474903366738
0.89 -0.753898377342809
0.9 -0.760073557057352
0.91 -0.765940226212572
0.92 -0.771440038607534
0.93 -0.776462869718439
0.94 -0.780898874787266
0.95 -0.784540758531558
0.96 -0.787055154706056
0.97 -0.787849870938261
0.98 -0.785619426159999
0.99 -0.776423747781326
};
\addplot [semithick, darkorange25512714]
table {%
0.01 -0.00889046459958966
0.02 -0.0177796156980996
0.03 -0.0266720827257805
0.04 -0.0355604141085444
0.05 -0.0444459648227016
0.06 -0.0533306202549497
0.07 -0.0622159109146751
0.08 -0.0710967113748008
0.09 -0.0799783544354731
0.1 -0.0888561320366923
0.11 -0.097729548706107
0.12 -0.106605652536182
0.13 -0.115478577304493
0.14 -0.124347675029182
0.15 -0.13321262496685
0.16 -0.142077561959736
0.17 -0.150936358433691
0.18 -0.159790302175451
0.19 -0.16864520358644
0.2 -0.177492117538826
0.21 -0.186337299200653
0.22 -0.195182138393236
0.23 -0.204019875761885
0.24 -0.212851635255831
0.25 -0.221682362062653
0.26 -0.230509211633434
0.27 -0.239324461668237
0.28 -0.248137483846661
0.29 -0.256940583868946
0.3 -0.265740554106605
0.31 -0.274532799757179
0.32 -0.283317850990316
0.33 -0.292093929054104
0.34 -0.300865209570289
0.35 -0.309629257623547
0.36 -0.318385733912542
0.37 -0.327135376724206
0.38 -0.335875704977965
0.39 -0.344610022918849
0.4 -0.353333224381196
0.41 -0.362047775860455
0.42 -0.370752508933266
0.43 -0.379445631277067
0.44 -0.388130328620071
0.45 -0.396801747771512
0.46 -0.40546032333596
0.47 -0.414109696291953
0.48 -0.422747200236957
0.49 -0.431370602957097
0.5 -0.439982103516837
0.51 -0.448578350399318
0.52 -0.457158134994293
0.53 -0.465722941266815
0.54 -0.474274922171076
0.55 -0.482805393398027
0.56 -0.491322624993705
0.57 -0.49981914635268
0.58 -0.50829633983644
0.59 -0.516755916907978
0.6 -0.525192311173585
0.61 -0.533605634985337
0.62 -0.541991309432144
0.63 -0.550354050569806
0.64 -0.558695025734355
0.65 -0.567006213315347
0.66 -0.575288073287817
0.67 -0.58353540185036
0.68 -0.591751062880459
0.69 -0.599937191601405
0.7 -0.608081762506041
0.71 -0.616187789816621
0.72 -0.624251080431273
0.73 -0.632271034752922
0.74 -0.640241281512838
0.75 -0.648161854699039
0.76 -0.656027005369666
0.77 -0.663829414414475
0.78 -0.67156658816267
0.79 -0.679236533219521
0.8 -0.686831684089836
0.81 -0.694344415597458
0.82 -0.701756177330285
0.83 -0.70906744371221
0.84 -0.71626036243613
0.85 -0.72332899970529
0.86 -0.73025390200524
0.87 -0.737011901861832
0.88 -0.743577234226205
0.89 -0.749922503251919
0.9 -0.756018659191296
0.91 -0.761799773679206
0.92 -0.767212846776941
0.93 -0.77215557979475
0.94 -0.776494169544796
0.95 -0.780035776825611
0.96 -0.782439969867819
0.97 -0.783113319120809
0.98 -0.780752465868505
0.99 -0.771409684873136
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 -0.00683462218583319
0.02 -0.015243872177041
0.03 -0.0236538786143788
0.04 -0.0320625835671748
0.05 -0.0404705381255289
0.06 -0.0488803694942348
0.07 -0.0572868055297105
0.08 -0.0656944229528676
0.09 -0.0740962297593343
0.1 -0.0824980161687995
0.11 -0.0908990821868374
0.12 -0.0992970824274131
0.13 -0.107693844077046
0.14 -0.116086952223602
0.15 -0.124476882734301
0.16 -0.132860365576506
0.17 -0.141237016367162
0.18 -0.149612135867499
0.19 -0.157982194965044
0.2 -0.166347457348928
0.21 -0.17470403202015
0.22 -0.18305693052211
0.23 -0.191398682781086
0.24 -0.199731725160193
0.25 -0.208057312295484
0.26 -0.216373218276259
0.27 -0.224678932841203
0.28 -0.232977156402481
0.29 -0.241259488398238
0.3 -0.249527830525844
0.31 -0.257783007942867
0.32 -0.266024451682241
0.33 -0.27425999958054
0.34 -0.282501500844751
0.35 -0.290743057033188
0.36 -0.298982025289261
0.37 -0.30721623408447
0.38 -0.315432434106922
0.39 -0.323643780663945
0.4 -0.331841489503916
0.41 -0.340025247105303
0.42 -0.348194150142739
0.43 -0.356353783476548
0.44 -0.364498007604146
0.45 -0.372632712775649
0.46 -0.380750845413828
0.47 -0.388854399332166
0.48 -0.396943177273354
0.49 -0.405015213646423
0.5 -0.413070356782019
0.51 -0.421109254711139
0.52 -0.429128745239223
0.53 -0.437125274558716
0.54 -0.445099569797205
0.55 -0.453052143380742
0.56 -0.460987387978836
0.57 -0.468891839495329
0.58 -0.476773384226001
0.59 -0.484630133520785
0.6 -0.492452786040412
0.61 -0.500243637196931
0.62 -0.508005786959754
0.63 -0.51573187221748
0.64 -0.523420754088782
0.65 -0.531077208802801
0.66 -0.538691859814828
0.67 -0.546270430288198
0.68 -0.553798564675491
0.69 -0.561280801522805
0.7 -0.568712784803199
0.71 -0.576089707214165
0.72 -0.583416373831632
0.73 -0.590676433274109
0.74 -0.597869825275519
0.75 -0.604995072067593
0.76 -0.612043591351132
0.77 -0.619009545382436
0.78 -0.625881013489792
0.79 -0.632653964813384
0.8 -0.639331742434363
0.81 -0.645890834754721
0.82 -0.652321108152728
0.83 -0.658604769768087
0.84 -0.664741186222278
0.85 -0.670707581219155
0.86 -0.676483462710868
0.87 -0.682040682587027
0.88 -0.687341502213515
0.89 -0.692346871307464
0.9 -0.69701072305789
0.91 -0.701252837142256
0.92 -0.7050001008161
0.93 -0.708121183767841
0.94 -0.710440869455979
0.95 -0.71169422202054
0.96 -0.711430904118533
0.97 -0.708863797103443
0.98 -0.702279728123336
0.99 -0.686528302732458
};
\addplot [semithick, crimson2143940]
table {%
0.01 -0.0053003946364582
0.02 -0.0135734403971889
0.03 -0.0218456477342144
0.04 -0.0301139190118289
0.05 -0.0383797187911772
0.06 -0.0466438741197682
0.07 -0.0549055926148589
0.08 -0.0631660878067267
0.09 -0.0714228758348942
0.1 -0.0796747057637268
0.11 -0.0879237830119182
0.12 -0.0961785374202051
0.13 -0.104426560897564
0.14 -0.112667699983485
0.15 -0.120908720167379
0.16 -0.129144373990527
0.17 -0.137378033932072
0.18 -0.145602015370513
0.19 -0.153819422855004
0.2 -0.16203207512125
0.21 -0.170232336714249
0.22 -0.178427218049432
0.23 -0.186617758712791
0.24 -0.194797648655501
0.25 -0.202974044550569
0.26 -0.211140935585117
0.27 -0.219291603723755
0.28 -0.22743773642695
0.29 -0.235572624668872
0.3 -0.243700207832095
0.31 -0.251818986075795
0.32 -0.259919710496579
0.33 -0.268014301301012
0.34 -0.276102274990653
0.35 -0.284174375452053
0.36 -0.292233770609617
0.37 -0.300285578255437
0.38 -0.308326608260792
0.39 -0.316362974870536
0.4 -0.324381950069095
0.41 -0.332396415321275
0.42 -0.340397185896388
0.43 -0.34837266114359
0.44 -0.356339402214327
0.45 -0.364299448130565
0.46 -0.372235655358842
0.47 -0.38016255595171
0.48 -0.388065839318479
0.49 -0.395951226196215
0.5 -0.403812692569812
0.51 -0.411661473472535
0.52 -0.419488404316197
0.53 -0.427292463970099
0.54 -0.435075077376316
0.55 -0.44283000029949
0.56 -0.450559639603001
0.57 -0.458268610869867
0.58 -0.465946676190606
0.59 -0.47359995880118
0.6 -0.481222174987772
0.61 -0.488802939837781
0.62 -0.49635559641974
0.63 -0.503873316959693
0.64 -0.511355268555327
0.65 -0.518796244582907
0.66 -0.526194256303149
0.67 -0.533548469467912
0.68 -0.540858259734838
0.69 -0.548115947179173
0.7 -0.555319292855796
0.71 -0.562463202359365
0.72 -0.569548329774155
0.73 -0.57657432601596
0.74 -0.583525262117579
0.75 -0.59040209209169
0.76 -0.597201104898156
0.77 -0.603910744911765
0.78 -0.610531746861143
0.79 -0.617049924024982
0.8 -0.623451673165681
0.81 -0.629729377622492
0.82 -0.635869454629228
0.83 -0.64185295518877
0.84 -0.647690098020031
0.85 -0.653346186114208
0.86 -0.658795446696575
0.87 -0.664009066690448
0.88 -0.668953636996552
0.89 -0.673596364067192
0.9 -0.6778708023212
0.91 -0.681706195161642
0.92 -0.685017689441154
0.93 -0.687663436680514
0.94 -0.689468215819377
0.95 -0.690149282922168
0.96 -0.689247433561852
0.97 -0.685935695199672
0.98 -0.678428084116172
0.99 -0.661358043610206
};
\end{axis}

\end{tikzpicture}


==> results/varyingview-mipnerf360-auce-coverage/nerfacto-mcdropout/empirical_coverage_negative_error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.039392493546913, ymax=0.827242364485174,
ytick style={color=black}
]
\addplot [semithick, black, dash pattern=on 1.5pt off 2.475pt]
table {%
0 0
1 0
};
\addplot [semithick, steelblue31119180]
table {%
0.01 0.0089069909877712
0.02 0.0178202892862975
0.03 0.0267326762183336
0.04 0.0356442028510668
0.05 0.0445578921165974
0.06 0.0534680771676735
0.07 0.0623817531902899
0.08 0.071292637636608
0.09 0.0802047614951154
0.1 0.0891119026766454
0.11 0.0980169454843696
0.12 0.106923593520567
0.13 0.115824976681131
0.14 0.124725329737723
0.15 0.133620337061113
0.16 0.142514702133971
0.17 0.151406474163765
0.18 0.160294028368486
0.19 0.169177317471501
0.2 0.178059147853106
0.21 0.186939075229097
0.22 0.195813863767952
0.23 0.204682985836357
0.24 0.213552233198305
0.25 0.222413232451416
0.26 0.23127283112818
0.27 0.240123815699133
0.28 0.248970901968373
0.29 0.257816663439913
0.3 0.266652780631863
0.31 0.275482218249424
0.32 0.28430880077165
0.33 0.293127085236719
0.34 0.30193696127161
0.35 0.310738373766188
0.36 0.319534957544666
0.37 0.328323658420408
0.38 0.337104980085239
0.39 0.345875813527067
0.4 0.354639450361987
0.41 0.363394726139769
0.42 0.372142809538291
0.43 0.380879135555895
0.44 0.389605233619278
0.45 0.398322699390863
0.46 0.407027921359572
0.47 0.415722058732072
0.48 0.424404080117905
0.49 0.433072205050358
0.5 0.441727963623133
0.51 0.450369144262343
0.52 0.458999383127991
0.53 0.467611150676451
0.54 0.476204146909228
0.55 0.484783475089022
0.56 0.493346930856282
0.57 0.501886989423749
0.58 0.510413128953246
0.59 0.518916271878224
0.6 0.527401016343137
0.61 0.53586593277167
0.62 0.544304568253026
0.63 0.552717811728751
0.64 0.561104908424407
0.65 0.56946744649973
0.66 0.577804682688129
0.67 0.586112075934195
0.68 0.594381536729534
0.69 0.602615565828893
0.7 0.610817626975916
0.71 0.61897938908783
0.72 0.627102058659596
0.73 0.635177583179071
0.74 0.64320773837199
0.75 0.651185909330783
0.76 0.659111703631441
0.77 0.666975300690961
0.78 0.674774968722847
0.79 0.682507627505783
0.8 0.690164065078576
0.81 0.69773841256879
0.82 0.705217508284188
0.83 0.712598771115833
0.84 0.719868151068282
0.85 0.72700697889094
0.86 0.734000924277139
0.87 0.740829375884478
0.88 0.747474903366738
0.89 0.753898377342809
0.9 0.760073557057352
0.91 0.765940226212572
0.92 0.771440038607534
0.93 0.776462869718439
0.94 0.780898874787266
0.95 0.784540758531558
0.96 0.787055154706056
0.97 0.787849870938261
0.98 0.785619426159999
0.99 0.776423747781326
};
\addplot [semithick, darkorange25512714]
table {%
0.01 0.00889046459958966
0.02 0.0177796156980996
0.03 0.0266720827257805
0.04 0.0355604141085444
0.05 0.0444459648227016
0.06 0.0533306202549497
0.07 0.0622159109146751
0.08 0.0710967113748008
0.09 0.0799783544354731
0.1 0.0888561320366923
0.11 0.097729548706107
0.12 0.106605652536182
0.13 0.115478577304493
0.14 0.124347675029182
0.15 0.13321262496685
0.16 0.142077561959736
0.17 0.150936358433691
0.18 0.159790302175451
0.19 0.16864520358644
0.2 0.177492117538826
0.21 0.186337299200653
0.22 0.195182138393236
0.23 0.204019875761885
0.24 0.212851635255831
0.25 0.221682362062653
0.26 0.230509211633434
0.27 0.239324461668237
0.28 0.248137483846661
0.29 0.256940583868946
0.3 0.265740554106605
0.31 0.274532799757179
0.32 0.283317850990316
0.33 0.292093929054104
0.34 0.300865209570289
0.35 0.309629257623547
0.36 0.318385733912542
0.37 0.327135376724206
0.38 0.335875704977965
0.39 0.344610022918849
0.4 0.353333224381196
0.41 0.362047775860455
0.42 0.370752508933266
0.43 0.379445631277067
0.44 0.388130328620071
0.45 0.396801747771512
0.46 0.40546032333596
0.47 0.414109696291953
0.48 0.422747200236957
0.49 0.431370602957097
0.5 0.439982103516837
0.51 0.448578350399318
0.52 0.457158134994293
0.53 0.465722941266815
0.54 0.474274922171076
0.55 0.482805393398027
0.56 0.491322624993705
0.57 0.49981914635268
0.58 0.50829633983644
0.59 0.516755916907978
0.6 0.525192311173585
0.61 0.533605634985337
0.62 0.541991309432144
0.63 0.550354050569806
0.64 0.558695025734355
0.65 0.567006213315347
0.66 0.575288073287817
0.67 0.58353540185036
0.68 0.591751062880459
0.69 0.599937191601405
0.7 0.608081762506041
0.71 0.616187789816621
0.72 0.624251080431273
0.73 0.632271034752922
0.74 0.640241281512838
0.75 0.648161854699039
0.76 0.656027005369666
0.77 0.663829414414475
0.78 0.67156658816267
0.79 0.679236533219521
0.8 0.686831684089836
0.81 0.694344415597458
0.82 0.701756177330285
0.83 0.70906744371221
0.84 0.71626036243613
0.85 0.72332899970529
0.86 0.73025390200524
0.87 0.737011901861832
0.88 0.743577234226205
0.89 0.749922503251919
0.9 0.756018659191296
0.91 0.761799773679206
0.92 0.767212846776941
0.93 0.77215557979475
0.94 0.776494169544796
0.95 0.780035776825611
0.96 0.782439969867819
0.97 0.783113319120809
0.98 0.780752465868505
0.99 0.771409684873136
};
\addplot [semithick, forestgreen4416044]
table {%
0.01 0.00812000579508921
0.02 0.0163543633595751
0.03 0.0246228849675825
0.04 0.0329123370471042
0.05 0.0412793882185198
0.06 0.0496487519435422
0.07 0.0580147035759785
0.08 0.066382339376775
0.09 0.0747439466892536
0.1 0.0831050622478443
0.11 0.0914641543750817
0.12 0.0998195962423178
0.13 0.10817363820981
0.14 0.116523486184996
0.15 0.124870447718133
0.16 0.133210025153764
0.17 0.141544061008254
0.18 0.14987666822348
0.19 0.158204736670869
0.2 0.16652845043261
0.21 0.174844945020255
0.22 0.183157763438638
0.23 0.191460261012318
0.24 0.199756059828845
0.25 0.208057312295484
0.26 0.216373218276259
0.27 0.224678932841203
0.28 0.232977156402481
0.29 0.241259488398238
0.3 0.249527830525844
0.31 0.257783007942867
0.32 0.266024451682241
0.33 0.27425999958054
0.34 0.282501500844751
0.35 0.290743057033188
0.36 0.298982025289261
0.37 0.30721623408447
0.38 0.315432434106922
0.39 0.323643780663945
0.4 0.331841489503916
0.41 0.340025247105303
0.42 0.348194150142739
0.43 0.356353783476548
0.44 0.364498007604146
0.45 0.372632712775649
0.46 0.380750845413828
0.47 0.388854399332166
0.48 0.396943177273354
0.49 0.405015213646423
0.5 0.413070356782019
0.51 0.421109254711139
0.52 0.429128745239223
0.53 0.437125274558716
0.54 0.445099569797205
0.55 0.453052143380742
0.56 0.460987387978836
0.57 0.468891839495329
0.58 0.476773384226001
0.59 0.484630133520785
0.6 0.492452786040412
0.61 0.500243637196931
0.62 0.508005786959754
0.63 0.51573187221748
0.64 0.523420754088782
0.65 0.531077208802801
0.66 0.538691859814828
0.67 0.546270430288198
0.68 0.553798564675491
0.69 0.561280801522805
0.7 0.568712784803199
0.71 0.576089707214165
0.72 0.583416373831632
0.73 0.590676433274109
0.74 0.597869825275519
0.75 0.604995072067593
0.76 0.612043591351132
0.77 0.619009545382436
0.78 0.625881013489792
0.79 0.632653964813384
0.8 0.639331742434363
0.81 0.645890834754721
0.82 0.652321108152728
0.83 0.658604769768087
0.84 0.664741186222278
0.85 0.670707581219155
0.86 0.676483462710868
0.87 0.682040682587027
0.88 0.687341502213515
0.89 0.692346871307464
0.9 0.69701072305789
0.91 0.701252837142256
0.92 0.7050001008161
0.93 0.708121183767841
0.94 0.710440869455979
0.95 0.71169422202054
0.96 0.711430904118533
0.97 0.708863797103443
0.98 0.702279728123336
0.99 0.686528302732458
};
\addplot [semithick, crimson2143940]
table {%
0.01 0.00780999875298506
0.02 0.0158186738855194
0.03 0.0238873468888926
0.04 0.0319892794636772
0.05 0.0401043872425141
0.06 0.048234528727475
0.07 0.0563980560833175
0.08 0.0645937077348345
0.09 0.0728044682029785
0.1 0.0810096064823076
0.11 0.089211405503537
0.12 0.0974187036167048
0.13 0.10561874916399
0.14 0.113811813953542
0.15 0.12200486249212
0.16 0.130192274425338
0.17 0.138378258105217
0.18 0.146555512280523
0.19 0.154725662487247
0.2 0.162890954824671
0.21 0.171044891379078
0.22 0.179193518902932
0.23 0.187338545261544
0.24 0.195473048689596
0.25 0.203603163539382
0.26 0.211724806323958
0.27 0.21983165704264
0.28 0.227931586212575
0.29 0.236021180116296
0.3 0.244103184032268
0.31 0.252174895635874
0.32 0.260230411610158
0.33 0.268278748603261
0.34 0.27631761939106
0.35 0.284339561111193
0.36 0.292347743782983
0.37 0.300349105683565
0.38 0.30833824025939
0.39 0.316362974870536
0.4 0.324381950069095
0.41 0.332396415321275
0.42 0.340397185896388
0.43 0.34837266114359
0.44 0.356339402214327
0.45 0.364299448130565
0.46 0.372235655358842
0.47 0.38016255595171
0.48 0.388065839318479
0.49 0.395951226196215
0.5 0.403812692569812
0.51 0.411661473472535
0.52 0.419488404316197
0.53 0.427292463970099
0.54 0.435075077376316
0.55 0.44283000029949
0.56 0.450559639603001
0.57 0.458268610869867
0.58 0.465946676190606
0.59 0.47359995880118
0.6 0.481222174987772
0.61 0.488802939837781
0.62 0.49635559641974
0.63 0.503873316959693
0.64 0.511355268555327
0.65 0.518796244582907
0.66 0.526194256303149
0.67 0.533548469467912
0.68 0.540858259734838
0.69 0.548115947179173
0.7 0.555319292855796
0.71 0.562463202359365
0.72 0.569548329774155
0.73 0.57657432601596
0.74 0.583525262117579
0.75 0.59040209209169
0.76 0.597201104898156
0.77 0.603910744911765
0.78 0.610531746861143
0.79 0.617049924024982
0.8 0.623451673165681
0.81 0.629729377622492
0.82 0.635869454629228
0.83 0.64185295518877
0.84 0.647690098020031
0.85 0.653346186114208
0.86 0.658795446696575
0.87 0.664009066690448
0.88 0.668953636996552
0.89 0.673596364067192
0.9 0.6778708023212
0.91 0.681706195161642
0.92 0.685017689441154
0.93 0.687663436680514
0.94 0.689468215819377
0.95 0.690149282922168
0.96 0.689247433561852
0.97 0.685935695199672
0.98 0.678428084116172
0.99 0.661358043610206
};
\end{axis}

\end{tikzpicture}

